MED-VT++: Unifying Multimodal Learning with a Multiscale Encoder-Decoder Video Transformer

In this paper, we present an end-to-end trainable unified multiscale encoder-decoder transformer that is focused on dense prediction tasks in video. The presented Multiscale Encoder-Decoder Video Transformer (MED-VT) uses multiscale representation throughout and employs an optional input beyond video (e.g., audio), when available, for multimodal processing (MED-VT++). Multiscale representation at both encoder and decoder yields three key benefits: (i) implicit extraction of spatiotemporal features at different levels of abstraction for capturing dynamics without reliance on input optical flow, (ii) temporal consistency at encoding and (iii) coarse-to-fine detection for high-level (e.g., object) semantics to guide precise localization at decoding. Moreover, we present a transductive learning scheme through many-to-many label propagation to provide temporally consistent video predictions. We showcase MED-VT/MED-VT++ on three unimodal video segmentation tasks (Automatic Video Object Segmentation (AVOS), actor-action segmentation and Video Semantic Segmentation (VSS)) as well as a multimodal segmentation task (Audio-Visual Segmentation (AVS)). Results show that the proposed architecture outperforms alternative state-of-the-art approaches on multiple benchmarks using only video (and optional audio) as input, without reliance on optical flow. Finally, to document details of the model's internal learned representations, we present a detailed interpretability study, encompassing both quantitative and qualitative analyses.

==> core/abstract.tex <==
Deep spatiotemporal models are used in a variety of computer vision tasks, such as action recognition and video object segmentation. Currently, there is a limited understanding of what information is captured by these models in their intermediate representations. For example, while it has been observed that action recognition algorithms are heavily influenced by visual appearance in single static frames, 
there is no quantitative methodology for evaluating such static bias in the latent representation compared to bias toward dynamic information (\eg motion).
We tackle this challenge by proposing a novel approach for quantifying the static and dynamic biases of any spatiotemporal model. To show the efficacy of our approach, we analyse two widely studied tasks, action recognition and video object segmentation. 
Our key findings are threefold: (i) Most examined spatiotemporal models are biased toward static information; although, certain two-stream architectures with cross-connections show a better balance between the static and dynamic information captured. (ii) Some datasets that are commonly assumed to be biased toward dynamics are actually biased toward static information. (iii) Individual units (channels) in an architecture can be biased toward static, dynamic or a combination of the two.


==> core/application.tex <==


% \begin{itemize}
%     \item Motivation: we want to explore (i) how the identified units affect performance and (ii) if there is a way to manipulate these biases, and if so, what effect does this have on performance.
%     \item We first evaluate the effect on performance by masking out static, dynamic, and random units
%     % \item Given that dynamic is the most important factor 
% \end{itemize}


% We have shown that model architectures and datasets can greatly impact the amount of static and dynamic information encoded in deep spatiotemporal models. Moreover, we explored how these factors are learned by the model throughout training. 
We have demonstrated the affect to which architectures, datasets and training protocols have on a model's biases. 
We now ask: (i) \textit{Is it possible to control the static and dynamic biases of a model?} and (ii) \textit{What impact do static and dynamic units have on performance?} 
We first show that the type of bias encoded by a unit greatly determines the impact it has on final performance through \textit{neuron removal} experiments for action recognition and video segmentation. 
Motivated by the varying impact different biases have on overall performance, we aim to improve the performance for each task. 
For action recognition, we propose \textit{StaticDropout}, a novel dropout strategy that uses our estimation technique to dropout static-biased units during training, with the ultimate goal of debiasing models away from static information. 
For AVOS, we perform a detailed analysis on cross connections and fusion design choices with respect to their static and dynamic biases and show how to encourage a previously static biased model to become more biased toward dynamics. In both domains, we show an improvement in performance for tasks that require dynamics.

\subsection{Neuron Removal}\label{sec:neuron_removal}
\vspace{-0.1cm}
To evaluate the effect of static and dynamic units on overall performance, we conduct perturbation experiments where we remove the top-$k$ units (\ie channels) that are biased toward the static or dynamic factor during inference and evaluate the performance drop. The removal is done by setting all activations to zero in the identified channels. We compare these static or dynamic biased units with respect to randomly selected channels. Figure~\ref{fig:unit_removal} shows the unit removal results for action recognition and AVOS. In action recognition we evaluate the final layer in the SlowFast model trained on SSv2 and evaluate on the SSv2 validation set to report the top-1 accuracy. As can be seen in Fig.~\ref{fig:unit_removal} (top left), the dynamic factor maximally reduces the model's performance, which may be because the SlowFast model encodes a significant amount of dynamic information in the fast branch and dynamics are important for the SSv2 dataset. 



\begin{figure} [t]
	\begin{center}
     \centering 
     \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture} 
%                  \begin{axis}[
%                  line width=1.0,
%                  title={SlowFast},
%                  title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
%                  xlabel={Top-k Units Masked},
%                  ylabel={Top-1 (\%)},
%                  xmin=900, xmax=2100,
%                  ymin=25, ymax=65,
%                  xtick={1000,1200,1400,1600,1800,2000},
%                 %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
%                  x tick label style={font=\tiny, rotate=0, anchor=north},
%                  y tick label style={font=\tiny},
%                  x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
%                  y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
%                  width=6.5cm,
%                  height=4.3cm, % height=4.3cm, 
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                 %  legend pos=south west,
%                  legend columns=2,
%                  legend style={
%                   nodes={scale=0.8, transform shape},
%                   cells={anchor=west},
%                   legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
%              ]
%              \addlegendentry{Dynamic}
%              \addplot[line width=0.8pt, mark size=1.0pt, color=cyan, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(1000, 51.44)
%                                   (1200, 49.69)
%                                   (1400, 47.69)
%                                   (1600, 42.77)
%                                   (1800, 37.46)
%                                   (2000, 28.05)};
%             \addlegendentry{Static}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=orange, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(1000, 53.436)
%                                   (1200, 52.469)
%                                   (1400, 51.293)
%                                   (1600, 49.62)
%                                   (1800, 46.587)
%                                   (2000, 39.799)};
%             \addlegendentry{Random}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(1000, 54.48)
%                                   (1200, 53.916)
%                                   (1400, 53.775)
%                                   (1600, 53.316)
%                                   (1800, 52.415)
%                                   (2000, 46.983)
%             };
%             \addlegendentry{Standard}
%              \addplot[line width=0.8pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(800, 54.9)
%                                   (2200, 54.9)};
%               \end{axis}
% \end{tikzpicture}
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 title={\textbf{SlowFast}},
                 title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
                %  xlabel={Top-k \% Units Masked},
                 ylabel={Top-1 Acc. (\%)},
                 xmin=39, xmax=91,
                 ymin=25, ymax=65,
                 xtick pos=left,
                 ytick pos=bottom,
                 xtick={50,60,70,80},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\small, rotate=0, anchor=north},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                %  x label style={at={(axis description cs:0.5,0.0)},anchor=north,font=\large},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.3cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                %  legend pos=south west,
                 legend columns=2,
                 legend style={
                %  draw=none,
                  nodes={scale=0.52, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.37,0.05)},anchor=south,row sep=0.01pt}, font =\large}
             ]
             \addlegendentry{Dynamic}
             \addplot[line width=1.2pt, mark size=1.7pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(43.4, 51.44)
                                  (52.08, 49.69)
                                  (60.76, 47.69)
                                  (69.44, 42.77)
                                  (78.1, 37.46)
                                  (86.80, 28.05)};
                    %  coordinates {(1000, 51.44)
                    %               (1200, 49.69)
                    %               (1400, 47.69)
                    %               (1600, 42.77)
                    %               (1800, 37.46)
                    %               (2000, 28.05)};
            \addlegendentry{Static}
            \addplot[line width=1.2pt, mark size=1.7pt, color=red, mark=square,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(43.4, 53.436)
                                  (52.08, 52.469)
                                  (60.76, 51.293)
                                  (69.44, 49.62)
                                  (78.1, 46.587)
                                  (86.80, 39.799)};
                    %  coordinates {(1000, 53.436)
                    %               (1200, 52.469)
                    %               (1400, 51.293)
                    %               (1600, 49.62)
                    %               (1800, 46.587)
                    %               (2000, 39.799)};
            \addlegendentry{Random}
            \addplot[line width=1.2pt, mark size=1.7pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(43.4, 54.48)
                                  (52.08, 53.916)
                                  (60.76, 53.775)
                                  (69.44, 53.316)
                                  (78.1, 52.415)
                                  (86.80, 46.983)
                                  };
                    %  coordinates {(1000, 54.48)
                    %               (1200, 53.916)
                    %               (1400, 53.775)
                    %               (1600, 53.316)
                    %               (1800, 52.415)
                    %               (2000, 46.983)
            % };
            \addlegendentry{NoDropout}
             \addplot[line width=1.2pt, mark size=0, color=gray, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0, 54.9)
                                  (100, 54.9)};
              \end{axis}
\end{tikzpicture}
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 title={\textbf{MATNet - Fusion Layer 2}},
                 title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
                %  xlabel={Top-k \% Units Masked},
                 ylabel={mIoU (\%)},
                 xmin=30, xmax=80,
                 ymin=55, ymax=70,
                 xtick pos=left,
                 ytick pos=bottom,
                 xtick={40,50,60,70},
                 ytick={55, 60, 65},
                 x tick label style={font=\small, rotate=0, anchor=north},
                 y tick label style={font=\small},
                %  x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.3cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                %  legend pos=south west,
                % legend columns=2,
                %   legend style={
                %  draw=none,
                %   nodes={scale=0.63, transform shape},
                %   cells={anchor=west},
                %   legend style={at={(0.5,1.15)},anchor=south,row sep=0.01pt}, font =\large}
             ]

            %  \addlegendentry{Dynamic}
             \addplot[line width=1.2pt, mark size=1.7pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 58.8)
                                  (50, 57.4)
                                  (60, 56.5)
                                  (70, 56.1)};
            % \addlegendentry{Static}
            \addplot[line width=1.2pt, mark size=1.7pt, color=red, mark=square,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 61.1)
                                  (50, 57.3)
                                  (60, 56.4)
                                  (70, 56.5)};
            % \addlegendentry{Random}
            \addplot[line width=1.2pt, mark size=1.7pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 61.7)
                                  (50, 61.0)
                                  (60, 60.7)
                                  (70, 58.6)
            };
            % \addlegendentry{Standard}
             \addplot[line width=1.2pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(30, 66.9)
                                  (80, 66.9)};
              \end{axis}
\end{tikzpicture}}
\vspace{-0.2cm}
% \hspace{0.1cm}
% \begin{tikzpicture} 
%                  \begin{axis}[
%                  line width=1.0,
%                  title={MATNet - Fusion Layer 3},
%                  title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
%                  xlabel={Top-k \% Units Masked},
%                  ylabel={},
%                  xmin=30, xmax=80,
%                  ymin=50, ymax=70,
%                  xtick={40,50,60,70},
%                 %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
%                  x tick label style={font=\tiny, rotate=0, anchor=north},
%                  y tick label style={font=\tiny},
%                  x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
%                  y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
%                  width=6.5cm,
%                  height=4.3cm, % height=4.3cm, 
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                 %  legend pos=south west,
%                  %legend columns=2,
%                  %legend style={
%                  % nodes={scale=0.8, transform shape},
%                  % cells={anchor=west},
%                  % legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
%              ]
            
%              %\addlegendentry{Dynamic}
%              \addplot[line width=0.8pt, mark size=1.0pt, color=cyan, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(40, 61.7)
%                                   (50, 61.9)
%                                   (60, 61.5)
%                                   (70, 59.8)};
%             %\addlegendentry{Static}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=orange, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(40, 55.6)
%                                   (50, 50.8)
%                                   (60, 51.4)
%                                   (70, 50.8)};
%             %\addlegendentry{Random}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(40, 62.3)
%                                   (50, 62.1)
%                                   (60, 61.8)
%                                   (70, 60.8)
%             };
%             %\addlegendentry{Standard}
%              \addplot[line width=0.8pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(30, 66.9)
%                                   (80, 66.9)};
%               \end{axis}
% \end{tikzpicture}
\resizebox{0.49\textwidth}{!}{
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 title={\textbf{MATNet - Fusion Layer 4}},
                    title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
                 xlabel={Top-k \% Units Masked},
                 ylabel={mIoU (\%)},
                 xtick pos=left,
                 ytick pos=bottom,
                 xmin=20, xmax=80,
                 ymin=0, ymax=80,
                 xtick={30,40,50,60,70},
                 ytick={20,40,60},
                 x tick label style={font=\small, rotate=0, anchor=north},
                 y tick label style={font=\small},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.3cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                %  legend pos=south west,
                 %legend columns=2,
                 %legend style={
                 % nodes={scale=0.8, transform shape},
                 % cells={anchor=west},
                 % legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
             ]
            %
             %\addlegendentry{Dynamic}
             \addplot[line width=1.2pt, mark size=1.7pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(30, 53.2)
                                  (40, 52.3)
                                  (50, 49.4)
                                  (60, 31.2)
                                  (70, 2.9)};
            %\addlegendentry{Static}
            \addplot[line width=1.2pt, mark size=1.7pt, color=red, mark=square,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(30, 21.7)
                                  (40, 1.6)
                                  (50, 1.969784267764861e-06)
                                  (60, 3.4545299701601246e-05)
                                  (70, 1.0245879243979795e-07)};
            %\addlegendentry{Random}
            \addplot[line width=1.2pt, mark size=1.7pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(30, 61.3)
                                  (40, 58.8)
                                  (50, 53.2)
                                  (60, 45.8)
                                  (70, 49.5)
            };
            %\addlegendentry{Standard}
             \addplot[line width=1.2pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(20, 66.9)
                                  (80, 66.9)};
              \end{axis}
\end{tikzpicture}
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 title={\textbf{MATNet - Fusion Layer 5}},
                 title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
                 xlabel={Top-k \% Units Masked},
                 ylabel={mIoU (\%)},
                 xmin=30, xmax=80,
                 ymin=51, ymax=70,
                xtick pos=left,
                ytick pos=bottom,
                 xtick={40,50,60,70},
                 ytick={55, 60, 65},
                 x tick label style={font=\small, rotate=0, anchor=north},
                 y tick label style={font=\small},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.3cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                %  legend pos=south west,
                 %legend columns=2,
                 %legend style={
                 % nodes={scale=0.8, transform shape},
                 % cells={anchor=west},
                 % legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
             ]
            
             %\addlegendentry{Dynamic}
             \addplot[line width=1.2pt, mark size=1.7pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 60.1)
                                  (50, 59.2)
                                  (60, 58.3)
                                  (70, 55.8)};
            %\addlegendentry{Static}
            \addplot[line width=1.2pt, mark size=1.7pt, color=red, mark=square,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 55.9)
                                  (50, 56.5)
                                  (60, 55.2)
                                  (70, 54.8)};
            %\addlegendentry{Random}
            \addplot[line width=1.2pt, mark size=1.7pt, color=green, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(40, 60.9)
                                  (50, 60.2)
                                  (60, 60.5)
                                  (70, 60.3)
            };
            %\addlegendentry{Standard}
             \addplot[line width=1.2pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(30, 66.9)
                                  (80, 66.9)};
              \end{axis}
\end{tikzpicture}
}
\end{center}
\vspace{-0.57cm}
\caption{Top-$k$ unit removal results for static and dynamic factors with respect to random units on: (action recognition) the final layer of SlowFast model trained on SSv2 dataset, and (video object segmentation) three fusion layers of the MATNet model trained on DAVIS and YouTube-VOS.}\label{fig:unit_removal}
\vspace{-0.56cm}
\end{figure}

We conduct similar experiments to AVOS for the early and late fusion layers of the MATNet model trained on DAVIS and YouTube-VOS. 
Empirically, we found that at intermediate layers there is a higher chance of randomly selecting units that cumulatively have a significant impact on the performance unlike the final layers, which was also found in~\cite{cheng2022deeply}. Thus, in video object segmentation, as we remove units from the intermediate fusion layers (unlike action recognition where we ablate the final layer), we randomly sample from the units that are least biased towards the dominant factor (i.e., static or dynamic) of that layer to avoid the aforementioned scenario. More specifically, the random baseline first takes the least biased units toward the significant factor of this layer (\ie dynamics in fusion layer 2, and static in other fusion layers) and then randomly samples $x\%$ units within $(x+5)\%$ of these units.
We evaluate on the moving camouflaged animals~\cite{lamdouar2020betrayed} (MoCA) dataset, where the objects of interest are camouflaged animals and hence largely indistinguishable from their backgrounds in the absence of motion, and report the mean intersection over union (mIoU) (see Sec.~\ref{sec:vos_cc_study} for more details on evaluation). The results in Fig.~\ref{fig:unit_removal} (bottom left and right) consistently demonstrate that for every fusion layer the factor with the highest impact on performance is the factor it is most biased toward, as examined earlier (Fig.~\ref{fig:stagewise_vos}c and Sec.~\ref{sec:epochwise_vos}).

In both tasks, these experiments document that masking out the top-$k$ channels based on our metric can help remove biased units in the model and consequently affect its accuracy more compared with randomly selected channels. We now aim to use these insights to show possible mechanisms for improving the performance of a model.






\begin{figure}[t]
    \includegraphics[width=0.5\textwidth]{images/Staticdropout_v4.pdf}
    \vspace{-0.67cm}
    \caption{An overview of our StaticDropout method. Given a video, $v_1$, we generate $v_2$ by randomly shuffling the frames. $v_1$ and $v_2$ are passed through the model, $f_\theta$, to produce intermediate representations of the videos, $z_1$ and $z_2$. Using these representations, we estimate the mutual information (using \ref{eq:biasscores}) of each channel, $i$, between the two representations, $S_i$. We determine the probability of dropping out channel, $p_i$, by performing a Softmax over $S_i$. }
    \label{fig:staticdropout_method}
    \vspace{-0.7cm}
\end{figure}

\vspace{-0.4cm}
\subsection{StaticDropout}\label{sec:staticdropout}
\vspace{-0.1cm}
We propose StaticDropout, a semantically guided dropout technique with the goal of static-debiasing a model. Previous work, InfoDropout~\cite{shi2020informative}, used a measure of self information to identify neurons in a CNN that encode texture information for image-based models. Alternatively, we perform StaticDropout during training on static-biased channels in action recognition models.

\textbf{Approach.} Our overall approach is outlined in Fig.~\ref{fig:staticdropout_method}. We determine the channels in the model encoding static information by constructing statically similar video pairs during training. More specifically, given a video $v_1$, we shuffle the video frames to generate $v_2$. We pass both representations through the model to obtain intermediate representations $z_1$ and $z_2$ from layer $l$ (for fair comparison against standard dropout, we set $l$ to the last layer before the fully connected layer, and hereon omit $l$ for brevity). Using the unitwise metric, (\ref{eq:bias_scores_indv}), we calculate a score, $S_i$, representing the static information encoded by channel $i$. We calculate the probability of dropping channel $i$ via a multinomial distribution defined as

\vspace{-0.25cm}
\begin{equation}\label{eq:static_dropout}
p_i = \frac{e^{S_i}}{\sum^C_{k=1} e^{S_k}}.
\end{equation}
\vspace{-0.2cm}








% \begin{figure} [t]
% 	\begin{center}
%      \centering 
%      %\vspace{-0.1cm}
%      \resizebox{0.7\textwidth}{!}{
% \begin{tikzpicture} 
%                  \begin{axis}[
%                  line width=1.0,
%                  title={Uniform Noise - Diving48},
%                  title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
%                  xlabel={Uniform Noise Width},
%                  ylabel={Top-1 (\%)},
%                  xmin=-0.1, xmax=2.1,
%                  ymin=35, ymax=73,
%                  xtick={0.5,1,1.5,2},
%                  ytick={40, 50, 60, 70},
%                  x tick label style={font=\tiny, rotate=0, anchor=north},
%                  y tick label style={font=\tiny},
%                  x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
%                  y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
%                  width=6.5cm,
%                  height=4.3cm, % height=4.3cm, 
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                 %  legend pos=south west,
%                  legend columns=2,
%                  legend style={
%                   nodes={scale=0.7, transform shape},
%                   cells={anchor=west},
%                   legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
%              ]
%              \addlegendentry{Standard}
%              \addplot[line width=0.8pt, mark size=1.0pt, color=red, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(0.0, 70)
%                                   (0.5, 68.5)
%                                   (1.0, 60)
%                                   (1.5, 48.7)
%                                   (2.0, 37.61)};
%             \addlegendentry{Ours}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=blue, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(0.0, 70.6)
%                                   (0.5, 70.7)
%                                   (1.0, 62.8)
%                                   (1.5, 53.3)
%                                   (2.0, 42.0)};
%             % \addlegendentry{Standard}
%             %  \addplot[line width=0.8pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
%                     %  coordinates {(800, 54.9)
%                     %               (2200, 54.9)};
%               \end{axis}
% \end{tikzpicture}
% \hspace{0.1cm}
% \begin{tikzpicture} 
%                  \begin{axis}[
%                  line width=1.0,
%                  title={Gaussian Noise - Diving48},
%                  title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
%                  xlabel={Standard Deviation},
%                  ylabel={Top-1 (\%)},
%                  xmin=-0.05, xmax=0.75,
%                  ymin=20, ymax=75,
%                  xtick={0.1,0.3,0.5,0.7},
%                  ytick={30, 40, 50, 60, 70},
%                  x tick label style={font=\tiny, rotate=0, anchor=north},
%                  y tick label style={font=\tiny},
%                  x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
%                  y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
%                  width=6.5cm,
%                  height=4.3cm, % height=4.3cm, 
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                 %  legend pos=south west,
%                  legend columns=2,
%                  legend style={
%                   nodes={scale=0.7, transform shape},
%                   cells={anchor=west},
%                   legend style={at={(0.36,0.0)},anchor=south,row sep=0.01pt}, font =\small}
%              ]
%              \addlegendentry{Standard}
%              \addplot[line width=0.8pt, mark size=1.0pt, color=red, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(0.0, 70)
%                                   (0.1, 57.82)
%                                   (0.2, 47.82)
%                                   (0.3, 40.51)
%                                   (0.4, 34.77)
%                                   (0.5, 28.88)
%                                   (0.6, 24.31)
%                                   (0.7, 21.37)};
%             \addlegendentry{Ours}
%             \addplot[line width=0.8pt, mark size=1.0pt, color=blue, mark=*,error bars/.cd, y dir=both, y explicit,]
%                      coordinates {(0.0, 70.6)
%                                   (0.1, 60.76)
%                                   (0.2, 52.28)
%                                   (0.3, 43.96)
%                                   (0.4, 37.82)
%                                   (0.5, 31.73)
%                                   (0.6, 27.16)
%                                   (0.7, 23.4)};
%             % \addlegendentry{Standard}
%             %  \addplot[line width=0.8pt, mark size=0, color=gray, mark=*,error bars/.cd, y dir=both, y explicit,]
%                     %  coordinates {(800, 54.9)
%                     %               (2200, 54.9)};
%               \end{axis}
% \end{tikzpicture}
% }
% \end{center}
% \caption{Robustness evaluation of our StaticDrop algorithm. We are more robust to all levels of noise for both Uniform and Gaussian noise settings.}\label{fig:ar_noise}
% \end{figure}


% \begin{figure*} [t]
%  \def\arraystretch{1.35}
%  \setlength\tabcolsep{2.4pt}
% \centering
% \begin{minipage}{1.0\linewidth}
% \resizebox{1.0\textwidth}{!}{
% 	\begin{tabu}{c|c | cccccc | cccccc}
% 	\tabucline[1pt]{-}
% 	 \multirow{3}{*}{Model}&\multirow{3}{*}{Dropout}&  \multicolumn{6}{c|}{\textbf{Diving48}} & \multicolumn{6}{c}{\textbf{SSv2}} \\
% 	 \cline{3-14}
% 	 && \multicolumn{2}{c}{\textbf{Top-1 Acc (\%)}} &\multicolumn{2}{c}{\textbf{Top-5 Acc (\%)}}& \multicolumn{2}{c|}{\textbf{Dims (\%)}} & \multicolumn{2}{c}{\textbf{Top-1 Acc (\%)}} &\multicolumn{2}{c}{\textbf{Top-5 Acc (\%)}}& \multicolumn{2}{c}{\textbf{Dims (\%)}} \\
% 	 \cline{3-14}
% 	  & &Normal & Shuffled &Normal& Shuffled & Dyn. & Stat. & Normal& Shuffled & Normal& Shuffled & Dyn. & Stat.\\
% 	   %\tabucline[1pt]{-}
% 	   \cline{1-14}
% 	   \multirow{3}{*}{3D ResNet18}&None & 64.6 & 39.6 & 91.9 & 77.9 & 19.3 & 38.0 & 49.4 & 19.8 & 77.4 & 45.7 & 28.6 & 30.7 \\
% 	   &Normal  & 64.8 & 41.2&  92.3& 78.3 &20.4& 36.0& 49.8 & 18.5 & 78.2 & 45.2 & 29.0 & 29.9 \\
% 	   &StaticDropout  &64.2&19.1&91.3&48.6&20.5 & 35.5& 49.9 & 13.7 & 78.2 & 33.8 & 30.2 & 28.2 \\
% 	   \cline{1-14}
% 	   \multirow{3}{*}{3D ResNet50}&None & 71.3& 45.1 & 93.2 & 80.6 &20.2& 36.9& 53.9&22.9&81.4&49.7&28.6 & 30.6\\
% 	   &Normal & 72.0 & 47.8 &93.3& 82.7 &22.9& 33.6,& 54.1 & 22.3 & 82.2 & 50.1 & 28.9 & 30.5\\
% 	   &StaticDropout& 70.4 & 17.0 & 92.5 & 42.4 &22.7 & 31.4& 54.8 & 14.4 & 81.9 & 34.8 &29.3& 27.7\\
% 	   \cline{1-14}
% 	   %\multirow{3}{*}{I3D}&None & 59.2 & 45.79 & 89.8 & 83.1 & 18.3 & 37.0 & 52.8 & 20.2 & 80.2 & 45.9 & 26.1 & 33.8 \\
% 	   %&Normal & 59.9 & 45.1 & 90.6 & 81.42 & 17.7 & 38.2  & 53.3 & 19.3 & 72 & 46.1 &29.4 & 29.8 \\
% 	   %%\cline{2-13}
% 	   %&StaticDropout &TBD&TBD&TBD&TBD&TBD&TBD &-&-&-&-&-&- \\
% 	  % \hline
% 	\tabucline[1pt]{-}
% 	\end{tabu}}
% 		\end{minipage}
% \caption{StaticDropout results for SlowOnly trained on Diving48 and SSv2. Models trained with StaticDropout result in significantly less static bias and more dynamic bias compared to the regular dropout and no dropout baselines.}\label{fig:AR_infodrop}
% \end{figure*}





% \begin{figure} [t]
% 	\begin{center}
% % 	\put(0,9){{\small Top: \textcolor{red}{Test}}}
%      \centering 
%      %\vspace{-0.1cm}
%      \resizebox{0.49\textwidth}{!}{
% 	\begin{tikzpicture} \ref{shuff_ss_legend}
%     \begin{axis}[
%       line width=1.0,
%         title={SSv2 - Shuffled Frames Val.},
%         title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
%         xlabel={Dropout Type},
%         % x label style={font=\small},
%         ylabel={Relative Performance (\%)},
%         % xmin=0, xmax=550,
%         ymin=27, ymax=46,
%         % xtick={50,100,200,300,400,500},
%         ytick={0,10,15,20,25,30,35,40,45},
%         symbolic x coords={None, Normal, SD0.1,SD0.3, SD0.5, SD0.7},
%         xtick=data,
%         x tick label style={font=\footnotesize,rotate=25,anchor=east},
%         % x tick label style={font=\footnotesize,rotate=20,anchor=east},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
%         y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
%         xtick pos=left,
%         ytick pos=bottom,
%         width=6.7cm,
%         height=5.5cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         major grid style={dotted,green!20!black},
%         legend style={
%          %draw=none,
%          nodes={scale=0.9, transform shape},
%          cells={anchor=west},
%          legend style={at={(1.4,0.25)},anchor=south}, font =\footnotesize},
%          %legend columns=1,
%          legend entries={[black]3DResNet50,[black]3DResNet18},
%         legend to name=shuff_ss_legend,
%     ]
%     % R50
%     \addplot[only marks,mark size=4pt,color=purple,mark=x,]
%     coordinates {(None,42.486) (Normal,41.220) (SD0.1,35.748) (SD0.3,31.851) (SD0.5,30.389) (SD0.7,30.635)};
        
%     % R18
%     \addplot[only marks,mark size=3.2pt,color=blue,mark=o,]
%         coordinates {(None,40.113) (Normal,37.138) (SD0.1,35.407) (SD0.3,34.510) (SD0.5,32.837) (SD0.7,31.404)};
        
        
%     % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
% 	   % coordinates {([normalized]-10,0)([normalized]10,0)};
%     \end{axis}
% \end{tikzpicture}
% \hspace{0.1cm}
% 	\begin{tikzpicture} %\ref{dim_ss_legend}
%     \begin{axis}[
%       line width=1.0,
%         title={SSv2 - Dyn/Static Dims},
%         title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
%         xlabel={Dropout Type},
%         % x label style={font=\small},
%         ylabel={Fraction of Dyn Dims (\%)},
%         % xmin=0, xmax=550,
%         ymin=20, ymax=103,
%         % xtick={50,100,200,300,400,500},
%         ytick={0,10,20,30,40,50,60,70,80,90},
%         symbolic x coords={None, Normal, SD0.1,SD0.3, SD0.5, SD0.7},
%         xtick=data,
%         x tick label style={font=\footnotesize,rotate=25,anchor=east},
%         % x tick label style={font=\footnotesize,rotate=20,anchor=east},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
%         y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
%         xtick pos=left,
%         ytick pos=bottom,
%         width=6.7cm,
%         height=5.5cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         major grid style={dotted,green!20!black},
%         legend style={
%          %draw=none,
%          nodes={scale=0.9, transform shape},
%          cells={anchor=west},
%          legend style={at={(1.4,0.25)},anchor=south}, font =\footnotesize},
%          %legend columns=1,
%          legend entries={[black]3DResNet50,[black]3DResNet18},
%         legend to name=dim_ss_legend,
%     ]
%     % R50
%     \addplot[only marks,mark size=4pt,color=purple,mark=x,]
%     coordinates {(None,39.28571429) (Normal,61.047463180) (SD0.1,76.7) (SD0.3,81.0) (SD0.5,90.7) (SD0.7,89.2)};
        
%     % R18
%     \addplot[only marks,mark size=3.2pt,color=blue,mark=o,]
%         coordinates {(None,31.80987203) (Normal,60.9671848) (SD0.1,64.8) (SD0.3,79.7) (SD0.5,88.8) (SD0.7,93.6)};
        
        
%     % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
% 	   % coordinates {([normalized]-10,0)([normalized]10,0)};
%     \end{axis}
% \end{tikzpicture}}
% \hspace{0.1cm}
% \resizebox{0.49\textwidth}{!}{
% 	\begin{tikzpicture} %\ref{shuff_ss_legend}
%     \begin{axis}[
%       line width=1.0,
%         title={D48 - Shuffled Frames Val.},
%         title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
%         xlabel={Dropout Type},
%         % x label style={font=\small},
%         ylabel={Relative Performance (\%)},
%         % xmin=0, xmax=550,
%         ymin=35, ymax=74,
%         % xtick={50,100,200,300,400,500},
%         ytick={0,10,20,30,40,50,60,70,80,90},
%         symbolic x coords={None, Normal, SD0.1,SD0.3, SD0.5, SD0.7},
%         xtick=data,
%         x tick label style={font=\footnotesize,rotate=25,anchor=east},
%         % x tick label style={font=\footnotesize,rotate=20,anchor=east},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
%         y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
%         xtick pos=left,
%         ytick pos=bottom,
%         width=6.7cm,
%         height=5.5cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         major grid style={dotted,green!20!black},
%         legend style={
%          %draw=none,
%          nodes={scale=0.9, transform shape},
%          cells={anchor=west},
%          legend style={at={(1.4,0.25)},anchor=south}, font =\footnotesize},
%          %legend columns=1,
%          legend entries={[black]3DResNet50,[black]3DResNet18},
%         legend to name=shuff_ss_legend,
%     ]
    
%     % R50
%     \addplot[only marks,mark size=4pt,color=purple,mark=x,]
%     coordinates {(None,63.323) (Normal,66.849) (SD0.1,47.576) (SD0.3,44.987) (SD0.5,43.433) (SD0.7,42.193)};
        
%     % R18
%     \addplot[only marks,mark size=3.2pt,color=blue,mark=o,]
%         coordinates {(None,61.391) (Normal,63.591) (SD0.1,47.413) (SD0.3,46.258) (SD0.5,44.479) (SD0.7,41.466)};
        
        
%     % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
% 	   % coordinates {([normalized]-10,0)([normalized]10,0)};
%     \end{axis}
% \end{tikzpicture}
% \hspace{0.1cm}
% 	\begin{tikzpicture} %\ref{dim_ss_legend}
%     \begin{axis}[
%       line width=1.0,
%         title={D48 - Dyn/Static Dims},
%         title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
%         xlabel={Dropout Type},
%         % x label style={font=\small},
%         ylabel={Fraction of Dyn Dims (\%)},
%         % xmin=0, xmax=550,
%         ymin=-5, ymax=45,
%         % xtick={50,100,200,300,400,500},
%         ytick={0,10,20,30,40,50,60,70,80,90},
%         symbolic x coords={None, Normal, SD0.1, SD0.3, SD0.5, SD0.7},
%         xtick=data,
%         x tick label style={font=\footnotesize,rotate=25,anchor=east},
%         % x tick label style={font=\footnotesize,rotate=20,anchor=east},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
%         y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
%         xtick pos=left,
%         ytick pos=bottom,
%         width=6.7cm,
%         height=5.5cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         major grid style={dotted,green!20!black},
%         legend style={
%          %draw=none,
%          nodes={scale=0.9, transform shape},
%          cells={anchor=west},
%          legend style={at={(1.4,0.25)},anchor=south}, font =\footnotesize},
%          %legend columns=1,
%          legend entries={[black]3DResNet50,[black]3DResNet18},
%         legend to name=dim_ss_legend,
%     ]
    
%     \addplot[only marks,mark size=4pt,color=purple,mark=x,]
%     coordinates {(None,4.085872576) (Normal,10.64204046) (SD0.1,9.0) (SD0.3,11.9) (SD0.5,29.9) (SD0.7,42.3)};
        
%     \addplot[only marks,mark size=3.2pt,color=blue,mark=o,]
%         coordinates {(None,0.05733944954) (Normal,0.7343941248) (SD0.1,0.3) (SD0.3,1.8) (SD0.5,5.0) (SD0.7,4.4)};
        
        
%     % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
% 	   % coordinates {([normalized]-10,0)([normalized]10,0)};
%     \end{axis}
% \end{tikzpicture}
% }
% \end{center}
% \caption{StaticDropout influences the static and dynamic information of a model. We evaluate the relative performance of a model evaluate on normal \vs shuffled frames at validation time (left) and show the fraction of channels encoding dynamic information relative to the channels encoding either static or dynamic (right). Larger StaticDropout rates generally result in less bias toward static information.}
% \end{figure}\label{fig:static_dropout_bias1}




\noindent\textbf{Evaluation Protocol.} We first demonstrate the ability of our proposed StaticDropout technique to manipulate static and dynamic biases as measured by two different metrics. For the first metric, we use the unitwise metric, (\ref{eq:ind_bias_scores_diff_b}), to calculate the ratio of dynamic units relative to dynamic and static units. The second metric is the model's relative validation performance on shuffled \vs unshuffle frames. We apply StaticDropout to two different 3D-Resnet variants (\ie the SlowOnly architecture) with 18 and 50 layers, on two different datasets, Diving48 and SSv2.

\textbf{Implementation Details.} Models trained on SSv2 are trained with the original SlowFast~\cite{feichtenhofer2019slowfast} repository hyperparameters. 
They are trained for 30 epochs and use a cosine learning rate decay with three warmup epochs, a base learning rate of 0.1 and a warmup starting learning rate of 0.08.
Models trained on Diving48 are trained for 100 epochs and use a cosine learning rate decay with 10 warmup epochs, a base learning rate of 0.1 and a warmup starting learning rate of 0.01. We experiment with dropout rates of $r=\{0.1,0.3,0.5,0.7\}$. The static channel scores, $S_i$, are re-estimated using \ref{eq:static_dropout} every 30 iterations. Following InfoDropout~\cite{shi2020informative}, we finetune our models without any dropout with a learning rate of 1e-5 for two and five epochs on SSv2 and Diving48, respecively. For baselines, we consider the same model architectures with standard dropout~\cite{srivastava2014dropout} and without any dropout applied. 


\begin{figure} [t]
	\begin{center}
     \centering 
     \resizebox{0.49\textwidth}{!}{
	\begin{tikzpicture}\ref{bias_eval_legend}
    \begin{axis}[
       line width=1.0,
        title={Shuffled Frames},
        title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
        xlabel={Dropout Type},
        ylabel={Relative Performance (\%)},
        ymin=25, ymax=75,
        ytick={0,10,20,30,40,50,60,70,80},
        symbolic x coords={None, Normal, SD0.1,SD0.3, SD0.5, SD0.7},
        xtick=data,
        x tick label style={font=\footnotesize,rotate=25,anchor=east},
        % x tick label style={font=\footnotesize,rotate=20,anchor=east},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
        y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
        xtick pos=left,
        ytick pos=bottom,
        width=6.7cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
         %draw=none,
         nodes={scale=0.9, transform shape},
         cells={anchor=west},
         legend style={at={(3.26,3)},anchor=south}, font =\footnotesize},
         legend columns=2,
         legend entries={[black]SSv2-3DR50,[black]SSv2-3DR18,[black]D48-3DR50,[black]D48-3DR18},
        legend to name=bias_eval_legend,
    ]
    % ssv2
    % R50
    \addplot[only marks,mark size=4pt,color=magenta,mark=triangle*,]
    coordinates {(None,42.486) (Normal,41.220) (SD0.1,35.748) (SD0.3,31.851) (SD0.5,30.389) (SD0.7,30.635)};
        
    % R18
    \addplot[only marks,mark size=3.2pt,color=cyan,mark=*,]
        coordinates {(None,40.113) (Normal,37.138) (SD0.1,35.407) (SD0.3,34.510) (SD0.5,32.837) (SD0.7,31.404)};
        
       % d48 
    % R50
    \addplot[only marks,mark size=4pt,color=magenta,mark=triangle,]
    coordinates {(None,63.323) (Normal,66.849) (SD0.1,47.576) (SD0.3,44.987) (SD0.5,43.433) (SD0.7,42.193)};
        
    % R18
    \addplot[only marks,mark size=3.2pt,color=cyan,mark=o,]
        coordinates {(None,61.391) (Normal,63.591) (SD0.1,47.413) (SD0.3,46.258) (SD0.5,44.479) (SD0.7,41.466)};
        
    % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
	   % coordinates {([normalized]-10,0)([normalized]10,0)};
    \end{axis}
\end{tikzpicture}
\hspace{0.1cm}
	\begin{tikzpicture} %\ref{dim_ss_legend}
    \begin{axis}[
       line width=1.0,
        title={Dyn/Static Dim.},
        title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
        xlabel={Dropout Type},
        % x label style={font=\small},
        ylabel={Fraction of Dyn Dims (\%)},
        % xmin=0, xmax=550,
        ymin=-5, ymax=103,
        % xtick={50,100,200,300,400,500},
        ytick={0,10,20,30,40,50,60,70,80,90,100},
        symbolic x coords={None, Normal, SD0.1,SD0.3, SD0.5, SD0.7},
        xtick=data,
        x tick label style={font=\footnotesize,rotate=25,anchor=east},
        % x tick label style={font=\footnotesize,rotate=20,anchor=east},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
        y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
        xtick pos=left,
        ytick pos=bottom,
        width=6.7cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
         %draw=none,
         nodes={scale=0.9, transform shape},
         cells={anchor=west},
         legend style={at={(1.4,0.25)},anchor=south}, font =\footnotesize},
         %legend columns=1,
         legend entries={[black]3DResNet50,[black]3DResNet18},
        legend to name=dim_ss_legend,
    ]
    
    % SSV2
    % R50
    \addplot[only marks,mark size=4pt,color=magenta,mark=triangle*,]
    coordinates {(None,39.28571429) (Normal,61.047463180) (SD0.1,76.7) (SD0.3,81.0) (SD0.5,90.7) (SD0.7,89.2)};
        
    % R18
    \addplot[only marks,mark size=3.2pt,color=cyan,mark=*,]
        coordinates {(None,31.80987203) (Normal,60.9671848) (SD0.1,64.8) (SD0.3,79.7) (SD0.5,88.8) (SD0.7,93.6)};
    
    % D48
    % R50
    \addplot[only marks,mark size=4pt,color=magenta,mark=triangle,]
    coordinates {(None,4.085872576) (Normal,10.64204046) (SD0.1,9.0) (SD0.3,11.9) (SD0.5,29.9) (SD0.7,42.3)};
    % r18
    \addplot[only marks,mark size=3.2pt,color=cyan,mark=o,]
        coordinates {(None,0.05733944954) (Normal,0.7343941248) (SD0.1,0.3) (SD0.3,1.8) (SD0.5,5.0) (SD0.7,4.4)};
        
    % \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
	   % coordinates {([normalized]-10,0)([normalized]10,0)};
    \end{axis}
\end{tikzpicture}}
\end{center}
\vspace{-0.5cm}
\caption{StaticDropout influences the static and dynamic information of a model. We evaluate the relative performance of a model evaluate on normal \vs shuffled frames at validation time (left) and show the fraction of channels encoding dynamic information relative to the channels encoding either static or dynamic (right). Larger StaticDropout rates generally result in less bias toward static information.}
\label{fig:static_dropout_bias1}
\vspace{-0.7cm}
\end{figure}


\textbf{Results.} Figure~\ref{fig:static_dropout_bias1} shows the debiasing results for models trained on Diving48 and SSv2. StaticDropout is successful in debiasing the model away from static and toward dynamic information. In terms of our metric, (\ref{eq:ind_bias_scores_diff_b}), both the models see a significant jump in the ratio of dynamic to static units on SSv2 and Diving48 (Fig.~\ref{fig:static_dropout_bias1} right). 
% On SSv2, both models see this ratio increase from between 30\%-40\% to above 90\%, while on Diving48, the effect is consistent but less pronounced for the ResNet18 model. 
The debiasing also has a strong effect in reducing the models' ability to classify shuffled video frames compared with the standard or no-dropout baselines (Fig.~\ref{fig:static_dropout_bias1} left). 
% For example, on normal \vs shuffled frames for the Diving48 dataset, 3D-ResNet50 achieves 71.2\% \vs 47.6\%, while our static dropout with $r=0.7$ achieves 71.2\% \vs 30.1\%. 
% Similar findings with respect to shuffled frame performance are seen on SSv2. 
These results suggest that StaticDropout has a strong influence on the types of specialized units contained in the model and also the model's bias toward encoding dynamic and static information. Notably, the effect of StaticDropout on the model bias is consistently \textit{dose-dependant}, meaning the biases are tunable via the dropout rate, $r$.

We evaluate the performance of models trained with StaticDropout on the SSv2~\cite{goyal2017something}, as it requires the maximal amount of dynamics compared with other datasets (see Sec~\ref{sec:ar_dataset}). We also evaluate on the SomethingElse~\cite{materzynska2020something} dataset, an `object debiased' relabelled version of SSv2 where the set of objects (\ie ``somethings'') appearing in the training set for a specific action is disjoint from the set of objects appearing in the validation set for the same action (see\cite{materzynska2020something} for additional details). 
% The goal of this relabelling is to remove any object bias from the training and validation distributions~\cite{materzynska2020something}.
We experiment on the SomethingElse compositional split with the intuition that our StaticDropout technique may debias the model from focusing on object appearances and more generally toward longer range motions contained in the videos. The results for both dataset splits are shown in Fig.~\ref{fig:AR_infodrop_somethingelse} (top) in terms of Top-1 accuracy and percentage of dynamic units in the model's final layer. StaticDropout outperforms both the baselines in terms of accuracy, and significantly increases the number of dynamic units. However, a dropout rate of $r=0.7$ does not achieve the best performance, suggesting that simply maximizing the number of dynamic units is not optimal, and that a balance of dynamics and statics should be learned.
Figure~\ref{fig:AR_infodrop_somethingelse} (bottom) shows the average performance difference between a 3D-ResNet50 trained with StaticDropout compared with standard dropout on the top-\textit{k} most and least common classes. Interestingly, on average, our model significantly outperforms the baseline on the rarest classes in the dataset while slightly under-performing the baseline on the most common classes. This result suggests that our regularization specifically targets classes in the tail end of the data distribution.
% We also show qualitative examples of attention heatmaps using GradCAM~\cite{selvaraju2017grad} in Fig.~\ref{fig:static_dropout_gradcam} which compares the baseline dropout to our StaticDropout with $r=0.1$ trained on SomethingElse. The baseline model incorrectly classifies actions involving objects which are used in multiple other actions, such as paper. The CAMs generated from our model are focused on regions pertaining to the correct action class over more time steps (\eg at the location of the tearing before and after the tearing occurs).




\begin{figure} [t]
 \def\arraystretch{1.35}
 \setlength\tabcolsep{2.4pt}
\centering
\resizebox{0.4\textwidth}{!}{
	\begin{tabu}{c cccc}
\tabucline[1pt]{-}
 \multirow{2}{*}{Dropout}&  \multicolumn{2}{c}{\textbf{SSv2~\cite{goyal2017something}}} & \multicolumn{2}{c}{\textbf{SomethingElse~\cite{materzynska2020something}}}    \\
\cline{2-5}
  & Top-1 (\%) & Dyn. Units (\%) & Top-1 (\%) &  Dyn. Units (\%) \\
\tabucline[1pt]{-}
        None & 54.18 & 10.7 & 49.43  & 4.6 \\
        Normal & 54.55 & 18.2 & 49.79 &  17.5\\
        \hline
        StaticDropout  ($r$=0.1) & \textbf{55.19} & 56.9  & 50.38 &  34.2 \\
        StaticDropout ($r$=0.3) & 54.55 & 53.6  & \textbf{51.16} &  45.1 \\
        StaticDropout ($r$=0.5) & 54.01 & \textbf{80.0}  & 50.06 &  \textbf{51.4} \\
        % StaticDropout ($r$=0.7) &  &  & 50.93  & 45.1  \\
	  % \hline
	\tabucline[1pt]{-}
	\end{tabu}}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 % 0.3
\vfill
\resizebox{0.49\textwidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            ybar,
            height=3.6cm,
            width=8cm,
            % enlargelimits=0.15,
            legend style={at={(0.5,-0.15)},
              anchor=north,legend columns=-1},
            ylabel={Ave. Acc. Diff. (\%)},
            xmin=0, xmax=55,
            ymin=-11, ymax=11,
            xtick={5,10,15,20,25,30,35,40,45,50},
            xlabel={Top-$k$ \textbf{least} common classes},
            x tick label style={font=\small},
            y tick label style={font=\small},
            x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
            y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
            nodes near coords,
            every node near coord/.append style={font=\scriptsize},
            nodes near coords align={vertical},
            extra y ticks = 0.0,
            extra y tick labels={},
            extra y tick style={grid=major,major grid style={draw=black}}
            ]
        \addplot[blue,fill=blue] coordinates {(5,1.1) (10,2.2) (15,4.1) (20,4.5) (25,4.8) (30,4.5) (35,4.6) (40,4.8) (45,4.7) (50,4.4)};

        \end{axis}
        \end{tikzpicture}
        \begin{tikzpicture}
        \begin{axis}[
            ybar,
            height=3.6cm,
            width=8cm,
            % enlargelimits=0.15,
            legend style={at={(0.5,-0.15)},
              anchor=north,legend columns=-1},
            % ylabel={Ave. Ac c. Diff. (\%)},
            xmin=0, xmax=55,
            ymin=-11, ymax=11,
            xtick={5,10,15,20,25,30,35,40,45,50},
            xlabel={Top-$k$ \textbf{most} common classes},
            x tick label style={font=\small},
            y tick label style={font=\small},
            yticklabel pos=right,
            x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
            y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\small},
            nodes near coords,
            every node near coord/.append style={font=\scriptsize},
            nodes near coords align={vertical},
            extra y ticks = 0.0,
            extra y tick labels={},
            extra y tick style={grid=major,major grid style={draw=black}}
            ]
        \addplot[red,fill=red] coordinates {(5,-1.1) (10,-0.7) (15,-1.2) (20,-1.3) (25,-1.0) (30,-0.9) (35,-0.5) (40,-0.3) (45,-0.2) (50,-0.3)};
        \end{axis}
        \end{tikzpicture}}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
 % 0.3

    
% \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             height=3.6cm,
%             width=8cm,
%             % enlargelimits=0.15,
%             legend style={at={(0.5,-0.15)},
%               anchor=north,legend columns=-1},
%             ylabel={Ave. Acc. Diff. (\%)},
%             xmin=0, xmax=55,
%             ymin=-11, ymax=11,
%             xtick={5,10,15,20,25,30,35,40,45,50},
%             xlabel={Top-$k$ \textbf{least} common classes},
%             x tick label style={font=\small},
%             y tick label style={font=\small},
%             x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
%             y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%             nodes near coords,
%             every node near coord/.append style={font=\scriptsize},
%             nodes near coords align={vertical},
%             extra y ticks = 0.0,
%             extra y tick labels={},
%             extra y tick style={grid=major,major grid style={draw=black}}
%             ]
%         \addplot[blue,fill=blue] coordinates {(5,1.9) (10,4.9) (15,6.2) (20,6.5) (25,7.4) (30,6.2) (35,5.6) (40,5.9) (45,5.8) (50,5.6)};
%         % \legend{used,understood,not understood}
%         \end{axis}
%         \end{tikzpicture}
%         \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             height=3.6cm,
%             width=8cm,
%             % enlargelimits=0.15,
%             legend style={at={(0.5,-0.15)},
%               anchor=north,legend columns=-1},
%             % ylabel={Ave. Ac c. Diff. (\%)},
%             xmin=0, xmax=55,
%             ymin=-11, ymax=11,
%             xtick={5,10,15,20,25,30,35,40,45,50},
%             xlabel={Top-$k$ \textbf{most} common classes},
%             x tick label style={font=\small},
%             y tick label style={font=\small},
%             yticklabel pos=right,
%             x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
%             y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\small},
%             nodes near coords,
%             every node near coord/.append style={font=\scriptsize},
%             nodes near coords align={vertical},
%             extra y ticks = 0.0,
%             extra y tick labels={},
%             extra y tick style={grid=major,major grid style={draw=black}}
%             ]
%         \addplot[red,fill=red] coordinates {(5,-2.3) (10,-1.9) (15,-1.7) (20,-2.1) (25,-1.9) (30,-1.7) (35,-1.4) (40,-1.1) (45,-0.9) (50,-0.9)};
%         % \legend{used,understood,not understood}
%         \end{axis}
%         \end{tikzpicture}
        
        \vspace{-0.35cm}
\caption{\textbf{Top:} StaticDropout results for 3D-ResNet50 trained on SSv2 and SomethingElse~\cite{materzynska2020something}. 
\textbf{Bottom:} Average performance difference between StaticDropout ($r=0.3$) and baseline dropout of a 3D-ResNet50 for the top-$k$ most and least common classes in the SomethingElse~\cite{materzynska2020something} compositional split. StaticDropout performs better on rare classes, while performing marginally worse on common classes. 
}\label{fig:AR_infodrop_somethingelse}
\vspace{-0.55cm}
\end{figure}







% \begin{figure}
%     \centering
% \resizebox{0.49\textwidth}{!}{
%         \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             height=3.6cm,
%             width=8cm,
%             % enlargelimits=0.15,
%             legend style={at={(0.5,-0.15)},
%               anchor=north,legend columns=-1},
%             ylabel={Ave. Acc. Diff. (\%)},
%             xmin=0, xmax=55,
%             ymin=-11, ymax=11,
%             xtick={5,10,15,20,25,30,35,40,45,50},
%             xlabel={Top-$k$ \textbf{least} common classes},
%             x tick label style={font=\small},
%             y tick label style={font=\small},
%             x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
%             y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%             nodes near coords,
%             every node near coord/.append style={font=\scriptsize},
%             nodes near coords align={vertical},
%             extra y ticks = 0.0,
%             extra y tick labels={},
%             extra y tick style={grid=major,major grid style={draw=black}}
%             ]
%         \addplot[blue,fill=blue] coordinates {(5,1.9) (10,4.9) (15,6.2) (20,6.5) (25,7.4) (30,6.2) (35,5.6) (40,5.9) (45,5.8) (50,5.6)};
%         % \legend{used,understood,not understood}
%         \end{axis}
%         \end{tikzpicture}
%         \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             height=3.6cm,
%             width=8cm,
%             % enlargelimits=0.15,
%             legend style={at={(0.5,-0.15)},
%               anchor=north,legend columns=-1},
%             % ylabel={Ave. Ac c. Diff. (\%)},
%             xmin=0, xmax=55,
%             ymin=-11, ymax=11,
%             xtick={5,10,15,20,25,30,35,40,45,50},
%             xlabel={Top-$k$ \textbf{most} common classes},
%             x tick label style={font=\small},
%             y tick label style={font=\small},
%             yticklabel pos=right,
%             x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\large},
%             y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\small},
%             nodes near coords,
%             every node near coord/.append style={font=\scriptsize},
%             nodes near coords align={vertical},
%             extra y ticks = 0.0,
%             extra y tick labels={},
%             extra y tick style={grid=major,major grid style={draw=black}}
%             ]
%         \addplot[red,fill=red] coordinates {(5,-2.3) (10,-1.9) (15,-1.7) (20,-2.1) (25,-1.9) (30,-1.7) (35,-1.4) (40,-1.1) (45,-0.9) (50,-0.9)};
%         % \legend{used,understood,not understood}
%         \end{axis}
%         \end{tikzpicture}
%         }
%         % \put(-200,100){{\small \rotatebox{90}{Average Top-1 Acc Difference (\%)}}}
%     \caption{The average performance difference between StaticDropout ($r=0.1$) and baseline dropout of a 3D-ResNet50 for the top-$k$ most common and least common classes in the SomethingElse~\cite{materzynska2020something} compositional split. On average, StaticDropout performs better on rare classes while performs marginally worse on the most common classes.}
%     \label{fig:se_per_class_perf}
% \end{figure}








%%% GRADCAM FIGURE!
% \begin{figure}
%   \begin{center}
% 		\resizebox{0.49\textwidth}{!}{
% 		\def\arraystretch{0.3}
%         \setlength\tabcolsep{0.5pt}
% 		\begin{tabular}{{cccccc}}	
%       \rotatebox{90}{{\Large Baseline}} \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/30_tear_into_2_pieces/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/30_tear_into_2_pieces/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/30_tear_into_2_pieces/frame_2.jpeg} &
%       \hspace{0.1cm}
%       \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/174_moving_towards_camera/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/174_moving_towards_camera/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/174_moving_towards_camera/frame_2.jpeg} \\
      
%     %   \hspace{0.1cm}
%     %   \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/33_tear_into_two_pieces/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/33_tear_into_two_pieces/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/33_tear_into_two_pieces/frame_2.jpeg} \\
%     %   \vspace{0.1cm}
%       \rotatebox{90}{{\Large StaticDropout}} \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/30/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/30/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/30/frame_2.jpeg} &  
%       \hspace{0.1cm}
%     %   \vspace{0.15cm}

%     %   \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/33/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/33/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/33/frame_2.jpeg} \\
%     %   \put(30,20){{\large Top: \textcolor{red}{Tearing Something into Two Pieces}}}
%     %   \put(40,5){{\large Bottom: \textcolor{green}{Tearing Something a Little Bit}}}
%     %   \put(400,400){{\large Top: \textcolor{red}{asdfghjklasdfgjkl}}}
%     %   \put(400,500){{\large Bottom: \textcolor{green}{asdfghjklasdfgjkl}}} 
%     %   \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/37_falling_like_paper/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/37_falling_like_paper/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/slow_else_baseline/37_falling_like_paper/frame_2.jpeg} & 
%     %   \hspace{0.1cm}
      
%     %   \vspace{0.1cm}
%     %   \rotatebox{90}{{\large StaticDropout}}
%     % \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/37/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/37/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/37/frame_2.jpeg} &   
%     %   \hspace{0.1cm}
%       \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/174/frame_0.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/174/frame_1.jpeg} & \includegraphics[width=0.2\textwidth]{images/gradcam/staticdropout/174/frame_2.jpeg} \\
%     %   \put(30,20){{\large Top: \textcolor{red}{Tearing Something into Two Pieces}}}
%     %   \put(40,5){{\large Bottom: \textcolor{green}{Tearing Something a Little Bit}}}
%     %   \put(200,20){{\large Top: \textcolor{red}{Tearing Something into Two Pieces}}}
%     %   \put(200,5){{\large Bottom: \textcolor{green}{Tearing Something a Little Bit}}}
      
%     \end{tabular}
%     }
%     \end{center}
%     \vspace{-0.4cm}
%     \caption{GradCAM visualizations of the baseline (BL) 3D-ResNet50 vs our proposed StaticDropout (SD) technique on the SomethingElse~\cite{materzynska2020something} compositional validation split. The baseline model commonly makes mistakes on objects which are used in multiple actions (\eg paper). Predictions (\textcolor{red}{incorrect}/\textcolor{green}{correct}) are: Left-BL: \textcolor{red}{Tearing something into two pieces}, Left-SD: \textcolor{green}{Tearing something a little bit}. Right-BL: \textcolor{red}{Moving something toward the camera}, Right-SD: \textcolor{green}{Bending something so that it deforms}.}
%     \label{fig:static_dropout_gradcam}
% \end{figure}


\vspace{-0.4cm}
\subsection{Fusion and Cross Connection Study}\label{sec:vos_cc_study}
\vspace{-0.1cm}
Our goal in this final section is to encourage a previously static biased AVOS model (\ie RTNet) to have more dynamic units. Based on our analysis in Sections~\ref{sec:ar_models} and~\ref{sec:vos_datasets}, we hypothesize that the reason behind AVOS models being static biased stems from the sub-optimal application of bidirectional cross connections.
% or their pre-training protocol on saliency segmentation datasets (DUTS). 
Toward this goal, we conduct a detailed analysis of the fusion and cross connection types in the aforementioned architectures and evaluate how they affect biases and model accuracy.

%1- Explain different cross connection and fusion types
%2- Explain the two new models
%3- Dimensionality estimation
%4- MoCA evaluation

%TODOs:
%======
%1- Dim Est. of 2 new models on four fusion layers.
%2- MoCA evaluation without flipping and using thresh=0.2
%3- 

% \begin{figure*}[t]
% \begin{minipage}{0.4\textwidth}
% \resizebox{1.0\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 5},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(37.5244140625,G+U) (0.0,RTNet) (44.2,CCG+U) (33.0,G+B)};
% \addplot coordinates {(44.62890625,G+U) (1.171875,RTNet) (44.6,CCG+U) (47.1,G+B)};
% \addplot coordinates {(17.8466796875,G+U) (98.828125,RTNet) (11.2,CCG+U) (20.0,G+B)};
% \addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (0.0,G+B)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \hfill
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 4},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(33.7890625,G+U) (0.0,RTNet)(36.6,CCG+U) (16.9,G+B)};
% \addplot coordinates {(37.40234375,G+U) (65.6,RTNet)(37.9,CCG+U) (53.4,G+B)};
% \addplot coordinates {(28.80859375,G+U) (34.4,RTNet)(25.5,CCG+U) (25.6,G+B)};
% \addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (4.1,G+B)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{1.0\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 3},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(33.69140625,G+U) (3.9,RTNet)(37.9,CCG+U) (31.1,G+B)};
% \addplot coordinates {(46.6796875,G+U) (64.1,RTNet)(43.9,CCG+U) (45.1,G+B)};
% \addplot coordinates {(19.62890625,G+U) (26.6,RTNet)(18.2,CCG+U) (23.8,G+B)};
% \addplot coordinates {(0.0,G+U) (5.5,RTNet)(0.0,CCG+U) (0.0,G+B)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 2},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(29.8828125,G+U) (6.3,RTNet)(34.2,CCG+U) (30.3,G+B)};
% \addplot coordinates {(46.2890625,G+U) (59.4,RTNet)(44.3,CCG+U) (43.8,G+B)};
% \addplot coordinates {(23.828125,G+U) (21.9,RTNet)(21.5,CCG+U) (26.0,G+B)};
% \addplot coordinates {(0.0,G+U) (12.5,RTNet)(0.0,CCG+U) (0.0,G+B)};
% % \legend {Dynamic,Static,Joint,Residual};
% \end{axis}
% \end{tikzpicture}}
% \end{minipage}
% \begin{minipage}{0.6\textwidth}
%     \centering \resizebox{1.0\textwidth}{!}{
% \begin{tabu}{@{}lcccccccccc}
% \tabucline[1pt]{-}
% \multirow{2}{*}{Method} & Fusion & CC & Flip &\multirow{2}{*}{mIoU} & \multicolumn{6}{c}{Success Rate} \\ \cmidrule(r{2pt}){6-11}
% &   & & &  & $\tau=0.5$ & $\tau=0.6$ & $\tau=0.7$& $\tau=0.8$ &  $\tau=0.9$ &  $SR_{\text{Mean}}$\\ \tabucline[1pt]{-}
% FusionSeg~\cite{jain2017fusionseg} & - & - & \xmark & 42.3 & 47.9 & 43.6 & 35.9 & 24.2 & 9.4 & 39.2\\
% RTNet~\cite{ren2021reciprocal} & CCG & B & \xmark & 60.7 & 67.9 & 62.4 & 53.6 & 43.4 & 23.9 & 50.2 \\ 
% MATNet~\cite{zhou2020motion} & G & U & \cmark & 64.2 & 71.2 & 67.0 & 59.9 & \textbf{49.2} & 24.6 & 54.4 \\\hline
% MATNet* & G & U & \xmark & \textbf{67.3} & \textbf{75.9} & \textbf{70.8} & \textbf{61.9} & 48.6 & \textbf{26.0} & \textbf{56.6}\\
% %MATNet NoBAR & G & U & \xmark& 65.1 & 73.6 & 68.0 & 58.9 & 44.7 & 21.5 &  53.3\\
% %MATNet NoYTB & G & U & \xmark& 54.7 & 59.9 & 53.5 & 44.0 & 31.0 & 13.4 & 40.3 \\ \hline
% MATNet* & CCG & U & \xmark& 64.4 & 73.8 & 68.1 & 57.1 & 41.7 & 18.1 & 51.8 \\
% RTNet* & G & B & \xmark & 70.3 & 81.5 & 75.2  & 64.5 & 47.1 & 22.2 &  58.1\\\hline
% MATNet* & G & U & \cmark & 68.5 & 77.3 & 72.2 & 63.5 & 50.6 &27.0 & 58.1 \\
% RTNet* & G & B & \cmark & \textbf{70.6} &81.2 &75.5 &65.0 &48.1 &23.0 & \textbf{58.6}\\ \hline
% \tabucline[1pt]{-}
% \end{tabu}}
% \end{minipage}
%     \caption{\textbf{Left:} Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (3), $\lambda=0.5$ at different fusion layers of RTNet. \textbf{Right:} Evaluation of AVOS models on MoCA~\cite{lamdouar2020betrayed} using varied IoU threshold success rates, $\tau$. 
%     * means networks implemented by us (see Sec.~\ref{sec:vos_archs}).
%     % The MATNet* variants are trained by us, while MATNet~\cite{zhou2020motion} is the original model. RTNet~\cite{ren2021reciprocal} is the off-the-shelf model and RTNet* is our version that aligns with the MATNet* backbone and training scheme. 
%     We compare cross connections: unidirectional motion-to-appearance (U) \vs bidirectional (B), and fusion types: gated (G) \vs convex combination gated (CCG). Flip means performing data augmentation with flipping during inference as originally done in~\cite{zhou2020motion}.}
%     \label{fig:moca_vs_davis_and_ind}
% \end{figure*}



\begin{figure}[t]
\begin{minipage}{0.45\textwidth}
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=3.7cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 5},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
    symbolic y coords={G+U, CCG+U, G+B, RTNet},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]

\addplot coordinates {(37.5244140625,G+U) (0.0,RTNet) (44.2,CCG+U) (33.0,G+B)};
\addplot coordinates {(44.62890625,G+U) (1.171875,RTNet) (44.6,CCG+U) (47.1,G+B)};
\addplot coordinates {(17.8466796875,G+U) (98.828125,RTNet) (11.2,CCG+U) (20.0,G+B)};
\addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (0.0,G+B)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture} 
\hfill
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=3.7cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 4},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={G+U, CCG+U, G+B, RTNet},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]

\addplot coordinates {(33.7890625,G+U) (0.0,RTNet)(36.6,CCG+U) (16.9,G+B)};
\addplot coordinates {(37.40234375,G+U) (65.6,RTNet)(37.9,CCG+U) (53.4,G+B)};
\addplot coordinates {(28.80859375,G+U) (34.4,RTNet)(25.5,CCG+U) (25.6,G+B)};
\addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (4.1,G+B)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\vfill
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=3.7cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 3},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    xlabel style = {font=\large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={G+U, CCG+U, G+B, RTNet},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]
\addplot coordinates {(33.69140625,G+U) (3.9,RTNet)(37.9,CCG+U) (31.1,G+B)};
\addplot coordinates {(46.6796875,G+U) (64.1,RTNet)(43.9,CCG+U) (45.1,G+B)};
\addplot coordinates {(19.62890625,G+U) (26.6,RTNet)(18.2,CCG+U) (23.8,G+B)};
\addplot coordinates {(0.0,G+U) (5.5,RTNet)(0.0,CCG+U) (0.0,G+B)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis} [xbar stacked,
     width=\axisdefaultwidth,
    height=3.7cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 2},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    xlabel style = {font=\large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={G+U, CCG+U, G+B, RTNet},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]
\addplot coordinates {(29.8828125,G+U) (6.3,RTNet)(34.2,CCG+U) (30.3,G+B)};
\addplot coordinates {(46.2890625,G+U) (59.4,RTNet)(44.3,CCG+U) (43.8,G+B)};
\addplot coordinates {(23.828125,G+U) (21.9,RTNet)(21.5,CCG+U) (26.0,G+B)};
\addplot coordinates {(0.0,G+U) (12.5,RTNet)(0.0,CCG+U) (0.0,G+B)};
% \legend {Dynamic,Static,Joint,Residual};
\end{axis}
\end{tikzpicture}}
\centering \resizebox{0.8\textwidth}{!}{
\begin{tabu}{@{}lccccc}
\tabucline[1pt]{-}
Method & Fusion & CC & Flip &mIoU & $SR_{\text{Mean}}$ \\ \tabucline[1pt]{-}
FusionSeg~\cite{jain2017fusionseg} & - & - & \xmark & 42.3 & 39.2\\
RTNet~\cite{ren2021reciprocal} & CCG & B & \xmark & 60.7 & 50.2 \\ 
MATNet~\cite{zhou2020motion} & G & U & \cmark & 64.2  & 54.4 \\\hline
MATNet* & G & U & \xmark & 67.3 & 56.6\\
MATNet* & CCG & U & \xmark& 64.4 & 51.8 \\
RTNet* & G & B & \xmark & \textbf{70.3} &  \textbf{58.1}\\\hline
MATNet* & G & U & \cmark & 68.5  & 58.1 \\
RTNet* & G & B & \cmark & \textbf{70.6} & \textbf{58.6}\\ \hline
\tabucline[1pt]{-}
\end{tabu}}
\end{minipage}
\vspace{-0.2cm}
    \caption{\textbf{Top:} Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (3), $\lambda=0.5$ at different fusion layers of RTNet. \textbf{Bottom:} Evaluation of AVOS models on MoCA~\cite{lamdouar2020betrayed}. 
    * means networks implemented by us (see Sec.~\ref{sec:vos_archs}).
    We compare cross connections: unidirectional motion-to-appearance (U) \vs bidirectional (B), and fusion types: gated (G) \vs convex combination gated (CCG). Flip means performing data augmentation with flipping during inference, as originally done in~\cite{zhou2020motion}.}
    \label{fig:moca_vs_davis_and_ind}
    \vspace{-0.6cm}
\end{figure}



\noindent \textbf{Approach.} We now analyze the different types of \textit{fusion} and \textit{cross connections}. Cross connections can operate \textit{Bidirectionally} (\ie motion-to-appearance and appearance-to-motion), as in RTNet, or \textit{Uni-directionally} with motion-to-appearance cross connection, as in MATNet. The \textit{Convex Combination Gated Fusion} in RTNet enforces the attention weights to sum to one for both motion and appearance streams. While the \textit{Gated Fusion} in MATNet learns to weight each stream without this constraint. Both mechanisms can be decomposed into channel attention followed by spatial attention. For the sake of unification we pose the channel attention in the \textit{Convex Combination Gated Fusion} as,
% \begin{subequations}
% \begin{equation}
%     A_c = \mathcal{F}_e(\mathcal{F}_s(U_a \oplus U_m)),
% \end{equation}
% \begin{equation}
%     Z_a = A_c \circ U_a,
% \end{equation}
% \begin{equation}
%     Z_m = (1-A_c) \circ U_m,
% \end{equation}
% \end{subequations}
\begin{subequations}
\begin{gather}
    A_c = \mathcal{F}_e(\mathcal{F}_s(U_a \oplus U_m)),  \quad   Z_a = A_c \circ U_a,  \tag{\theequation a,b} \\
 Z_m = (1-A_c) \circ U_m, \tag{\theequation c}
\end{gather}
\end{subequations}
where $U_a, U_m$ are the appearance and motion features, respectively, $\circ$ is the Hadamard product, $\oplus$ denotes concatenation, $\mathcal{F}_s$ and $\mathcal{F}_e$ are the squeeze and excitation operators, respectively, and $A_c \in \mathbb{R}^c$ are the channel attention weights where $c$ is the number of channels for the input appearance or motion feature maps. A weighted combination is used to attend to motion and appearance features, enforcing a strong constraint on the attention weights during training. On the other hand, the channel attention module in the \textit{Gated Fusion} can be given as
\vspace{-0.1cm}
\begin{subequations}
\begin{gather}
U = U_a \oplus U_m,  \quad  A_c = \mathcal{F}_e(\mathcal{F}_s(U)),   \quad   Z = A_c \circ U, \tag{\theequation a-c} 
\end{gather}
\end{subequations}
\vspace{-0.1cm}
where $A_c \in \mathbb{R}^{2c}$ is the channel-wise attention on the combined motion and appearance features without enforcing them to to sum to one, unlike in RTNet.

In contrast, the spatial attention in \textit{Convex Combination Gated Fusion} can be given as
\vspace{-0.1cm}
\begin{equation} 
Z = A_{sp} \circ Z_a \oplus (1-A_{sp}) \circ Z_m,
\end{equation}
\vspace{-0.1cm}
where $A_{sp}$ is the spatial attention maps generated from a convolutional layer and a sigmoid function, while $Z_a$ and $Z_m$ are the average pooled appearance and motion features. Finally, the spatial attention in \textit{Gated Fusion} can be given as
\vspace{-0.1cm}
\begin{equation}
 Z = A_{sp} \circ Z + Z,
\end{equation}
\vspace{-0.1cm}
\noindent where $Z$ is the combined motion and appearance features. Again, it is clear that the spatial attention module in the \textit{Convex Combination Gated Fusion} restricts the attention weights between both motion and appearance features, unlike the \textit{Gated Fusion}. Therefore we hypothesis that \textit{Gated Fusion} will yield better results for tasks requiring a complex interaction between motion and appearance features. We now ablate the fusion types along with the two different types of cross connections on such a task.

\noindent \textbf{Evaluation protocol.} We show the static and dynamic biases for the different fusion and cross connections, and evaluate accuracy on a dataset which requires dynamics (MoCA). We follow previous work by removing videos that contain no predominant target locomotion, which produces a subset of 88 videos for evaluation~\cite{yang2021selfsupervised}. We evaluate using mean intersection over union and success rate mean with varying IoU thresholds ranging from 0.5 to 0.9. The original MATNet used horizontal flipping during the inference and averaged predictions from the original and flipped versions. To ensure fair comparison between RTNet and FusionSeg we show results with and without the flipping augmentation during inference when reporting on MoCA.

\noindent\textbf{Results.}
Figure~\ref{fig:moca_vs_davis_and_ind} (top) shows the static and dynamic biases of the different fusion and cross connection types. It is seen that the bidirectional cross connections (G+B) incur a small decrease in the dynamic bias with respect to unidirectional ones (G+U), especially on the final fusion layers (\ie fusion 4 and 5). The convex combination gated fusion (CCG+U) leads to a decrease in the ratio of joint to dynamic units with respect to gated fusion (G+U) (\eg the final fusion layer for CCG+U Joint/Dynamic is 25.3 \vs 47.5 for G+U). The performance of all models on the MoCA dataset is shown in Fig.~\ref{fig:moca_vs_davis_and_ind} (bottom). The original MATNet and MATNet* both outperform the off-the-shelf RTNet model and FusionSeg, which is confirmation of our previous findings that both models are heavily static biased (see Fig.~\ref{fig:stagewise_vos}). Additionally, it demonstrates that our proposed model (RTNet*) with bidirectional cross connections and Gated Fusion (B+G) trained on YouTube-VOS and DAVIS shows sizable ($+9.9\%$) gain with respect to off-the-shelf RTNet. We also observe from the results of MATNet* (G+U) \vs MATNet* (CCG+U) that the added constraint of convex combination can degrade the performance with respect to gated fusion on a dynamically heavy task (\ie MoCA).

Motivated by the previous experiments. which showed the impact of static and dynamic biases on performance (Sec.~\ref{sec:neuron_removal}), these results demonstrate how simply selecting the appropriate combination of fusion and cross connection mechanisms can significantly impact what is encoded in models as well as the downstream performance.

% \begin{figure}[t]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 5},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(37.5244140625,G+U) (0.0,RTNet) (44.2,CCG+U) (33.0,G+B)};
% \addplot coordinates {(44.62890625,G+U) (1.171875,RTNet) (44.6,CCG+U) (47.1,G+B)};
% \addplot coordinates {(17.8466796875,G+U) (98.828125,RTNet) (11.2,CCG+U) (20.0,G+B)};
% \addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (0.0,G+B)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \hfill
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 4},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(33.7890625,G+U) (0.0,RTNet)(36.6,CCG+U) (16.9,G+B)};
% \addplot coordinates {(37.40234375,G+U) (65.6,RTNet)(37.9,CCG+U) (53.4,G+B)};
% \addplot coordinates {(28.80859375,G+U) (34.4,RTNet)(25.5,CCG+U) (25.6,G+B)};
% \addplot coordinates {(0.0,G+U) (0.0,RTNet)(0.0,CCG+U) (4.1,G+B)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 3},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(33.69140625,G+U) (3.9,RTNet)(37.9,CCG+U) (31.1,G+B)};
% \addplot coordinates {(46.6796875,G+U) (64.1,RTNet)(43.9,CCG+U) (45.1,G+B)};
% \addplot coordinates {(19.62890625,G+U) (26.6,RTNet)(18.2,CCG+U) (23.8,G+B)};
% \addplot coordinates {(0.0,G+U) (5.5,RTNet)(0.0,CCG+U) (0.0,G+B)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=3.7cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 2},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={G+U, CCG+U, G+B, RTNet},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(29.8828125,G+U) (6.3,RTNet)(34.2,CCG+U) (30.3,G+B)};
% \addplot coordinates {(46.2890625,G+U) (59.4,RTNet)(44.3,CCG+U) (43.8,G+B)};
% \addplot coordinates {(23.828125,G+U) (21.9,RTNet)(21.5,CCG+U) (26.0,G+B)};
% \addplot coordinates {(0.0,G+U) (12.5,RTNet)(0.0,CCG+U) (0.0,G+B)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (3), $\lambda=0.5$ at different fusion layers. We compare the different cross connections: unidirectional motion-to-appearance (U) \vs bidirectional (B), along with different fusion types: gated (G) \vs convex combination gated (CCG) and compare to the biases of RTNet off-the-shelf model.}
% \label{fig:vos_alllayers_cc}
% \end{figure}

==> core/conc.tex <==
% In this paper we proposed a generic framework for estimating the static and dynamic biases in deep spatiotemporal models. We first produced video pairs by disentangled the static and dynamic information by means of video stylization and frame shuffling. Using these video pairs, we then measured the static and dynamic information contained in the intermediate representations of any deep spatiotemporal model. We then performed a detail analysis on two tasks, action recognition and video object segmentation, to answer the question ``what effect do model architectures and training datasets have on static and dynamic biases?''. 

% Our study of numerous state-of-the-art models and datasets revealed multiple shared insights. We confirmed the belief that most models are biased towards encoding static information. We demonstrated the efficacy of motion-to-appearance cross connections in two-stream models to transfer dynamic information. By studying models on a per-unit level, we showed that dynamic biased models produce dynamic-specific units, contrary to the static and joint units found in static-biased models. 

% We then focused on evaluating the most common training datasets for the two tasks. We demonstrated that datasets have a significant impact on a models static and dynamic biases, and moreover, that datasets commonly used to evaluate a models ability to learn dynamics (\eg, Diving48 and DAVIS) might need to be reevaluated. Interestingly, we showed that models trained on Diving48 are largely using static information to make their predictions, contrasting previous assumptions that Diving48 is a ``temporally heavy dataset''. For the task of video object segmentation, TAO-VOS was found to have a better balance between static and dynamic factors than the widely adopted DAVIS dataset. 

% Video understanding is a complex and unsolved problem. The main flaws of current state-of-the-art models and benchmark datasets are poorly understood and requires a more fine-grained understanding of what information and biases are contained in the intermediate representations of DNNs. We strongly believe that our proposed framework will allow for further analysis into how spatiotemporal models make predictions, which datasets are candidates for evaluating dynamic understanding, and offer multiple directions to improve algorithms in their ability to encode temporal information.


This paper has advanced the interpretability of learned spatiotemporal models for video understanding, especially action recognition, AVOS and VIS. We introduced a general method for analyzing the extent that various architectures capitalize on static \vs dynamic information. We showed how our method can be applied to investigate the static \vs dynamic biases in datasets. Furthermore, we demonstrated the impact of static and dynamic biases on overall performance through a new type of regularization for action recognition (StaticDropout) and architectural modifications in the fusion and cross connection layers for AVOS. Future work can apply our method to additional video understanding tasks (\eg action prediction) and use the proposed performance enhancing techniques on different datasets, architectures and tasks which require dynamics.

==> core/graphs/vos_arch_indiv_histograms.tex <==

\begin{figure*}[t]
\centering
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/fseg/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/matnet/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/rtnet/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%

\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/fusionseg/app_fseg.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/fusionseg/mot_fseg.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/matnet/app_matnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/matnet/mot_matnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/rtnet/app_rtnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/rtnet/mot_rtnet.png}
    \caption{}
\end{subfigure}

    \caption{Individual Units Analysis Histograms in (a,b) FusionSeg~\cite{jain2017fusionseg} modified and (c,d) MATNet~\cite{zhou2020motion} respectively. It shows the histogram for static (a,c) and dynamic (b,d) factors for both models. }
    \label{fig:vos_indiviual_units}
\end{figure*}

==> core/graphs/vos_dataset_astable.tex <==
\begin{figure} [t]
\begin{center}

% \resizebox{0.47\textwidth}{!}{

% \begin{tabular}{c |cc|cc|cc}
% \specialrule{1.2pt}{1pt}{1pt}

%  \multirow{2}{*}{Method}&  \multicolumn{2}{c}{\textbf{TAO-VOS}} & \multicolumn{2}{c}{\textbf{ImageNetVID}} &  \multicolumn{2}{c}{\textbf{TAO-VOS}}   \\
% %\hline
%   & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%) \\
%     \specialrule{1.2pt}{1pt}{1pt}
%     	\specialrule{1.2pt}{1pt}{1pt}
% Sensor Fusion L5 & 26.4 & 25.8 & 26.4 & 33.1 & 27.8 & 30.1 \\ 
% Sensor Fusion L2 & 33.7 & 23.2 & 33.0 & 24.6 & 34.0 & 25.9 \\ \hline

% %TAO-VOS & 26.4 & 25.8  & 33.7 & 23.2 \\
% \end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\arraystretch{1.35}
\setlength\tabcolsep{2.4pt}
 
\resizebox{0.47\textwidth}{!}{
\begin{tabu}{c cccc}
\tabucline[1pt]{-}
 \multirow{2}{*}{Dataset}&  \multicolumn{2}{c}{\textbf{Fusion Layer5}} & \multicolumn{2}{c}{\textbf{Fusion Layer2}}    \\
\cline{2-5}
  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)\\
\tabucline[1pt]{-}
TAO-VOS & 26.4 & 25.8  & 33.7 & 23.2 \\
ImageNetVID & 26.4 & 33.1 & 33.0 & 24.6  \\
DAVIS & 27.8 & 30.1 & 34.0 & 25.9 \\

\tabucline[1pt]{-}
\end{tabu}
%%%%%%%%%%%%%%%%%%%%%%5
\hspace{0.08cm}
\begin{tabular}{c}
\includegraphics[width=0.12\textwidth]{tex/images/saliency_priors/prior2.pdf}
\end{tabular}

}
\end{center}
\vspace{-0.4cm}
\caption{Dynamic and static biases of video object segmentation datasets using the layer-wise metric, (\ref{eq:biasscores}). \textbf{Left}: Encoding of dynamic and static factors for FusionSeg model last sensor fusion layer, trained on \textbf{DAVIS}, \textbf{ImageNetVID} and \textbf{TAO-VOS}. \textbf{Right}: Center bias plots for DAVIS, ImagenetVID and TAO-VOS datasets. The first two datasets have more center bias than TAO-VOS. \textcolor{blue}{Order plots on right in the same order as table entries on the left and adjust the caption correspondingly. Also, the caption says that the LHS shows results for the \textit{last} sensor fusion layer only, while the actual table shows results for that layer and another. As it stands, I've deleted the interpretation and moved it to the text, because it seems a bit more complicated than was tersely stated here.}}\label{fig:vos_dataset}
\end{figure}

==> core/graphs/vos_iterwise.tex <==
\begin{figure}
\begin{tikzpicture}[trim axis left,trim axis right]\ref{target_legend7}
    \begin{axis}[
      line width=1.0,
        title={MATNet - (DAVIS+YTB)},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\normalsize},
        xlabel={Epoch},
        x label style={font=\small},
        ylabel={Number of Units (\%)},
        xmin=-1, xmax=200,
        ymin=15, ymax=40,
        xtick={20,40,60,80,100,120,140,160,180},
        ytick={20, 25, 30, 35, 40},
        % yticklabels={,,},
        x tick label style={font=\tiny, rotate=0, anchor=north},
        y tick label style={font=\tiny},
        x label style={at={(axis description cs:0.5,0.1)},anchor=north,font=\small},   
        y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},        width=6.5cm,
        height=4.3cm, % height=4.3cm,   
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend columns=2,
        legend style={
        % mark options={scale=0.1}
         nodes={scale=0.6, transform shape},
         cells={anchor=west},
         legend style={at={(1.9,0.0)},anchor=south,row sep=0.01pt}, font =\normalsize},
         legend entries={[black]Fusion2Static,[black]Fusion5Static,[black]Fusion2Dynamic,[black]Fusion5Dynamic},
        legend to name=target_legend7,
    ]
   %
    \addplot[line width=1.2pt,mark size=1.1pt,color=cyan]
        coordinates {(0,20.0)(5,22.5)(10,23.3)(15,25.0)(25,24.5)(45,26.5)(50,25.4)(60,28.5)(75,23.8)(80,24.4)(85,24.7)(90,24.7)(95,26.0)(105,24.7)(110,24.3)(115,23.7)(120,24.3)(125,23.7)(130,25.5)(140,24.1)(145,23.0)(150,23.5)(155,24.6)(160,24.1)(165,23.9)(170,24.3)(175,24.2)(180,23.4)(185,24.1)(190,24.0)};
    % APPEARANCE
    \addplot[line width=1.2pt,mark size=1.1pt,color=orange]
        coordinates {(0,39.6)(5,35.9)(10,23.3)(15,25.0)(25,34.0)(45,29.1)(50,30.7)(60,28.3)(75,34.0)(80,33.4)(85,32.5)(90,32.5)(95,31.4)(105,31.7)(110,31.1)(115,33.9)(120,33.7)(125,34.5)(130,31.1)(140,33.9)(145,33.3)(150,33.9)(155,32.7)(160,32.9)(165,33.4)(170,33.0)(175,32.8)(180,33.5)(185,32.9)(190,32.9)};
        % FAST
        % MOTION
    \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=cyan]
        coordinates {(0,22.3)(5,25.8)(10,27.3)(15,28.5)(25,27.7)(45,32.0)(50,31.2)(60,29.7)(75,28.5)(80,30.9)(85,31.6)(90,31.6)(95,32.8)(105,29.3)(110,31.6)(115,31.2)(120,33.6)(125,33.6)(130,31.2)(140,30.5)(145,30.9)(150,32.0)(155,32.4)(160,30.5)(165,31.2)(170,30.9)(175,30.1)(180,30.1)(185,30.9)(190,29.7)};
    % APPEARANCE
     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=orange]
        coordinates {(0,38.3)(5,32.4)(10,27.0)(15,25.0)(25,27.0)(45,23.0)(50,23.4)(60,22.7)(75,21.9)(80,21.9)(85,22.7)(90,20.7)(95,20.7)(105,21.9)(110,23.0)(115,23.4)(120,21.9)(125,22.3)(130,20.7)(140,22.7)(145,22.7)(150,21.9)(155,22.7)(160,22.7)(165,22.7)(170,21.1)(175,21.9)(180,23.4)(185,22.3)(190,22.7)};
\end{axis}
\end{figure}

==> core/intro.tex <==



% WHAT
% Deep spatiotemporal models, that learn features across space and time, have proven effective in a wide range of video understanding tasks~\cite{wang2021survey,zhu2020comprehensive,aafaq2019video}. The architecture design of these models can be broadly categorized (agnostic of the down-stream task) to (1) two-stream approaches that separately model motion and appearance features~\cite{carreira2017quo,jain2017fusionseg,zhou2020motion,ren2021reciprocal,feichtenhofer2019slowfast}, (2) models relying on 3D convolutions~\cite{carreira2017quo}, (3) attention based models with different forms of spatiotemporal data association~\cite{bertasius2021space,ren2021reciprocal}, (4) models relying on recurrent neural networks~\cite{tokmakov2017learning}, and (5) hybrid models that combine some of the previous~\cite{tokmakov2017learning,carreira2017quo, ren2021reciprocal}. The majority of these models learn hierarchical static and dynamic features in a distributed and end-to-end fashion. 
\IEEEPARstart{T}{his} paper focuses on the problem of interpreting the information learned by deep neural networks (DNNs) trained for video understanding tasks. Interpreting deep spatiotemporal models is a largely understudied topic in computer vision despite their achieving state-of-the-art performance on video understanding tasks, such as action recognition~\cite{zhu2020comprehensive} and video object segmentation~\cite{wang2021survey}. These models are trained in an end-to-end fashion to learn discriminative static and dynamic features over space and time. 
Here, we use the term \textit{static} to refer to attributes that can be extracted from a single image (\eg color and texture) and the term \textit{dynamic} to attributes that arise from consideration of multiple frames (\eg motion and dynamic texture). 

% WHY - XAI, VIDEO XAI
While this learning-based paradigm has led to great success across a wide range of tasks, the internal representations of the learned models remain largely opaque. This lack of explainability is unsatisfying from both scientific and application perspectives. From a scientific perspective, there is limited understanding of what information is driving the decision-making underlying the network output. Elucidating
the decision-making process may yield directions to improve models. From an applications perspective, there have been multiple cases showing 
the ethical and damaging consequences of deploying opaque vision models, 
%without understanding their decision-making process 
\eg~\cite{buolamwini2018gender,hansson2021self}.
%that deploying computer vision models without understanding how they make predictions can lead to unethical and
%damaging consequences, \eg,~\cite{buolamwini2018gender,hansson2021self}. 
Currently, however, the explainability of spatiotemporal models is under-explored~\cite{hiley2019explainable}. Some evidence suggests that these models exhibit considerable bias toward static information, \eg~\cite{vu2014predicting,he2016human,choi2019can,ilic2022appearance}; therefore, an interesting question 
%to address regarding 
to answer about 
the representations in deep spatiotemporal models is: \textit{How much static and dynamic information is being captured}? While a few video interpretation methods exist, they have various limitations, \eg being primarily qualitative~\cite{feichtenhofer2020deep}, using a certain dataset that prevents evaluating the effect of the training dataset~\cite{hadji2018new} or using classification accuracy as a metric without quantifying 
%semantic concepts in 
a model's \textit{internal} representations~\cite{hadji2018new, sevilla2021only,ilic2022appearance}.



\begin{figure}[t]
\centering
    \vspace{-0.4cm}
    \resizebox{0.48\textwidth}{!}{
    \includegraphics[]{images/teaser.pdf}}
    \vspace{-0.5cm}
    \caption{We introduce a general approach that, given a trained spatiotemporal model and a video dataset, can quantify the bias in any hidden representation within the model toward encoding static (red) or dynamic (blue) information. We use this technique to study action recognition (squares) and video segmentation (diamonds) and explore the effect of models and training datasets on static and dynamic biases.}
\vspace{-2em}
\end{figure}\label{fig:motivation}

%While this algorithmic paradigm is likely a reason for many of the recent successes involving deep learning, it also creates the issue of these models being largely black-box algorithms. Additionally, the video-understanding research community lacks a general understanding of what spatiotemporal models are learning in the intermediate features. 

% In this paper, we tackle this important but largely understudied problem and propose a quantifiable measure for estimating the bias towards learning static and temporal information in a models representations. More specifically, we define bias towards a certain factor (dynamic or static) as the percentage of units within intermediate layers that are affected by that factor. We demonstrate, through a comprehensive series of experiments, that two main elements affecting these biases include model design (such as cross connections in two-stream models, input modalities, or the use of slow and fast pathways) and training datasets. We further confirm the emergence of units in the learned intermediate representations that \textit{jointly encode} static and dynamic information. 
%We mainly focus on the first three broad categories that learn spatiotemporal features and the hybrid models based on them. 

%  Deep spatiotemporal models, that learn features across space and time, have proven effective in a wide range of tasks~\cite{wang2021survey}\cite{feichtenhofer2019slowfast}\cite{bertasius2021space}. They can be broadly categorized agnostic of the down-stream task to: (1) Two-stream approaches~\cite{carreira2017quo}\cite{jain2017fusionseg}\cite{zhou2020motion}\cite{ren2021reciprocal}. (2) Models relying on 3D convolution~\cite{carreira2017quo}. (4) Attention based models with different forms of temporal attention~\cite{bertasius2021space}\cite{ren2021reciprocal}. (5) Models relying on recurrent neural networks~\cite{tokmakov2017learning}. and (6) Hybrid models that combine few of the previous~\cite{tokmakov2017learning}\cite{carreira2017quo}. However, the current literature lacks a general understanding of what these models learn and whether they are biased towards temporal or appearance factors. In this paper we propose a quantifiable measure for estimating the bias towards temporal/appearance on the intermediate representations learned. We mainly focus on the first three broad categories of spatiotregularizersemporal models. Factors affecting that bias including model design decisions (such as cross connections in two-stream, or combining slow and fast path-ways) and training datasets are studied to provide interesting insights. We further demonstrate results that confirm the emergence of units in the learned intermediate representations that jointly encode appearance and temporal. 

% Additionally, our proposed metric for estimating individual unit biases can be of further use in model compression through pruning~\cite{zhu2017prune}. Thus, our work has important implications for industry as it seeks regulatory approval and compact algorithms for its AI products and services, \eg, mobile applications and autonomous driving.

% Techniques which can measure the concepts captured in the models latent representations can be seen as a means towards Explainable AI. There have been multiple incidences in recent years which have shown that deploying computer vision models before understanding how they make predictions can lead to unethical and damaging consequences~\cite{buolamwini2018gender,hansson2021self}. This has encouraged regulatory bodies to place law requirements of explainability in deployed DNNs~\cite{hamon2020robustness,ontario_law}. % A number of recent works have demonstrated that spatiotemporal models contain significant biases towards static information. For example, models can achieve good performance on popular action recognition benchmarks without looking at the human~\cite{he2016human} or using only static scenes~\cite{vu2014predicting,choi2019can}. 

% HOW

% old version nov 11
% In response, we present a quantitative paradigm for evaluating the extent that spatiotemporal models are biased toward static or dynamic information in their internal representations.
% More specifically, we define bias toward a certain factor (dynamic or static) as the percentage of units within intermediate layers that encode that factor. Inspired by previous work~\cite{islam2021shape,esser2020disentangling}, we propose a metric to estimate the amount of static/dynamic bias based on the mutual information between sampled video pairs corresponding to these factors. We explore two common tasks in this study to show the efficacy of our approach as a general tool for understanding spatiotemporal models: (i) action recognition and (ii) video object segmentation. We choose these two tasks to demonstrate the generality of our approach, as they have different semantics (\ie, multi-class vs.\ binary classification), labelling (\ie, video-level vs.\ pixel-level), input types (multi-frame images vs.\ single frame optical flow). We focus our study on answering the following three questions: (i) What effect does the model architecture have on static and dynamic biases? (ii) How does the training dataset affect these biases? (iii) What role do units that jointly encode static and dynamic information play in relation to the architecture and dataset? 

% Overall, we make three main contributions: First, We introduce a general framework for quantifying the amount of static and dynamic bias contained in spatiotemporal models. This includes a novel sampling procedure to produce static and dynamic video pairs, and a method for identifying units that jointly encode static and dynamic factors.  Second, we provide a unified study on two widely researched tasks, action recognition and video object segmentation. In \textit{action recognition}, we study numerous architectures, including 3D CNNs~\cite{carreira2017quo,feichtenhofer2020x3d}, two-stream networks~\cite{feichtenhofer2019slowfast}, and Transformers~\cite{bertasius2021space,fan2021multiscale}. In \textit{video object segmentation}, we study two-stream architectures~\cite{jain2017fusionseg,zhou2020motion,ren2021reciprocal} with different forms of cross connections. We discover in both tasks that all networks are heavily static biased except for two-stream architectures with cross connections that encourage models to better capture dynamics. (3) We also apply our proposed approach to three datasets, which differ in size and granularity. For action recognition, we consider Kinetics~\cite{carreira2017quo}, Something-Something-v2~\cite{goyal2017something} (SSv2), and Diving48~\cite{li2018resound}. For video object segmentation, we consider DAVIS~\cite{Perazzi2016} Imagenet VID~\cite{jain2017fusionseg}, and TAO VOS~\cite{Voigtlaender21WACV, Dave20ECCV} to reveal the impact of training datasets on these tasks. Additionally, we perform a detailed analysis to confirm, contrary to previous beliefs~\cite{li2018resound,bertasius2021space}, that Diving48 dataset is an appearance biased dataset and SSv2 is better suited to evaluate a models ability to capture dynamics. 


% new version
In response, we present a quantitative paradigm for evaluating the extent that spatiotemporal models are biased toward static or dynamic information in their internal representations.
We define bias toward a certain factor (dynamic or static) as the percentage of units (\ie channels) within intermediate layers that encode that factor; see Fig.~\ref{fig:motivation} (top). Inspired by previous work~\cite{esser2020disentangling,islam2021shape}, we propose a metric to estimate the amount of static \vs dynamic bias based on the mutual information between sampled video pairs corresponding to these factors. We explore three common tasks %in this study 
to show the efficacy of our approach as a general tool for understanding spatiotemporal models, action recognition, automatic video object segmentation (AVOS) and video instance segmentation (VIS). We focus our study on answering the following five questions: (i) How do model architectures affect static and dynamic biases? (ii) How does the training dataset affect these biases? (iii) What role do units that jointly encode static and dynamic information play in relation to the architecture and dataset? (iv) When are statics and dynamics learned during training? (v) What impact do these biases have on performance? In regards to the last question, we demonstrate that controlling the static and dynamic biases in action recognition and AVOS can improve performance on tasks requiring dynamics.

\noindent{\bf Contributions.} We make five main contributions in this extension to our previous work~\cite{kowal2022deeper}. (i) We introduce a general method for quantifying the static and dynamic bias contained in spatiotemporal models, including a novel sampling procedure to produce static and dynamic video pairs. (ii) We propose a technique for identifying units that jointly encode static and dynamic factors. (iii) Using the aforementioned techniques, we provide a unified study on three widely researched tasks, action recognition, AVOS and VIS, with a focus on the effect of architecture and training dataset on a model's static and dynamic biases; see Fig.~\ref{fig:motivation} (bottom). (iv) We propose StaticDropout, a semantically guided dropout technique for debiasing models from statics and toward dynamics that can improve model performance on datasets which require dynamics. (v) We demonstrate how a proper selection of the fusion and cross connection modules in AVOS architectures can guide a model to learn better dynamics and improve performance for the task of segmenting camouflaged entities.
% We provide a detailed analysis on the fusion and cross connections in AVOS architectures and, through the proper combination of the modules, demonstrate our ability to influence a model to learn better dynamics.
Among other findings, we discover that all studied networks are heavily static biased, except for two-stream architectures with cross connections encouraging models to capture dynamics. We show that the majority of models converge to their final static and dynamic biases within the first half of training iterations. Additionally, we confirm that, contrary to previous beliefs~\cite{li2018resound,bertasius2021space}, the Diving48~\cite{li2018resound} dataset is not dynamically biased and Something-Something-v2 (SSv2)~\cite{goyal2017something} is better suited to evaluate a model's ability to capture dynamics. Publicly available code is available\footnote{\url{https://yorkucvil.github.io/Static-Dynamic-Interpretability/}}.
% In \textit{action recognition}, we study numerous architectures, including 3D CNNs~\cite{carreira2017quo,feichtenhofer2020x3d}, two-stream networks~\cite{feichtenhofer2019slowfast}, and Transformers~\cite{bertasius2021space,fan2021multiscale}. In \textit{video object segmentation}, we study two-stream architectures~\cite{jain2017fusionseg,zhou2020motion,ren2021reciprocal} with different forms of cross connections. 
% We discover in both tasks that all networks are heavily static biased except for two-stream architectures with cross connections that encourage models to better capture dynamics. (3) We also apply our proposed approach to three datasets, which differ in size and granularity. For action recognition, we consider Kinetics~\cite{carreira2017quo}, Something-Something-v2~\cite{goyal2017something} (SSv2), and Diving48~\cite{li2018resound}. For video object segmentation, we consider DAVIS~\cite{Perazzi2016} Imagenet VID~\cite{jain2017fusionseg}, and TAO VOS~\cite{Voigtlaender21WACV, Dave20ECCV} to reveal the impact of training datasets on these tasks. Additionally, we perform a detailed analysis to confirm, contrary to previous beliefs~\cite{li2018resound,bertasius2021space}, that Diving48 dataset is an appearance biased dataset and SSv2 is better suited to evaluate a models ability to capture dynamics. 


%Finally, we use our findings to make algorithmic improvements on a difficult dataset biased to the dynamics.  

% , through a comprehensive series of experiments on both tasks, that two main elements affecting biases towards dynamics include model design (such as cross connections in two-stream models, input modalities, or the use of slow and fast pathways) and training datasets. We further confirm the emergence of units in the learned intermediate representations that \textit{jointly encode} static and dynamic information. 


%Recent work~\cite{zhi2021mgsampler} proposed an explainable temporal guided sampling in video recognition, but they do not provide a mean for understanding what the intermediate representations learned. On the other hand, our method provides a quantifiable measure for understanding intermediate representations learned in spatiotemporal models and assessing its effect on the downstream tasks. We perform our study on two widely studied tasks, action recognition and video object segmentation, to show the broad applicability of our proposed method and analysis. 



==> core/method.tex <==
%\newcommand{\covariance}[1]{\text{Cov}\bigl(#1\bigr)}
%\newcommand{\variance}[1]{\text{Var}(#1)}
%\newcommand{\MI}{\operatorname{MI}}
We introduce an approach to quantify the number of units encoding static and dynamic information in spatiotemporal models; for an overview, see % The overall method is presented in
Fig.~\ref{fig:mainmethod}. Our approach consists of two main steps. First, given a pretrained spatiotemporal model, we sample static and dynamic video pairs (Sec.~\ref{sec:sampling}). 
% In our study, we consider a wide range of standard architectures, ranging from convolution to transformers, and various standard video datasets. 
Second, we use the static and dynamic pairs to estimate the number of units in the model encoding each factor based on the mutual information shared between the pairs (Sec.~\ref{sec:mmi}).

\vspace{-0.4cm}
\subsection{Sampling static and dynamic pairs}\label{sec:sampling}
\noindent \textbf{Why static and dynamic?}
We define static as `information arising from single frames' and dynamic as `information arising from the consideration of multiple frames'. The main alternative attribute to dynamics that we considered is `image motion' (\ie trackable points or regions), but `motion' is a subset of dynamic information~\cite{wildes2000qualitative,derpanis2011spacetime} (\eg stationary flashing lights have dynamics but no motion). Thus, we consider dynamics over motion because it encompasses a wider range of visual phenomena. In complement, we choose the term `static' over the possible alternative `appearance', because dynamics also can provide appearance information,~\eg object contours, even if camouflaged in a single frame, can be revealed through motion.
For our metric, we produce video pairs that contain the same static information and perturbed dynamics, or vice versa, with the end goal of analyzing models trained on large-scale real-world datasets. We now detail our static and dynamic sampling techniques, as visualized in Fig.~\ref{fig:mainmethod} (panel 1).

%Moreover, it is a more viable option for generating video pairs sharing the same information over multiple frames. We also point out that it may not be possible to fully disentangle static information from dynamic information (particularly when considering real world video data). For example, given the movement of an object in an image, the boundary of the object is contained in both the static (\eg contour of a single frame) and dynamic (\eg contour displacement over multiple frames). Despite this issue, we believe that some overlap of information between the static and dynamic video pairs is acceptable as long as the perturbation of static information is sufficient. Given these two factors, we now detail our static and dynamic sampling techniques for both action recognition and VOS, which are visualized in Fig.~\ref{fig:mainmethod} (panel 1). 

% \blue{Kosta: Need to discuss the following - The main alternative to dynamics that we considered is the factor of `motion' (\ie imagery with trackable points), but `motion' is a subset of dynamic information~\cite{derpanis2009detecting} (\eg stationary flashing lights have dynamics but no motion). Thus, we consider dynamics over motion because it is a more viable option for generating video pairs which share the same information over multiple frames. Additionally, we use static opposed to other spatial features (\eg appearance) since we use optical flow as the input to VOS models. Rich appearance information (\eg object shape and boundaries) can be directly interpreted from optical flow maps while static information cannot (\ie static information considers only a single frame).} Given these two factors, we now detail our static and dynamic sampling techniques for both action recognition and VOS, which are visualized in Fig.~\ref{fig:mainmethod} (panel 1).




% We introduce a novel sampling method that provides static and dynamic video pairs to compute the mutual information. While multiple semantic factors could be considered using our technique, we choose to focus this study on `static' and `dynamic' factors for the following reasons. First, other factors (\eg motion and appearance) may not be possible to disentangle. In particular, both motion and appearance can relay information on the object shape. Thus, it is hard to disentangle the two when constructing a method for sampling videos which share the same motion, but not appearance, especially since our goal is to provide an analysis on state-of-the-art models trained on large-scale real-world datasets. To this end, we choose the factors of \textit{static}, which refers to features that can be extracted from a single frame, and \textit{dynamic}, which considers only attributes that arise from consideration of multiple frames. We now detail our sampling techniques for both action recognition and VOS, which is visualized in Fig.~\ref{fig:mainmethod} (panel 2). 

\noindent \textbf{Action recognition.} The action recognition models we consider take in multiple frames (four to thirty-two). To construct video pairs with the \textit{same} dynamics but \textit{different} static information (\ie~\textit{dynamic pairs}), we consider the same video but with two \textit{different} video styles. For video stylization, we use a recent video stylization method (with four possible styles) that perturbs static attributes like color, pixel intensity and texture~\cite{texler2020interactive}, but has less temporal artifacts (\eg flickering) than stylization methods that consider each image independently~\cite{huang2017arbitrary}. These video pairs will contain objects and scenes that have identical dynamics, but have perturbed static information. To construct pairs with the \textit{same} static information but \textit{different} dynamics (\ie~\textit{static pairs}), we take two videos of the same style, but randomly \textit{shuffle} the frames along the temporal axis; see Fig.~\ref{fig:mainmethod} (panel 1, left). In this case, the temporal correlations are altered while the static (\ie per-frame) information remains identical.

\noindent \textbf{Video object segmentation.} The AVOS models considered~\cite{jain2017fusionseg,zhou2020motion,ren2021reciprocal} take a single RGB frame and an optical flow frame as input to the appearance and motion streams, resp.; %(note the flow representation used in these works is not vectorized but RGB flow where the hue and saturation can control the direction and magnitude, respectively. 
see Fig.~\ref{fig:mainmethod} (panel 1, right). Therefore, we apply an alternative method to frame shuffling to obtain the \textit{static} pairs. For the \textit{static} pair, we use RGB images with the \textit{same} style but alter the dynamics by jittering the optical flow. % the dynamics by changing the hue and saturation of the optical flow map in it. 
The RGB flow representation is used with hue and saturation encoding direction and magnitude, resp., and it is those parameters that we jitter.
For the \textit{dynamic} pairs, we use the \textit{same} optical flow but a \textit{different} image style. For creating stylized images, we use the same video stylization techniques noted above for action recognition~\cite{texler2020interactive}, and then sample frames from the generated video. 

\noindent \textbf{Video instance segmentation.} The inputs to the VIS models considered~\cite{wang2021end} take single stream, multi-frame RGB inputs. Therefore, we select static and dynamic pairs similar to action recognition models, \ie shuffling and stylization for static and dynamic pairs, respectively.

% \begin{figure*}[t]
%     \includegraphics[width=\textwidth]{tex/images/main_figs/main_method.pdf}
%     % \vspace{-0.2cm}
%     \caption{Overview of our method for factor bias analysis.  We measure the dynamic and static biases in deep spatiotemporal models for two tasks: action recognition and video object segmentation. \textbf{(1)} We sample video pairs that share either \textit{static}, $(v^S_1, v^S_2)$, or \textit{dynamic}, ($v^D_1,v^D_2$), information using video stylization~\cite{texler2020interactive} and frame shuffling or optical flow jitter (flow visualized in RGB format). \textbf{(2)} Given a pretrained model, $f_\theta$, we compute the mutual information (MI) between intermediate representations of video pairs, $z^F$, to assess the model's bias toward either factor on a per-layer, $l$, or per-channel (\ie unit) basis. In the supplement, we provide stylization examples in video format as well as additional static and dynamic samples.}
%     \label{fig:mainmethod}
% \end{figure*}

\vspace{-0.5cm}
\subsection{Estimating static and dynamic units} \label{sec:mmi}

We seek to quantify the number of units (\ie \textit{channels}) in a layer encoding \textit{static} or \textit{dynamic} information and the extent to which individual units perform static, dynamic or joint encodings. Inspired by recent work that focused on single images~\cite{esser2020disentangling,islam2021shape}, we use %propose to use 
a mutual information estimator to measure the information shared between video pairs. 
% More specifically, we sample video pairs that contain the same \textit{static} or \textit{dynamic} information, but not both. The sampling strategy and method for generating such pairs of semantically similar videos as explained in Sec~\ref{sec:sampling}. 

\noindent\textbf{Layer-wise metric.} Given a pre-trained network, $f_\theta$, and a pair of videos, $v^F_1$
and $v^F_2$, that share the semantic factor $F$ (\ie \textit{static} or \textit{dynamic}), we compute the features for an intermediate layer $l$ as $z^F_1 = f^l_{\theta}(v^F_1)$ and $z^F_2 = f^l_{\theta}(v^F_2)$ (omitting the $l$ on $z$ to reduce notation). We use $z^F_1(i), z^F_2(i)$ to denote the $i^{\text{th}}$ unit (\ie channel) in $N^l$ dimensional features after a global average pooling layer. Units biased toward the \textit{static} factor will result in a higher correlation among \textit{static} pairs than the \textit{dynamic} pairs and vice versa. Under the assumption that units in the intermediate representation, $z^F_1(i)$ and $z^F_2(i)$, across the dataset are jointly Gaussian, the correlation coefficient can be used as a lower bound on mutual information~\cite{kraskov2004estimating,foster2011lower}, as used in previous work~\cite{esser2020disentangling,islam2021shape}.
%Although layer responses are not exacl
%(note although this assumption is not likely to hold exactly for a DNNs representations, 
% Although layer responses may not be exactly Gaussian, previous work has empirically demonstrated the tightness of the bound for DNNs is sufficient for our purposes ~\cite{esser2020disentangling,islam2021shape} \blue{Really? Appears to be a weak justification.  Inviting reviewers to jump on it.}).
The number of units encoding factor $F$, $N_F$, is obtained by computing the correlation coefficient, $S_F$, over all $N^l$ channels between all video pairs $z^F_1, z^F_2$, as
\vspace{-0.3cm}
% \begin{equation}
% \begin{split}
%   N_F = \sigma(\textbf{S})\cdot N^l = \frac{\exp{(S_F)}}{\sum\limits_{k=0}^K{\exp{(S_k)}}} \cdot N^l,\\
%      S_F = \sum\limits_{i=1}^{N^l} \frac{\text{Cov}(z^F_1(i), z^F_2(i))}{
%         \sqrt{\text{Var}(z^F_1(i)) \;\text{Var}(z^F_2(i))}},
% \end{split}\label{eq:biasscores}
% \end{equation}
\begin{equation}
\begin{split}
  N_F = \frac{\exp{(S_F)}}{\sum\limits_{k=0}^K{\exp{(S_k)}}} \cdot N^l,
     S_F = \sum\limits_{i=1}^{N^l} \frac{\text{Cov}(z^F_1(i), z^F_2(i))}{
        \sqrt{\text{Var}(z^F_1(i)) \;\text{Var}(z^F_2(i))}},
\end{split}\label{eq:biasscores}
\end{equation}
where we multiply the Softmax by the number of units in that layer, $N^l$, to compute the number of units encoding the semantic factor $F$ relative to the other factors considered and $K=\{{\text{static}, \text{dynamic}, \text{identical}}\}$. In addition to \textit{static} and \textit{dynamic}, we consider a third factor in (\ref{eq:biasscores}), the \textit{identical} factor, where the video pairs have the same static and dynamic factors (\ie same video, style, frame ordering and optical flow). This baseline factor is the correlation between the model's encoding of the same videos, that gives $S_\text{Identical}=1$ for all layers. %which ensures that the dimensionality of all factors will be equal if they are all captured entirely by $f_{\theta}$.

% \textcolor{blue}{You say you multiply by the number of units, $N$, at layer $l$. But only $N^l$ appears in the equations, which earlier is defined as the feature dimensions of a unit. Clarification is needed.}

\noindent\textbf{Unit-wise metric.} The correlation coefficient, $S_F$, estimates the relative amount of static and dynamic information over all units in a particular layer; note the pooling done by the summation \textit{before} the Softmax in the layer-wise metric, (\ref{eq:biasscores}). However, it is also desirable to measure static and dynamic information contained in each individual channel. This measurement allows for a more fine-grained analysis of how many channels (\ie units) encode a factor $F$ above a certain threshold, as well as identify any joint or residual (\ie non-dynamic or static) units. Thus, we categorize each unit based on how much information (\ie static \vs dynamic) is encoded, whether any units jointly encode both factors or if there are units that do not correlate with either type of information. We measure the amount of static and dynamic information encoded in each unit  $i \in {1, \dotsc, N^l}$ as
%To measure individual units we simply compute the score on the individual unit:
\begin{equation}
s^i_{F} = \frac{\text{Covariance}(z^F_1(i), z^F_2(i))}{\sqrt{ \text{Variance}( z^F_1(i)) \text{Variance}( z^F_2(i))}},\label{eq:bias_scores_indv}
\end{equation} 
where each $s^i_{F}$ is the information of semantic factor $F$ in unit $i$. Given these individual correlations, we calculate the individual factors by excluding the use of a Softmax and simply threshold the correlation for each factor with a constant parameter, $\lambda$, to yield our unit-wise metrics as
% The first method (see Eq.~\ref{eq:ind_bias_scores_diff_a}) simply performs a \texttt{softmax} over each unit and produces a dynamic and static score. 
% \begin{subequations}
% \begin{equation}
% P^i_F = \frac{\texttt{exp}(s^i_F)}{\sum\limits_{k=0}^K \texttt{exp}(s^i_k)}
% \label{eq:ind_bias_scores_diff_a}
% \end{equation}
% \begin{equation}
% \begin{split}
% N_{\text{Joint}} = \sum_{i=1}^N\mathbbm{1}[ s^i_{F} > \lambda \forall_F \in K] \\
% N_{\text{F}} = \sum_{i=1}^N\mathbbm{1}[ s^i_{F} > \lambda \land s^i_{k} < \lambda \forall_k \in K, k \neq F] \\
% N_{\text{None}} = \sum_{i=1}^N\mathbbm{1}[ s^i_F < \lambda \forall_F \in K].
% \end{split}
% \label{eq:ind_bias_scores_diff_b}
% \end{equation}
% %\label{eq:ind_bias_scores_diff}
% \end{subequations}
\begin{equation}
\begin{split}
N_{\text{F}} = \sum_{i=1}^{N^l}\mathbbm{1}[ s^i_{F} > \lambda \land s^i_{k} < \lambda \forall k \in K, k \neq F] \\
N_{\text{J}} = \sum_{i=1}^{N^l}\mathbbm{1}[ s^i_{F} > \lambda \forall F \in K], \,
N_{\text{R}} = \sum_{i=1}^{N^l}\mathbbm{1}[ s^i_F < \lambda \forall F \in K],
\end{split}
\label{eq:ind_bias_scores_diff_b}
\end{equation}
where $K=\{\text{static}, \text{dynamic}\}$, $N_{\text{J}}$ indicates units jointly encoding both and $N_{\text{R}}$ are residual units not correlating with these factors under a threshold, $\lambda$. Note that we assign units to either joint, dynamic, static or residual and do not allow for an overlap to occur. This approach allows us to investigate the existence of units that jointly encode static and dynamic factors. For all experiments, we set $\lambda=0.5$ since it is halfway between \textit{no} and \textit{full} positive correlation. 
% The supplement has results with varying $\lambda$.
% Please see the Supplemental Material for experiments with varying threshold values, $\lambda$.

%These two methods each have their own advantages. Unlike the second method, the first approach (Eq.~\ref{eq:ind_bias_scores_diff_a}) does not require a hyper-parameter threshold to be set, and the assumption on the residuals factor allows for capturing the remaining factors not encoded by spatial or temporal ones. This strongly relates to what has been shown in previous works~\cite{esser2020disentangling} that there are residual factors not encoded in the considered semantic factors, and the dimensionality estimation technique should consequently consider them. It also allows us to rank all $N$ units according to the temporal, spatial, and residual scores. This can be used to evaluate the performance of the model when removing the top $M$ units for each of these three factors as shown in the results section~\ref{}. 

%On the other hand, the second method removes the hard assumption on the existance of residual factors, with scores $s^i_0 = 1$. It only estimates units that does not correlate to neither of the considered semantic factors under a certain threshold. This has the advantage to let us discover models that do not have any residual factors even under different $\lambda$ thresholds as shown in the appendix section~\ref{}. Additionally, it allows us to isolate units which jointly encode spatial and temporal information (a phenomenon identified in previous work~\cite{feichtenhofer2020deep}).

%will not allow for this, as there may only exist a handful of units encoding a semantic factor with a score greater than $\lambda$ (and this finding is supported experimentally). On the other hand, method 2 removes the assumption of any residual factor, which may result in a more meaningful calculation of $N_{residual}$ rather than assuming $s^i_0 = 1$. Additionally, method two allows us to isolate units which jointly encode spatial and temporal information (a phenomenon identified in previous work~\cite{feichtenhofer2020deep}). 


==> core/related.tex <==
\noindent \textbf{Interpretability of spatiotemporal models.}
%Spatiotemporal models is vastly adopted in different video tasks such as action recognition and video object segmentation. Early action recognition methods relied on 3D convolutions, and two-stream architectures that use optical flow as input. Recent improvements to learn without explicit optical flow was introduced in, with slow and fast branches. Recently, spatiotemporal attention has been investigated for action recognition tasks. 
%video segmentation using deep learning has been recently surveyed in~\cite{wang2021survey}, that categorized the main approaches into automatic, semi-automatic and interactive methods. Our current focus is on automatic methods which segments objects that are visually and motion salient in videos. We specifically focus on two-stream models that learn multi-modal fusion between motion and appearance features. Then study the effect of haing no cross connections, against cross connections motion-to-appearance and bidirectional. We study these different types of models with our framework to provide further key findings and shared insights among both tasks. 
Limited work has been dedicated to the interpretability of spatiotemporal models. Several efforts predicate model interpretation on proxy tasks, \eg dynamic texture recognition~\cite{hadji2018new} or future frame selection~\cite{ghodrati2018video}. These approaches do not interpret the learned representations in the intermediate layers and in some cases require training to be performed on specific datasets~\cite{hadji2018new}. Work also has appeared that introduced a dataset to completely decouple static and dynamic information, but used it only to examine overall architecture performance on action recognition and did not examine intermediate representations~\cite{ilic2022appearance}. Other work focused on understanding latent representations in spatiotemporal models either mostly concerned qualitative visualization~\cite{feichtenhofer2020deep} or a specific architecture type~\cite{zhao2021interpretable}. A related task is understanding the scene representation bias of action recognition datasets~\cite{li2018resound, li2019repair}. %, which is quantified by the ratio of correct action classifications using a pretrained scene classification model. 
%Various techniques have been proposed to overcome such scene biases~\cite{li2018resound, li2019repair}. 
% \blue{Kosta: We are being inconsistent with the use of the term ``metric''.  It is not a metric in the mathematical sense.  Anyways, we need to pick a term and stick with it.}
However, these efforts did not focus on the effect of different architectural inductive biases on the learned intermediate representations. Our proposed interpretability technique is
%, to the best of our knowledge, 
the first to \emph{quantify} static and dynamic biases on \textit{intermediate} representations learned in off-the-shelf models for multiple video-based tasks. Most prior efforts focused on a single task, and studied either datasets~\cite{li2018resound} or architectures~\cite{feichtenhofer2020deep,manttari2020interpreting}. In contrast, our unified study covers seven datasets and dozens of architectures on three different tasks, \ie action recognition, AVOS and VIS. 

%%%%%%% Related Work I ommitted for space reasons
%1- or the performance ratio between original and temporally perturbed clips through reverse or freeze operations\cite{manttari2020interpreting}

%2- A recent work~\cite{sevilla2021only} has discussed the bias in the current video recognition datasets towards appearance, and proposed splits based on human annotators to define temporal and static action classes. We also study the effect of the dataset on static/dynamic bias, but we rather study it from an interpretability point of view on the intermediate representation without relying on external human annotations. 

%3- In a recent work~\cite{zhao2021interpretable}, a quantifiable interpretability method was proposed for future prediction models relying on kernel motion transformations, but is dependant on specific motion kernels and thus it can not be extended to any off-the-shelf spatiotemporal model.

%4- proxy tasks, or others~\cite{manttari2020interpreting}

\noindent \textbf{Spatiotemporal models.} Deep spatiotemporal models that learn discriminative features across space and time have proven effective for %in a wide range of 
video understanding tasks~\cite{aafaq2019video,zhu2020comprehensive}. 
Extant models 
%The architecture design of these models 
can be broadly categorized (agnostic of the downstream task) into: two-stream approaches that separately model motion and appearance features~\cite{carreira2017quo,jain2017fusionseg,zhou2020motion,ren2021reciprocal,feichtenhofer2019slowfast}, 
3D convolutions that jointly model motion and appearance~\cite{carreira2017quo},
%models relying on 3D convolutions~\cite{carreira2017quo}, 
attention-based models with different forms of spatiotemporal data association~\cite{bertasius2021space,ren2021reciprocal}, models relying on recurrent neural networks~\cite{tokmakov2017learning} and hybrid models that combine elements of the aforementioned models~\cite{tokmakov2017learning,carreira2017quo, ren2021reciprocal}. 
%The majority of these models learn hierarchical static and dynamic features in a distributed and end-to-end fashion.
% \noindent \textbf{Action recognition.}
% Classifying human actions is a longstanding open problem in computer vision. After the breakthrough performance of AlexNet [CITE] on ImageNet [CITE], many researchers have found success using DNNs for video-based tasks as well, including action recognition. Soon after this breakthrough, traditional hand-crafted techniques were soon outperformed by DNN architectures trained on vast amounts of data in an end-to-end manner. 
%Many of the first deep learning approaches for action recognition used recurrent neural networks with a 2D convolutional feature extractor as the backbone~\cite{karpathy2014large,ng2015beyond}. Since action recognition datasets were relatively small during that period, the 2D backbone allowed for ImageNet pretraining to be used and high quality features to be extracted. They were then fed into a recurrent layer, such as an LSTM [CITE], which could model long and short range temporal dependencies. However, another line of work which uses 3D convolutions to learn spatiotemporal representations of videos~\cite{taylor2010convolutional, ji20123d} generally tend to outperform recurrent architectures on action recognition datasets. Stacks of convolutional layers build up a hierarchy of spatiotemporal representations with an increasing effective receptive field in the temporal and spatial dimensions. Architectures of this form include C3D~\cite{tran2015learning}, I3D~\cite{carreira2017quo}, 3D-ResNets~\cite{hara2017learning}, and ResNet(2+1)D~\cite{tran2018closer} (which performs temporal and spatial convolutions in separate layers). 
%Rather than extract dynamic information implicitly (\eg, using 3D convolutions to learn motion features), another line of works used two-stream architectures. The general motivation is to capture appearance and motion information separately in each stream, followed by some method of combining the two types of information. Many works have used RGB as input to the appearance stream and optical flow for the motion stream. Methods of combining the two types of information include ... Motivated by the human visual stream, the SlowFast network~\cite{feichtenhofer2019slowfast} is a two stream 3D CNNs with a slow (appearance) and fast (motion) stream taking only RGB images as the input. The slow branch is a 3D ResNet like architecture, while the fast branch has the same number of layers as the slow branch, but only 1/8th of the channels and a sampling rate four times larger, encouraging less static information to be captured. One of the main issues with 3D CNNs is their vast number of parameters, which can be orders of magnitude larger than their 2D counterparts. 
%Attention based architectures have proven to be a flexible architecture suited for both static and time-series visual data. In particular, different variants of the Transformer have achieved state-of-the-art performance on almost all action recognition benchmarks [CITE]. Attention-based architectures have weaker inductive biases than convolutional based architectures. This causes them to be generally less sample efficient but potentially able to learn more useful invariances of video-based data than 3D convolutions. The best type of attention layer for action recognition is an exploding topic, with multiple variants appearing within the last two years including the Video Transformer, TimeSformer, ViVit, and MotionFormer, all of which claimed state-of-the-art over the preceding transformer variant. 
% \blue{Strong concluding statement.} 
Our approach to quantifying bias is not limited to the particulars of a model and is applicable to all extant and future models. We empirically demonstrate the flexibility of our approach by evaluating a diverse set of models.


\begin{figure*}[t]
    \includegraphics[width=\textwidth]{images/main_method.drawio.pdf}
    \vspace{-0.8cm}
    \caption{Overview of our methodology for analysing bias toward static or dynamic information. We measure the dynamic and static biases in deep spatiotemporal models for three tasks: action recognition, automatic video object segmentation and video instance segmentation. \textbf{(1)} We sample video pairs that share either \textit{static}, $(v^S_1, v^S_2)$, or \textit{dynamic}, ($v^D_1,v^D_2$), information using video stylization~\cite{texler2020interactive} and frame shuffling or optical flow jitter (flow visualized in RGB format). \textbf{(2)} Given a pretrained model, $f_\theta$, we compute the mutual information (MI) between intermediate representations of video pairs, $z^F$, to assess the model's bias toward either factor on a per-layer, $l$, or per-channel (\ie unit) basis. }
    \label{fig:mainmethod}
    \vspace{-0.6cm}
\end{figure*}

\noindent{\bf Action recognition.} 
3D convolutional networks are popular for learning 
%Early methods for action recognition used 3D convolutions 
spatiotemporal representations of videos for action recognition, \eg~\cite{taylor2010convolutional, ji20123d,tran2015learning,carreira2017quo,hara2017learning}. 
%Stacks of convolutional layers build up a hierarchy of spatiotemporal representations with an increasing effective receptive field in the temporal and spatial dimensions. Architectures of this form include C3D~\cite{tran2015learning}, I3D~\cite{carreira2017quo}, 3D-ResNets~\cite{hara2017learning}, and ResNet(2+1)D~\cite{tran2018closer}. 
Other work has considered two-stream architectures,
where the dynamics were provided directly to one of the streams as optical flow, \eg~\cite{simonyan2014two,feichtenhofer2017spatiotemporal}.
%rather than extracting dynamic information implicitly (\eg, using 3D convolutions). 
Representative of the state-of-the-art with convolutional networks is SlowFast~\cite{feichtenhofer2019slowfast}, which
is a two-stream 3D CNN that only takes RGB videos as input.
To encourage each stream to specialize in capturing predominately static or dynamic information, 
the temporal sampling rates of the inputs to each stream differ.
% its input differs from the other in temporal sampling rate.
%Each stream samples the input imagery differently to encourage the network to specialize 
%The fast stream has lower capacity and higher sampling rate than the slow stream, to encourage less static and more dynamic information to be captured. 
Recently, attention based approaches have proven to be suited to both static and time-series visual data, including action recognition, with variants of the transformer architecture~\cite{vaswani2017attention,bertasius2021space,fan2021multiscale,patrick2021keeping}.

%Motivated by the human visual system~\cite{goodale1992separate}, 
%the SlowFast network~\cite{feichtenhofer2019slowfast} was proposed as a two stream 3D CNN with a slow and a fast stream taking only RGB images as the input. The fast stream has lower capacity and higher sampling rate than the slow stream, to encourage less static and more dynamic information to be captured. Recently, attention based architectures have proven to be a flexible architecture suited for both static and time-series visual data with different variants of the Transformer architecture~\cite{vaswani2017attention,bertasius2021space,fan2021multiscale,patrick2021keeping}. %Attention-based architectures have weaker inductive biases than convolutional based architectures which results in a less sample efficient model but is potentially able to learn more useful invariances of video-based data than 3D convolutions.

% \noindent \textbf{Video object segmentation.} 
\noindent{\bf Video segmentation.} Deep video segmentation approaches can be categorized into two categories~\cite{wang2021survey}: (i) class agnostic, which are referred to as video object segmentation (VOS) and (ii) video semantic segmentation, which predict different semantic categories. Video semantic segmentation has been investigated with both instance-agnostic~\cite{gadde2017semantic} and instance-aware~\cite{wang2021end} approaches, where the latter is referred to as video instance segmentation (VIS)~\cite{wang2021end}. Video object segmentation methods can be categorized into automatic, semi-automatic and interactive~\cite{wang2021survey}. AVOS tries to segment the visual and motion salient objects in videos without a predefined mask initialization, while semi-automatic VOS requires mask initialization in the first frame to consequently track objects within a video. In this work, we mainly focus on AVOS approaches that segment salient objects in videos. 
% Since we study the dynamic bias of VOS models, we focus on automatic approaches as they are more relevant where motion is an important cue to capture the foreground objects.
%A related task is motion segmentation~\cite{dave2019towards}, which segments all moving objects regardless of its saliency. 
We consider two-stream models that fuse motion and appearance features. We also investigate the effect of no cross connections~\cite{jain2017fusionseg} relative to both motion-to-appearance~\cite{zhou2020motion} or bidirectional~\cite{ren2021reciprocal} cross connections. Additionally, we explore video instance segmentation approaches that use raw images as input to demonstrate the versatility of our methodology across different video segmentation tasks.
%Early deep learning models relied on optical flow to tackle automatic video segmentation~\cite{jain2017fusionseg,tokmakov2017learning}. In~\cite{jain2017fusionseg} a two-stream method with fusion on the final predictions from both motion and appearance streams was proposed. In~\cite{zhou2020motion} cross connections (i.e. motion-to-appearance) was proposed using attention blocks to leverage the interaction between motion and appearance. Finally, in~\cite{ren2021reciprocal} bidirectional cross connections were proposed and denoted as reciprocal transformations. %We focus on understanding the effect of cross connections on the static/dynamic biases.


==> core/results.tex <==
% \input{tex/graphs/ar_layer-wise}
\begin{figure*} [t]
%\vspace{-0.3cm}
	\begin{center}
     \centering
\begin{minipage}{0.58\textwidth}
		\resizebox{\textwidth}{!}{
\begin{tikzpicture}\ref{legend_all} \ref{legend_color}
    \begin{groupplot}[group style = {group size = 3 by 1, horizontal sep = 20pt}, width = 6.0cm, height = 6.4cm]
\nextgroupplot[
      line width=1.0,
        title={\textbf{(a) 3D CNNs}},
        title style={at={(axis description cs:0.5,0.92)},anchor=north},
        xlabel={Network Layer},
        % x label style={font=\small},
        ylabel={Number of Units (\%)},
        xmin=0.8, xmax=5.2,
        ymin=13, ymax=46,
        xtick={1,2,3,4,5},
        ytick={15, 20, 25, 30, 35, 40},
        x tick label style={font=\footnotesize},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.06)},anchor=north,font=\small}, 
        y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\normalsize},
        width=6.5cm,
        height=5cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        %legend style={
         %draw=none,
         %legend style={row sep=0.1pt},
        %  nodes={scale=0.7, transform shape},
        % cells={anchor=west},
        % legend columns=2,
        % legend style={at={(2.5,4)},anchor=south,row sep=0.01pt}, font =\small},
        % legend entries={[black]C2D-Dynamic,[black]C2D-Static,[black]I3D-Dynamic,[black]I3D-Static,[black]X3D-m-Dynamic,[black]X3D-m-Static},
        %legend to name=target_legend_3dcnn,
    ]
    % MOTION
    % c2d
    \addplot[line width=1.2pt,dashed,mark options={scale=0.8,solid},color=blue!100,mark=triangle*,]
        coordinates {(1,18.8)(2,20.3)(3,21.1)(4,21.0)(5,22.4)};
        % \label{pgfplots:c1r1}
    % APPEARANCE
        % c2d
    \addplot[line width=1.2pt,mark size=1.1pt,color=red!100,mark=triangle*,]
        coordinates {(1,39.1)(2,39.5)(3,38.9)(4,39.1)(5,37.1)};
        % \label{pgfplots:c2r1}
    % MOTION
        % I3D
    \addplot[line width=1.2pt,dashed,mark options={scale=0.8,solid},color=blue!100,mark=*,]
        coordinates {(1,17.2)(2,21.5)(3,21.9)(4,22.9)(5,23.0)};
        % \label{pgfplots:c1r2}
    % APPEARANCE
        % I3D
    \addplot[line width=1.2pt,mark options={scale=0.8,solid},color=red!100,mark=*,]
        coordinates {(1,40.6)(2,37.5)(3,38.1)(4,37.1)(5,35.2)};
        % \label{pgfplots:c2r2}
    % MOTION
        % X3D-m
    \addplot[line width=1.2pt,dashed,mark options={scale=1.5,solid},color=blue!100,mark=+,]
        coordinates {(1,16.7)(2,20.8)(3,22.9)(4,24.0)(5,23.4)};
        % \label{pgfplots:c1r3}
    % APPEARANCE
        % X3D-m
    \addplot[line width=1.2pt,mark options={scale=1.5,solid},color=red!100,mark=+,]
        coordinates {(1,37.5)(2,37.5)(3,35.4)(4,35.4)(5,35.9)};
        % \label{pgfplots:c2r3}

\nextgroupplot[
      line width=1.0,
        title={\textbf{(b) SlowFast}},
        title style={at={(axis description cs:0.5,0.92)},anchor=north,font=\normalsize},
        xlabel={Network Layer},
        % x label style={font=\small},
        %ylabel={Bias (\%)},
        % ylabel={Number of Units (\%)},
        xmin=0.8, xmax=5.2,
        ymin=10, ymax=48,
        xtick={1,2,3,4,5},
        ytick={15, 20, 25, 30, 35, 40},
        x tick label style={font=\footnotesize},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.06)},anchor=north,font=\small},   %y label style={at={(axis description cs:0.15,.5)},anchor=south,font=\normalsize},
        width=6.5cm,
        height=5cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
        nodes={scale=0.87, transform shape},
        cells={anchor=west},
        legend style={at={(2,3.6)},anchor=south,row sep=0.01pt}, font =\normalsize},
        legend image post style={scale=0.9},
        legend columns=2,
        legend to name=legend_color,
    ]
    % % SFSLOW Motion
    \addplot[line width=1pt,dashed,mark options={scale=0.9,solid},color=blue!100,mark=diamond*,forget plot]
        coordinates {(1,17.5)(2,20.0)(3,21.9)(4,26.0)(5,24.7)};
        % \label{pgfplots:c1r4}
    % % SFSLOW App
    \addplot[line width=1pt,mark options={scale=0.9,solid},color=red!100,mark=diamond*,forget plot]
        coordinates {(1,40.0)(2,38.8)(3,37.0)(4,32.3)(5,33.3)};
        % \label{pgfplots:c2r4}
    % % SFFAST Motion
    \addplot[line width=1pt,dashed,mark options={scale=1.5,solid},color=blue!100,mark=x,forget plot]
        coordinates {(1,12.5)(2,28.1)(3,29.7)(4,31.2)(5,34.0)};
        % \label{pgfplots:c1r5}
    % % SFFAST App
    \addplot[line width=1pt,mark options={scale=1.5,solid},color=red!100,mark=x,forget plot]
        coordinates {(1,25.0)(2,28.1)(3,25.0)(4,25.0)(5,23.0)};
        % \label{pgfplots:c2r5}
    % MOTION
    % SlowOnly 8x8
    \addplot[line width=1pt,dashed,mark options={scale=0.8,solid},color=blue!100,mark=square*,forget plot]
        coordinates {(1,17.2)(2,18.8)(3,20.1)(4,22.5)(5,21.4)};
        % \label{pgfplots:c1r6}
    % APPEARANCE
        % SlowOnly 8x8
    \addplot[line width=1pt,mark options={scale=0.8,solid},color=red!100,mark=square*,forget plot]
        coordinates {(1,40.6)(2,40.6)(3,39.6)(4,37.9)(5,38.4)};
        % \label{pgfplots:c2r6}
    % MOTION
    % FastOnly
    \addplot[line width=1pt,dashed,mark options={scale=1.5,solid},color=blue!100,mark=|,forget plot]
        coordinates {(1,12.5)(2,18.8)(3,21.9)(4,23.4)(5,27.3)};
        % \label{pgfplots:c1r7}
    % APPEARANCE
    % FastOnly
    \addplot[line width=1pt,mark options={scale=1.5,solid},color=red!100,mark=|,forget plot]
        coordinates {(1,37.5)(2,37.5)(3,32.8)(4,32.8)(5,30.9)};
        % \label{pgfplots:c2r7}
    
    \addlegendimage{line width=1.2pt,color=red}\label{pgfplots:ar_stat}
    \addlegendentry[color=black]{Static}
    \addlegendimage{line width=1.2pt,dashed,color=blue}\label{pgfplots:ar_dyn}
    \addlegendentry[color=black]{Dynamic}
          
\nextgroupplot[
      line width=1.0,
        title={\textbf{(c) Transformers}},
        title style={at={(axis description cs:0.5,0.92)},anchor=north,font=\normalsize},
        xlabel={Network Layer},
        % x label style={font=\small},
        % ylabel={Bias (\%)},
        xmin=0, xmax=17,
        ymin=15, ymax=48,
        xtick={1,3,5,7,9,11,13,15},
        ytick={20, 25, 30, 35, 40},
        % xticklabels={MSA1,MSA2,MSA3,MSA,MSA1,MSA1,MSA1,MSA1,MSA1,MSA1,MSA1,MSA1},
        x tick label style={font=\footnotesize},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.06)},anchor=north,font=\small},
        %y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
        width=6.5cm,
        height=5cm,         
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
        %  draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(10,3.6)},anchor=south,row sep=0.01pt}, font =\normalsize},
        legend to name=legend_all,
    ]
    % MOTION
    % MViT
    \addplot[line width=1pt,dashed,mark options={scale=1,solid},color=blue!100,mark=pentagon*,forget plot]
        coordinates {(1,22.9)(2,24.5)(3,27.1)(4,25.8)(5,25.3)(6,26.6)(7,27.1)(8,27.1)(9,26.6)(10,26.0)(11,26.0)(12,26.8)(13,25.8)(14,25.8)(15,25.0)(16,25.0)};
        % \label{pgfplots:c1r8}
    % APPEARANCE
    % MViT
    \addplot[line width=1pt,mark options={scale=1,solid},color=red!100,mark=pentagon*,forget plot]
        coordinates {(1,36.5)(2,35.9)(3,33.9)(4,34.6)(5,33.6)(6,33.6)(7,33.6)(8,34.1)(9,34.4)(10,34.4)(11,34.4)(12,33.6)(13,34.6)(14,33.2)(15,33.3)(16,32.7)};
        % \label{pgfplots:c2r8}
            % MOTION
    % TimeSformer
    \addplot[line width=1pt,dashed,mark options={line width=0.5pt,scale=1.3,solid},color=blue!100,mark=star,forget plot]
        coordinates {(1,18.5)(2,19.1)(3,19.4)(4,20.1)(5,21.7)(6,24.6)(7,25.7)(8,25.5)(9,24.5)(10,24.2)(11,23.6)(12,22.0)};
        % \label{pgfplots:c1r9}
    % APPEARANCE
    % TimeSformer
    \addplot[line width=1pt,mark options={scale=1.3,solid},color=red!100,mark=star,forget plot]
        coordinates {(1,40.6)(2,40.4)(3,40.2)(4,39.8)(5,38.8)(6,37.9)(7,37.1)(8,36.8)(9,37.9)(10,37.8)(11,37.9)(12,38.8)};
    % \label{pgfplots:c2r9}

%%%%%%%%%%%%%%% legend
    
    \addlegendimage{only marks,mark=triangle*,mark size=2.2pt,color=black!70}\label{pgfplots:ar_c1r1}
\addlegendentry[color=black]{C2D  \hspace{1cm}}
    \addlegendimage{only marks,mark=*,mark size=2.1pt,color=black!70}\label{pgfplots:ar_c1r2}
\addlegendentry[color=black]{I3D  \hspace{1cm}}
    \addlegendimage{only marks,mark=+,mark size=2.5pt,color=black!90}\label{pgfplots:ar_c1r3}
\addlegendentry[color=black]{X3D  \hspace{1cm}}
    \addlegendimage{only marks,mark=diamond*,mark size=2.3pt,color=black!70}\label{pgfplots:ar_c1r4}
\addlegendentry[color=black]{SF-Slow  \hspace{1cm}}
    \addlegendimage{only marks,mark=x,mark size=2.6pt,color=black!90}\label{pgfplots:ar_c1r5}
\addlegendentry[color=black]{SF-Fast  \hspace{1cm}}
    \addlegendimage{only marks,mark=square*,mark size=2pt,color=black!70}\label{pgfplots:ar_c1r6}
\addlegendentry[color=black]{SlowOnly  \hspace{1cm}}
    \addlegendimage{only marks,mark=|,mark size=3pt,color=black!90}\label{pgfplots:ar_c1r7}
\addlegendentry[color=black]{FastOnly  \hspace{1cm}}
    \addlegendimage{only marks,mark=pentagon*,mark size=2.2pt,color=black!70}\label{pgfplots:ar_c1r8}
\addlegendentry[color=black]{MViT  \hspace{1cm}}
    \addlegendimage{only marks,mark=star,mark size=2.6pt,color=black!90}\label{pgfplots:ar_c1r9}
\addlegendentry[color=black]{TimeSformer  \hspace{1cm}}

% \addlegendimage{area legend,fill=red!100,color=red}\label{pgfplots:ar_stat}
% \addlegendimage{area legend,fill=blue!100,color=blue}\label{pgfplots:ar_dyn}
\end{groupplot}
% \node[draw,fill=white,inner sep=0pt,above left=0.5em] at ($(group c2r1) + (8, -3.5cm)$) {\small
%         \begin{tabular}{ccc||cccc||ccc}
%               C2D\ref{pgfplots:ar_c1r1}  & I3D\ref{pgfplots:ar_c1r2} & X3D\ref{pgfplots:ar_c1r3} & SF-Slow\ref{pgfplots:ar_c1r4} & SF-Fast\ref{pgfplots:ar_c1r5} & SlowOnly\ref{pgfplots:ar_c1r6} & FastOnly\ref{pgfplots:ar_c1r7} & MViT\ref{pgfplots:ar_c1r8} & TimesFormer\ref{pgfplots:ar_c1r9}\\
%     \end{tabular}};
% \node[draw,fill=white,inner sep=0pt,above left=0.5em] at ($(group c2r1) + (-5.2, -3.5cm)$) {\small
%         \begin{tabular}{ccc||cccc||ccc}
%               Static & \ref{pgfplots:ar_stat} \\
%               Dynamic & \ref{pgfplots:ar_dyn} \\
%     \end{tabular}};

%\begin{tabular}{lccc|cccc|ccc}
%               & C2D & I3D & X3D & SF-Slow & SF-Fast & SlowOnly & FastOnly & MViT & TimesFormer\\
%    Dynamic & \ref{pgfplots:c1r1} & \ref{pgfplots:c1r2} & \ref{pgfplots:c1r3}& \ref{pgfplots:c1r4} & \ref{pgfplots:c1r5} & \ref{pgfplots:c1r6}& \ref{pgfplots:c1r7} & \ref{pgfplots:c1r8} & \ref{pgfplots:c1r9}\\
%    Static & \ref{pgfplots:c2r1} & \ref{pgfplots:c2r2} & \ref{pgfplots:c2r3} & \ref{pgfplots:c2r4} & \ref{pgfplots:c2r5} & \ref{pgfplots:c2r6}&\ref{pgfplots:c2r7} & \ref{pgfplots:c2r8} & \ref{pgfplots:c2r9}\\
%    \end{tabular}};
    
\end{tikzpicture}
}
\end{minipage}%
\begin{minipage}{0.42\textwidth}
%\vspace{3em}
\resizebox{1.0\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     % width = \axisdefaultwidth,
%     width=7cm,
%     bar width = 7pt,
%     height=5.4cm,  
%     %draw=none,
%     xmin = 0,
%     xmax = 100,
%   % title = \textbf{Individual Unit Analysis on Action Recognition Architectures},
%     x label style={at={(axis description cs:0.5,0.05)},anchor=north,font=\small},
%     xlabel = Units Encoding Factor F (\%),
%     ytick=data,
%     legend style={
%             draw = none,
% 			area legend,
% 			at={(0.5,1.17)},
% 			anchor=north,
% 			legend columns=-1},
%     symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
%     enlarge x limits = {value = .1},
%     % enlarge y limits={abs=12pt}
% ]

% % \addplot coordinates {(0,C2D) [0] (0.1,I3D) [2] (0,MViT) [0] (0,TimeSf) [0] (0.1,SlowOnly) [2] (0.3,SF-Slow) [6] (9.0,FastOnly) [23] (39.5,SF-Fast) [101]}; % dynamic
% \addplot coordinates {(0,C2D) [0] (0.1,I3D) [2] (0,MViT) [0] (0,TimeSf) [0] (0.1,SlowOnly) [2] (0.3,SF-Slow) [6] (20.3125,FastOnly) [23] (37.890625,SF-Fast) [101]}; % dynamic



% \addplot coordinates {(82.2,C2D) [1684] (86.3,I3D) [1767] (75,MViT) [576] (89.2,TimeSf) [685] (81.4,SlowOnly) [1668] (64.9,SF-Slow) [1329] (23.046875,FastOnly) [82] (30.078125,SF-Fast) [72]}; % static

% \addplot coordinates {(17.8,C2D) [364] (13.6,I3D) [278] (25,MViT) [192] (10.8,TimeSf) [83] (18.5,SlowOnly) [378] (34.7,SF-Slow) [710] (46.09375,FastOnly) [149] (29.296875,SF-Fast) [78]}; % joint

% \addplot coordinates {(0,C2D) [0] (0.05,I3D) [1] (0,MViT) [0] (0,TimeSf) [0] (0,SlowOnly) [0] (0.14,SF-Slow) [3] (10.546875,FastOnly) [2] (2.734375,SF-Fast) [5]}; % none


% \legend {Dynamic,Static,Joint,Residual};
% \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.5cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Stage 5},
    title style={at={(axis description cs:0.5,1.12)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    % ytick style = {font=\large}
%     legend style={
% 			area legend,
% 			at={(0.5,1.2)},
% 			anchor=north,
% 			legend columns=-1},
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.35)},anchor=north,row sep=0.01pt}, font =\large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=4pt}
]

\addplot coordinates {(0,C2D) [0] (0.1,I3D) [2] (0,MViT) [0] (0,TimeSf) [0] (0.1,SlowOnly) [2] (0.3,SF-Slow) [6] (20.3125,FastOnly) [23] (37.890625,SF-Fast) [101]}; % dynamic
\addplot coordinates {(82.2,C2D) [1684] (86.3,I3D) [1767] (75,MViT) [576] (89.2,TimeSf) [685] (81.4,SlowOnly) [1668] (64.9,SF-Slow) [1329] (23.046875,FastOnly) [82] (30.078125,SF-Fast) [72]}; % static
\addplot coordinates {(17.8,C2D) [364] (13.6,I3D) [278] (25,MViT) [192] (10.8,TimeSf) [83] (18.5,SlowOnly) [378] (34.7,SF-Slow) [710] (46.09375,FastOnly) [149] (29.296875,SF-Fast) [78]}; % joint
\addplot coordinates {(0,C2D) [0] (0.05,I3D) [1] (0,MViT) [0] (0,TimeSf) [0] (0,SlowOnly) [0] (0.14,SF-Slow) [3] (10.546875,FastOnly) [2] (2.734375,SF-Fast) [5]}; % none

% \addplot coordinates {(0.09765625,SlowOnly) (0.29296875,SF-Slow) (37.890625,SF-Fast) (20.3125,FastOnly) (0.0,MViT)};
% \addplot coordinates {(78.41796875,SlowOnly) (64.94140625,SF-Slow) (30.078125,SF-Fast) (23.046875,FastOnly) (76.5625,MViT)};
% \addplot coordinates {(21.484375,SlowOnly) (34.619140625,SF-Slow) (29.296875,SF-Fast) (46.09375,FastOnly) (23.4375,MViT)};
% \addplot coordinates {(0.0,SlowOnly) (0.146484375,SF-Slow) (2.734375,SF-Fast) (10.546875,FastOnly) (0.0,MViT)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture} 
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.5cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Stage 4},
    title style={at={(axis description cs:0.5,1.12)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
% 			legend columns=-1},
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.35)},anchor=north,row sep=0.01pt}, font =\large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=4pt}
]

\addplot coordinates {(0,C2D) (0.1,I3D) (0.48828125,SlowOnly) (0,TimeSf) (14.53125,SF-Slow) (41.40625,SF-Fast) (39.0625,FastOnly) (0.13020833333333334,MViT)};
\addplot coordinates {(56,C2D) (45.02,I3D) (41.015625,SlowOnly) (85.9,TimeSf) (36.71875,SF-Slow)  (3.125,SF-Fast) (6.25,FastOnly) (43.619791666666664,MViT)};
\addplot coordinates {(44,C2D) (54.88,I3D) (58.49609375,SlowOnly) (14.1,TimeSf) (48.671875,SF-Slow) (55.46875,SF-Fast) (49.21875,FastOnly) (56.25,MViT)};
\addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.078125,SF-Slow) (0.0,SF-Fast) (5.46875,FastOnly) (0.0,MViT)};
\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\vfill
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.5cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Stage 3},
    title style={at={(axis description cs:0.5,1.12)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    xlabel style = {font=\large,at={(axis description cs:0.5,0.07)}},
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=4pt}
]

\addplot coordinates {(0,C2D) (0.6,I3D) (0.0,SlowOnly) (0,TimeSf) (8.59375,SF-Slow) (20.3125,SF-Fast) (26.5625,FastOnly) (0.78125,MViT)};
\addplot coordinates {(56.05,C2D) (48.2,I3D) (61.71875,SlowOnly) (85.8,TimeSf) (50.15625,SF-Slow) (9.375,SF-Fast) (17.1875,FastOnly) (29.166666666666668,MViT)};
\addplot coordinates {(43.9,C2D) (51.2,I3D) (38.28125,SlowOnly) (14.2,TimeSf) (40.78125,SF-Slow) (68.75,SF-Fast) (48.4375,FastOnly) (69.53125,MViT)};
\addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.46875,SF-Slow) (1.5625,SF-Fast) (7.8125,FastOnly) (0.5208333333333334,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.5cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Stage 2},
    title style={at={(axis description cs:0.5,1.12)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    xlabel style = {font=\large,at={(axis description cs:0.5,0.07)}},
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=4pt}
]

\addplot coordinates {(0,C2D) (1.2,I3D) (0.0,SlowOnly) (0,TimeSf) (6.5625,SF-Slow) (18.75,SF-Fast) (15.625,FastOnly) (1.8229166666666667,MViT)};
\addplot coordinates {(77.7,C2D) (63.3,I3D) (78.90625,SlowOnly) (93,TimeSf) (66.875,SF-Slow) (6.25,SF-Fast) (31.25,FastOnly) (38.541666666666664,MViT)};
\addplot coordinates {(22.3,C2D) (35.5,I3D) (21.09375,SlowOnly) (7,TimeSf) (25.9375,SF-Slow) (75.0,SF-Fast) (43.75,FastOnly) (58.333333333333336,MViT)};
\addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.625,SF-Slow) (0.0,SF-Fast) (9.375,FastOnly) (1.3020833333333333,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\end{minipage}%
	\end{center}
	\vspace{-0.5cm}
	\caption{Layer and unit-wise analyses on action recognition networks trained on Kinetics-400~\cite{carreira2017quo}. \textbf{Left:} Layer-wise encoding of static and dynamic factors using the layer-wise metric, (\ref{eq:biasscores}), for: (a) single stream 3D CNNs, (b) SlowFast variants and (c) transformer variants. SF-Slow and SF-Fast denote the representation taken before the fusion layer from the slow and fast branches, resp. \textbf{Right:} Estimates of the dynamic, static, joint and residual units using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}).
% 	Since models have different numbers of channels, the number of units are normalized to the graph width.
	}\label{fig:stagewise_ar_all_models}
	\vspace{-0.7cm}
\end{figure*}






% \begin{figure}[t]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.5cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 5},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     % ytick style = {font=\large}
% %     legend style={
% % 			area legend,
% % 			at={(0.5,1.2)},
% % 			anchor=north,
% % 			legend columns=-1},
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=4pt}
% ]

% \addplot coordinates {(0,C2D) [0] (0.1,I3D) [2] (0,MViT) [0] (0,TimeSf) [0] (0.1,SlowOnly) [2] (0.3,SF-Slow) [6] (20.3125,FastOnly) [23] (37.890625,SF-Fast) [101]}; % dynamic
% \addplot coordinates {(82.2,C2D) [1684] (86.3,I3D) [1767] (75,MViT) [576] (89.2,TimeSf) [685] (81.4,SlowOnly) [1668] (64.9,SF-Slow) [1329] (23.046875,FastOnly) [82] (30.078125,SF-Fast) [72]}; % static
% \addplot coordinates {(17.8,C2D) [364] (13.6,I3D) [278] (25,MViT) [192] (10.8,TimeSf) [83] (18.5,SlowOnly) [378] (34.7,SF-Slow) [710] (46.09375,FastOnly) [149] (29.296875,SF-Fast) [78]}; % joint
% \addplot coordinates {(0,C2D) [0] (0.05,I3D) [1] (0,MViT) [0] (0,TimeSf) [0] (0,SlowOnly) [0] (0.14,SF-Slow) [3] (10.546875,FastOnly) [2] (2.734375,SF-Fast) [5]}; % none

% % \addplot coordinates {(0.09765625,SlowOnly) (0.29296875,SF-Slow) (37.890625,SF-Fast) (20.3125,FastOnly) (0.0,MViT)};
% % \addplot coordinates {(78.41796875,SlowOnly) (64.94140625,SF-Slow) (30.078125,SF-Fast) (23.046875,FastOnly) (76.5625,MViT)};
% % \addplot coordinates {(21.484375,SlowOnly) (34.619140625,SF-Slow) (29.296875,SF-Fast) (46.09375,FastOnly) (23.4375,MViT)};
% % \addplot coordinates {(0.0,SlowOnly) (0.146484375,SF-Slow) (2.734375,SF-Fast) (10.546875,FastOnly) (0.0,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.5cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 4},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
% % 			legend columns=-1},
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=4pt}
% ]

% \addplot coordinates {(0,C2D) (0.1,I3D) (0.48828125,SlowOnly) (0,TimeSf) (14.53125,SF-Slow) (41.40625,SF-Fast) (39.0625,FastOnly) (0.13020833333333334,MViT)};
% \addplot coordinates {(56,C2D) (45.02,I3D) (41.015625,SlowOnly) (0,TimeSf) (36.71875,SF-Slow)  (3.125,SF-Fast) (6.25,FastOnly) (43.619791666666664,MViT)};
% \addplot coordinates {(44,C2D) (54.88,I3D) (58.49609375,SlowOnly) (0,TimeSf) (48.671875,SF-Slow) (55.46875,SF-Fast) (49.21875,FastOnly) (56.25,MViT)};
% \addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.078125,SF-Slow) (0.0,SF-Fast) (5.46875,FastOnly) (0.0,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.5cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 3},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     xlabel style = {font=\large},
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=4pt}
% ]

% \addplot coordinates {(0,C2D) (0.6,I3D) (0.0,SlowOnly) (0,TimeSf) (8.59375,SF-Slow) (20.3125,SF-Fast) (26.5625,FastOnly) (0.78125,MViT)};
% \addplot coordinates {(0,C2D) (48.2,I3D) (61.71875,SlowOnly) (0,TimeSf) (50.15625,SF-Slow) (9.375,SF-Fast) (17.1875,FastOnly) (29.166666666666668,MViT)};
% \addplot coordinates {(0,C2D) (51.2,I3D) (38.28125,SlowOnly) (0,TimeSf) (40.78125,SF-Slow) (68.75,SF-Fast) (48.4375,FastOnly) (69.53125,MViT)};
% \addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.46875,SF-Slow) (1.5625,SF-Fast) (7.8125,FastOnly) (0.5208333333333334,MViT)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=4.5cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 2},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     xlabel style = {font=\large},
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={C2D, I3D, MViT, TimeSf, SlowOnly, SF-Slow, FastOnly, SF-Fast},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=4pt}
% ]

% \addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (6.5625,SF-Slow) (18.75,SF-Fast) (15.625,FastOnly) (1.8229166666666667,MViT)};
% \addplot coordinates {(0,C2D) (0,I3D) (78.90625,SlowOnly) (0,TimeSf) (66.875,SF-Slow) (6.25,SF-Fast) (31.25,FastOnly) (38.541666666666664,MViT)};
% \addplot coordinates {(0,C2D) (0,I3D) (21.09375,SlowOnly) (0,TimeSf) (25.9375,SF-Slow) (75.0,SF-Fast) (43.75,FastOnly) (58.333333333333336,MViT)};
% \addplot coordinates {(0,C2D) (0,I3D) (0.0,SlowOnly) (0,TimeSf) (0.625,SF-Slow) (0.0,SF-Fast) (9.375,FastOnly) (1.3020833333333333,MViT)};
% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (\ref{eq:ind_bias_scores_diff_b}), $\lambda=0.5$, for models trained on Kinetics-400~\cite{goyal2017something}. We compare SlowOnly, SlowFast, FastOnly, and MViT at different layers. Since MViT has 16 layers, we estimate the dimensionality at layers 6, 9, 13, 16.}
% \label{fig:ar_perunit_alllayers}
% \end{figure}



We choose the tasks of action recognition, AVOS, and VIS to demonstrate the generality of our approach. They differ in their semantics (\ie multi-class \vs binary \vs instance-based), labelling (\ie video-level \vs pixel-level), and input types (multi-frame images \vs single frame and optical flow). We explore five main research questions and show the corresponding results with respect to our quantitative techniques for both tasks: (i) What is the effect of the model architecture on the \textit{static} and \textit{dynamic} biases (Sec.~\ref{sec:architectures})? (ii) What effect does the training dataset have on \textit{static} and \textit{dynamic} biases (Sec.~\ref{sec:dataset_effect})? (iii) What are the characteristics of jointly encoding units in relation to model architectures and datasets (Sec.~\ref{sec:architectures} and~\ref{sec:dataset_effect})?  (iv) When are static and dynamic biases learned during training (Sec.~\ref{sec:epoch_effect})? (v) What is the effect of static and dynamic biased units on performance (Sec.~\ref{sec:neuron_removal})? Finally, we demonstrate two approaches where we use our insights to improve the performance of action recognition (Sec.~\ref{sec:staticdropout}) and AVOS models (Sec.~\ref{sec:vos_cc_study}).

%  Details. and (iii) do benchmark datasets that are claimed to be heavily biased to \textit{dynamics} (\eg, Diving48~\cite{li2018resound}) actually require dynamic information?. 
% renouncing widely known assumption on certain datasets being dynamicly bias is described in section~\ref{sec:dataset_effect}.
% \input{tex/graphs/ar_models}

\vspace{-0.3cm}
\subsection{Model architectures}
\label{sec:architectures}

\subsubsection{Action recognition}\label{sec:ar_models}
\noindent\textbf{Architectures.} 
% As the field of action recognition has largely moved away from explicit input motion representations (\eg optical flow), we restrict our analysis to models that solely use the RGB modality. 
We study three types of models with respect to their static and dynamic biases: (i) single stream 3D CNNs (\ie C2D~\cite{wang2018non}, I3D~\cite{carreira2017quo} and X3D~\cite{feichtenhofer2020x3d} models), (ii) SlowFast~\cite{feichtenhofer2019slowfast} variations, where the individual streams are referred to as the SlowOnly and FastOnly models and (iii) transformer-based architectures~\cite{fan2021multiscale,bertasius2021space}. For all models, the number of frames and sampling rate is ($8\times8$), except for the FastOnly network ($32\times2$), MViT ($16\times4$), and TimeSformer ($8\times32$). To identify the static and dynamic units of all models, we generate the Stylized ActivityNet~\cite{caba2015activitynet} validation set and use it for sampling \textit{static} and \textit{dynamic} pairs. We choose this dataset since the action distribution is similar to Kinetics-400, yet much smaller in size making it memory efficient when computing our metrics.

\noindent\textbf{Implementation details.} All models were taken from the SlowFast~\cite{feichtenhofer2019slowfast} repository\footnote{\url{https://github.com/facebookresearch/SlowFast}} except the TimeSformer~\cite{bertasius2021space}, which has its own codebase\footnote{\url{https://github.com/facebookresearch/TimeSformer}}. All model weights trained on Kinetics-400~\cite{carreira2017quo} and Something-Something-v2~\cite{goyal2017something} (SSv2) are taken directly from the SlowFast repository, except for the FastOnly model which we train ourselves. The FastOnly model is trained for 40 epochs on Kinetics-400 with SGD, a weight decay of 1e-4, a batch size of 32 and a base learning rate of 0.03 that decreases by a factor of 10 at epochs 15, 30 and 35. On SSv2, the FastOnly model is trained for 25 epochs with SGD, weight decay of 1e-4, a batch size of 32 and a base learning rate that is decreased by a factor of 10 at epochs 10 and 20. On Diving48~\cite{li2018resound} the FastOnly model is trained for 100 epochs with SGD, weight decay of 1e-4, a batch size of 32 and a base learning rate of 0.0375 that decreases by a factor of 10 at epochs 40, 60 and 80. The SlowOnly model is trained on Diving48 for 100 epochs with SGD, weight decay of 1e-4, a batch size of 32 and a base learning rate of 0.00375 that decreases by a factor of 10 at epochs 40, 60 and 80. All models trained with temporal frame shuffling (see Sec.~\ref{sec:ar_dataset}) incur the same hyperparameters as their unshuffled counterparts.

%trained on Kinetics-400

%%%%%% PREVIOUS VERSION WITH LARGE SINGLE LAST LAYER PLOT
% The SlowFast network~\cite{feichtenhofer2019slowfast} is a two stream model with a fast and slow stream, that differ in the number of channels and the input frame rate. The intuition is that the fast stream should use a higher frame rate to capture detailed dynamic information but does not have as many channels that are required for capturing static information. We also study the two streams when trained individually, referred to as the SlowOnly and FastOnly models. Finally, we analyze two recent spatiotemporal attention-based architectures. The Multiscale Vision transformer (MViT)~\cite{fan2021multiscale} performs full spatiotemporal attention at each layer and reduces computation by pooling either the query or keys and values throughout the network. The TimeSformer~\cite{bertasius2021space} has no pooling and performs divided space-time attention at each layer. 



% \noindent\textbf{Architectures.} As the field of action recognition has largely moved away from explicit input motion representations (\eg, optical flow), we restrict our analysis to models that use solely the RGB modality. To this end, we study three types of models with respect to their static and dynamic biases: (i) single stream 3D CNNs, C2D~\cite{wang2018non}, I3D~\cite{carreira2017quo}, and X3D~\cite{feichtenhofer2020x3d} models, (ii) SlowFast~\cite{feichtenhofer2019slowfast} variations, where we also study the two streams when trained individually, referred to as the SlowOnly and FastOnly models, and (iii) transformer-based architectures~\cite{fan2021multiscale,bertasius2021space,feichtenhofer2020x3d}. All models in this subsection are trained on the Kinetics-400 dataset~\cite{carreira2017quo} and taken from the SlowFast repository~\cite{feichtenhofer2019slowfast} without any training or fine-tuning on our part (except FastOnly which we implement). For every architecture, we show the (number of frames $\times$ sampling rate), \eg, ($8\times8$). To identify the static and dynamic units of these models, we generate Stylized ActivityNet~\cite{caba2015activitynet} and use the validation set for sampling \textit{static} and \textit{dynamic} pairs. We choose this dataset since the action distribution is very similar to Kinetics-400, yet much smaller in size. 

% % The SlowFast network~\cite{feichtenhofer2019slowfast} is a two stream model with a fast and slow stream, that differ in the number of channels and the input frame rate. The intuition is that the fast stream should use a higher frame rate to capture detailed dynamic information but does not have as many channels that are required for capturing static information. We also study the two streams when trained individually, referred to as the SlowOnly and FastOnly models. Finally, we analyze two recent spatiotemporal attention-based architectures. The Multiscale Vision transformer (MViT)~\cite{fan2021multiscale} performs full spatiotemporal attention at each layer and reduces computation by pooling either the query or keys and values throughout the network. The TimeSformer~\cite{bertasius2021space} has no pooling and performs divided space-time attention at each layer. 

% The static and dynamic units, of the last layer before the linear layer, of multiple spatiotemporal models are quantified in Fig.~\ref{fig:ar_model_kin400} using~\eqref{eq:biasscores}. Interestingly, all single stream networks (\eg, I3D and C2D) are heavily biased toward \textit{static} information even though the video frames of the static pairs are \textit{randomly shuffled}. This demonstrates the heavy bias toward static feature representations in modern action recognition models. In fact, many of the models (\eg, I3D and SlowOnly) have a similar percentage of dynamic units as the C2D network. This finding further suggests that 3D convolutions by themselves (\eg, simply inflating a 2D kernel to 3D) is not sufficient to capture complex dynamic representations.
%%%%%% END



%\input{tex/graphs/vos_layer-wise_2}



% \begin{figure}[t]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.2cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 5},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(8.7890625,FusionSeg) (37.6953125,MATNet) (37.5244140625,MATNet*) (40.185546875,MATNet NoBAR) (49.560546875,MATNet NoYTB) (0.0,RTNet)};
% \addplot coordinates {(17.08984375,FusionSeg) (47.8515625,MATNet)  (44.62890625,MATNet*) (45.3857421875,MATNet NoBAR) (45.60546875,MATNet NoYTB) (1.171875,RTNet)};
% \addplot coordinates {(73.486328125,FusionSeg) (14.453125,MATNet) (17.8466796875,MATNet*) (14.4287109375,MATNet NoBAR) (4.736328125,MATNet NoYTB) (98.828125,RTNet)};
% \addplot coordinates {(0.634765625,FusionSeg) (0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.09,MATNet NoYTB) (0.0,RTNet)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \hfill
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.2cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 4},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     % xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
%          draw=none,
%          legend style={row sep=0.1pt},
%         nodes={scale=0.87, transform shape},
%         legend columns=-1,
%         cells={anchor=west},
%         legend style={at={(0.5,1.5)},anchor=north,row sep=0.01pt}, font =\large},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]

% \addplot coordinates {(28.6,MATNet) (33.7890625,MATNet*) (30.3,MATNet NoBAR) (46.044921875,MATNet NoYTB) (0.0,RTNet)};
% \addplot coordinates {(40.3,MATNet) (37.40234375,MATNet*) (39.0,MATNet NoBAR) (32.080078125,MATNet NoYTB) (65.6,RTNet)};
% \addplot coordinates {(31.1,MATNet) (28.80859375,MATNet*) (30.7,MATNet NoBAR) (9.716796875,MATNet NoYTB) (34.4,RTNet)};
% \addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (12.158203125,MATNet NoYTB) (0.0,RTNet)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{0.49\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=4.2cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 3},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(38.3,MATNet) (33.69140625,MATNet*) (33.3,MATNet NoBAR) (30.95703125,MATNet NoYTB) (3.9,RTNet)};
% \addplot coordinates {(43.7,MATNet) (46.6796875,MATNet*) (44.9,MATNet NoBAR) (47.75390625,MATNet NoYTB) (64.1,RTNet)};
% \addplot coordinates {(18.1,MATNet) (19.62890625,MATNet*) (21.8,MATNet NoBAR) (20.99609375,MATNet NoYTB) (26.6,RTNet)};
% \addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.29296875,MATNet NoYTB) (5.5,RTNet)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=4.2cm,
%     bar width = 8pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Fusion Layer 2},
%     title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     xlabel style = {font=\large},
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=10pt}
% ]
% \addplot coordinates {(32.0,MATNet) (29.8828125,MATNet*) (31.1,MATNet NoBAR) (20.5078125,MATNet NoYTB) (6.3,RTNet) (32.421875,FusionSeg)};
% \addplot coordinates {(45.9,MATNet) (46.2890625,MATNet*) (44.1,MATNet NoBAR) (52.5390625,MATNet NoYTB) (59.4,RTNet) (12.109375,FusionSeg)};
% \addplot coordinates {(22.1,MATNet) (23.828125,MATNet*) (24.8,MATNet NoBAR) (26.7578125,MATNet NoYTB) (21.9,RTNet) (54.296875,FusionSeg)};
% \addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.1953125,MATNet NoYTB) (12.5,RTNet) (1.171875,FusionSeg)};

% % \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (3), $\lambda=0.5$, comparing MATNet variants and RTNet at different fusion layers. Our modified version of FusionSeg has only two fusion layers (\ie fusion layer two and five) to be compared.}
% \label{fig:vos_perunit_alllayers}
% \end{figure}




\noindent \textbf{Layer-wise analysis.} 
Figure~\ref{fig:stagewise_ar_all_models} (left) shows the layer-wise analysis, (\ref{eq:biasscores}), for various action recognition models. The transformers are measured at every layer and the convolutional architectures are measured at five `stages', corresponding to ResNet blocks~\cite{he2016deep}. Interestingly, all single stream networks are biased toward static information at all layers even though the video frames of the static pairs are randomly shuffled. Most of the 3D CNNs (\eg I3D and SlowOnly) have a similar percentage of dynamic units as the C2D network, suggesting that these models do not capture sufficiently complex dynamic representations. While the static and dynamic biases in 3D CNNs do not fluctuate significantly over the different layers, the transformer-based architectures encode an increasing amount of dynamic information up until about halfway through the model, at which point the pattern tapers off and even reverses slightly. 


For the SlowFast network, we measure the biases on the representations for the slow and the fast branches  before fusion of the features. As shown in Fig.~\ref{fig:stagewise_ar_all_models} (b), the fast branch has a nontrivial number of dynamic units. A key component of the SlowFast network is the fusion branches that aim to transfer information from the fast branch to the slow branch. This transfer is accomplished by concatenating the slow and fast features followed by a time-strided convolution. Comparing the dynamic and static between the SlowOnly and SlowFast (slow) branch can reveal whether dynamic information is transferred between the pathways. The addition of the fast branch increases the dynamic units in the slow pathway by 3.3\% as early as stage two, showing the ability of the two-stream architecture to capture dynamics.
% \textcolor{red}{Additional experiments in the supplement show the robustness of our conclusion with a varying number of input frames and sampling rates.}
%Indeed, the addition of the fast pathway results in an increase in the amount of dynamic information in the slow branch. The SlowFast network sees the number of dynamic dimensions in the last layer increase by 2.4\% (note that the increase of dynamics occurs as early as stage two). We demonstrate in the supplement, through additional experiments, that this conclusion is robust to changes in the number of frames and sampling rate.

%  and 3.0\% (24.5\% versus 21.5\%) for the $8 \times 8$ \blue{and $4 \times 16$ networks, respectively.}

% Looking beyond solely the final layer of the models reveal a number of interesting observations.
% Fig.~\ref{fig:stagewise_ar_all_models} demonstrates how all models are biased toward \textit{static} information at the earlier layers, with a tendency to encode more dynamics deeper in the network. 
% The C2D, I3D and X3D models have only small, generally monotonic, changes in dynamic and static information at each stage. The SlowFast-Fast branch has the largest change in terms of the dynamic units, again showing the ability of the two-stream architecture to capture dynamic information. Conversely, the per-layer characteristics of static and dynamic encoding is different in both transformer-based architectures. They encode an increasing amount of dynamic information up until about halfway through the model, at which point the pattern tapers off and even reverses slightly. 

\noindent \textbf{Unit-wise analysis.} 
We now examine individual units using our unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}),
%our corresponding methodology (~\eqref{eq:ind_bias_scores_diff_b} 
with $\lambda=0.5$ and report the results in Fig.~\ref{fig:stagewise_ar_all_models} (right). Considering the final representation before the fully connected layer (\ie stage 5), all single stream models, other than FastOnly, contain mainly \textit{static} and \textit{joint} units. In contrast, the FastOnly model and SlowFast-Fast branch produce a nontrivial number of \textit{dynamic} units. Another finding consistent with the results from Fig.~\ref{fig:stagewise_ar_all_models} (left), is that the Fast model extracts more dynamic information \textit{when trained jointly with the Slow branch} than when trained independently. Studying the earlier layers (Fig.~\ref{fig:stagewise_ar_all_models} (right)) confirms the previous findings that the SlowFast model's cross connections are successful at transferring dynamic information from the fast branch to the slow branch throughout the network. SF-Slow (\ie the slow branch) produces a small but notable number of dynamic units early in the network. Interestingly, SF-Fast (\ie the fast branch) gradually produces more dynamic units as the representation flows deeper through the network. All single stream models other than the FastOnly model produces mainly static and joint units in all layers. The MViT and TimeSformer produce mainly static and joint units; however, the ratio of these units changes through the layers of the MViT model while it remains stable through the layers of the TimeSformer.






% \input{tex/graphs/ar_arch_indiv}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.2cm}
\subsubsection{Automatic video object segmentation} 
\label{sec:vos_archs}
\noindent\textbf{Architectures.} We study the dynamic and static biases of two-stream fusion AVOS models that take optical flow and an RGB image as input, with different types of cross connections: (i) FusionSeg~\cite{jain2017fusionseg} with no cross connections, (ii) MATNet~\cite{zhou2020motion} with motion-to-appearance cross connections and (iii) RTNet~\cite{ren2021reciprocal} with bidirectional cross connections. We concentrate on two-stream models because they currently are the strongest AVOS performers. For both MATNet~\cite{zhou2020motion} and RTNet~\cite{ren2021reciprocal}, we use the models provided by the authors without further fine-tuning. 
We use a stylized version of DAVIS16 in our analysis to evaluate the static and dynamic biases for the previous models, with stylization according to Sec.~\ref{sec:sampling}. In the case of both motion and appearance streams, we analyse features after cross connections, if present. Similarly, we analyze the features extracted after the fusion layers in all models, if present. 
% In FusionSeg, the features after the convolutional layers fusing motion and appearance from the second and fifth ResNet stages are used.

% As detailed in Sec.~\ref{sec:sampling}, since the input to VisTR is a single stream, multi-frame RGB input, we select static pairs based on the same shuffling-based sampling technique as for action recognition models.

% For a fair comparison with the two other models that fuse motion and appearance in the intermediate representations, we use a modified version of FusionSeg~\cite{jain2017fusionseg} trained on DAVIS16~\cite{Perazzi2016} in our analysis. Our modified model follows an encoder-decoder approach~\cite{chen2018encoder}, resulting in two fusion layers. Our model achieves similar performance to the original on DAVIS16 (70.8\% \vs 70.7\% mIoU).




\begin{figure*} [t]
	\begin{center}
     \centering 
     \begin{minipage}{0.55\textwidth}
		\resizebox{\textwidth}{!}{
     
     \begin{tikzpicture} \ref{legend_color_vos} \ref{legend_shades_vos}
     \begin{groupplot}[group style = {group size = 3 by 1, horizontal sep = 20pt}, width = 5.0cm, height = 5.0cm]
     \nextgroupplot[
                 line width=1.0,
                 title={\textbf{(a) Appearance Stream}},
                 title style={at={(axis description cs:0.5,0.93)},anchor=north,font=\normalsize},
                 xlabel={Network Layer},
                 ylabel={Number of Units (\%)},
                 xmin=0.5, xmax=5.5,
                 ymin=12, ymax=49,
                 xtick={1,2,3,4,5},
                 ytick={15,25,35,45},
                 x tick label style={font=\footnotesize},
                 y tick label style={font=\footnotesize},
                 x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\normalsize},
                 width=6.5cm,
                 height=5cm,
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend style={
                nodes={scale=0.87, transform shape},
                cells={anchor=west},
                legend style={at={(4.7,3.7)},anchor=south,row sep=0.01pt}, font =\normalsize},
                legend image post style={scale=0.9},
                legend columns=2,
                legend to name=legend_color_vos,
             ]
            \addlegendimage{line width=1.2pt,mark=square,mark options={line width=0.9pt,scale=1.2,solid},color=blue}
            \addlegendentry[color=black]{Dynamic}
            \addlegendimage{line width=1.2pt,mark=oplus,color=red,mark options={line width=0.7pt,scale=1.3,solid}}
            \addlegendentry[color=black]{Static}
            
             % RTNet
             \addplot[line width=1.2pt, mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=square, style=solid]
                     coordinates {(1,14.9)
                                  (2,25.6)
                                  (3,24.1)
                                  (4,25.4)
                                  (5,28.3)};
            
            
            \addplot[line width=1.2pt,mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=solid]
                     coordinates {(1,40.3)
                                  (2,34.1)
                                  (3,35.2)
                                  (4,35.9)
                                  (5,33.4)};
            
            %MATNet
            \addplot[line width=1.2pt,mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=square, style=dashed]
                     coordinates {(1,14.9)
                                  (2,16.4)
                                  (3,16.3)
                                  (4,18.5)
                                  (5,18.2)};
            \addplot[line width=1.2pt,mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=dashed]
                     coordinates {(1,40.6)
                                  (2,41.1)
                                  (3,41.4)
                                  (4,40.3)
                                  (5,40.6)};
                                  
            %FusionSeg
            \addplot[line width=1.2pt,mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=square, style=loosely dotted]
                     coordinates {(1,14.9)
                                  (2,15.8)
                                  (3,15.8)
                                  (4,19.0)
                                  (5,19.3)};
                                  
             \addplot[line width=1.2pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=loosely dotted]
                     coordinates {(1,40.6)
                                  (2,41.0)
                                  (3,41.0)
                                  (4,39.9)
                                  (5,40.0)};
                               
                               
            % %VisTR
            % \addplot[line width=1.2pt,mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=square, style=dashdotted]
            %          coordinates {(1,23.7)
            %                       (2,25.0)
            %                       (3,22.9)
            %                       (4,23.2)
            %                       (5,22.9)};
                                  
            % \addplot[line width=1.2pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=dashdotted]
            %          coordinates {(1,37.5)
            %                       (2,35.9)
            %                       (3,38.8)
            %                       (4,38.3)
            %                       (5,38.5)};
                                  
            
                                  
                                %   0.416
            
            \nextgroupplot[ line width=1.0,
                 title={\textbf{(b) Motion Stream}},
                 title style={at={(axis description cs:0.5,0.92)},anchor=north,font=\normalsize},
                 xlabel={Network Layer},
                 ylabel={},
                 xmin=0.5, xmax=5.5,
                 ymin=12, ymax=49,
                 xtick={1,2,3,4,5},
                ytick={15,25,35,45},
                x tick label style={font=\footnotesize},
                 y tick label style={font=\footnotesize},
                 x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\small},
                 %y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\normalsize},
                 width=6.5cm,
                 height=5cm,
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend style={
                    %  draw=none,
                     legend style={row sep=0.1pt},
                    nodes={scale=0.87, transform shape},
                    legend columns=-1,
                    cells={anchor=west},
                    legend style={at={(10.5,3.7)},anchor=south,row sep=0.01pt}, font =\normalsize},
                    legend to name=legend_shades_vos,
                 ]
             
            \addlegendimage{line width=1.2pt,color=black, style=solid}
            \addlegendentry[color=black]{RTNet}
            \addlegendimage{line width=1.2pt,color=black, style=dashed}
            \addlegendentry[color=black]{MATnet}
            \addlegendimage{line width=1.2pt,color=black, style=loosely dotted}
            \addlegendentry[color=black]{FusionSeg}
            % \addlegendimage{line width=1.2pt,color=black, style=dashdotted}
            % \addlegendentry[color=black]{VisTR}
            
            
            \addplot[line width=1.2pt, mark options={line width=0.8pt,scale=1.1,solid}, color=blue, style=loosely dotted, mark=square]
                     coordinates {(1,38.7)
                                  (2,39.3)
                                  (3,38.9)
                                  (4,37.1)
                                  (5,38.6)};
                                 
            %MATNet
            \addplot[line width=1.2pt, mark options={line width=0.8pt,scale=1.1,solid}, color=blue, style=dashed, mark=square]
                     coordinates {(1,36.3)
                                  (2,36.7)
                                  (3,36.5)
                                  (4,36.3)
                                  (5,35.9)};
            %RTNet
            \addplot[line width=1.2pt, mark options={line width=0.8pt,scale=1.1,solid}, color=blue, style=solid, mark=square]
                     coordinates {(1,34.0)
                                  (2,30.1)
                                  (3,28.9)
                                  (4,31.2)
                                  (5,32.1)};
                                  
            \addplot[line width=1.2pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=loosely dotted, mark=oplus]
                     coordinates {(1,21.1)
                                  (2,21.6)
                                  (3,21.2)
                                  (4,20.5)
                                  (5,20.7)};
            %MATNet
            \addplot[smooth, line width=1.2pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=dashed, mark=oplus]
                     coordinates {(1,22.3)
                                  (2,22.8)
                                  (3,22.7)
                                  (4,23.2)
                                  (5,24.7)};
            
            %RTNet                     
            \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=solid, mark=oplus]
                     coordinates {(1,23.4)
                                  (2,25.9)
                                  (3,25.8)
                                  (4,27.6)
                                  (5,28.8)};
        
        \nextgroupplot[ line width=1.0,
                 title={\textbf{(c) Fusion}},
                 title style={at={(axis description cs:0.5,0.92)},anchor=north,font=\normalsize},
                 xlabel={Network Layer},
                 ylabel={},
                 xmin=1.5, xmax=5.5,
                 ymin=12, ymax=49,
                 xtick={1,2,3,4,5},
                ytick={15,25,35,45},
                x tick label style={font=\footnotesize},
                 y tick label style={font=\footnotesize},
                 x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\small},
                 %y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\normalsize},
                 width=6.5cm,
                 height=5cm,
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
             ]
            \addplot[line width=1.2pt, mark options={line width=0.9pt,scale=1.1,solid}, color=blue, style=loosely dotted, mark=square]
                     coordinates {(2,33.9)
                                  (5,27.5)};
                                 
            %MATNet
            \addplot[line width=1.2pt, mark options={line width=0.9pt,scale=1.1,solid}, color=blue, style=dashed, mark=square]
                     coordinates {(2,32.1)
                                  (3,26.5)
                                  (4,23.0)
                                  (5,23.1)};
            %RTNet
             \addplot[line width=1.2pt, mark options={line width=0.9pt,scale=1.1,solid}, color=blue, mark=square]
                     coordinates {(2,20.7)
                                  (3,20.9)
                                  (4,21.4)
                                  (5,28.0)};
                                  
            \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=loosely dotted, mark=oplus]
                     coordinates {(2,25.1)
                                  (5,30.5)};
            %MATNet                      
            \addplot[line width=1.2pt,   mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=dashed, mark=oplus]
                     coordinates {(2,26.2)
                                  (3,30.6)
                                  (4,35.2)
                                  (5,35.5)};
            
            %RTNet                     
            \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus]
                     coordinates {(2,32.8)
                                  (3,35.0)
                                  (4,36.7)
                                  (5,33.1)};

\end{groupplot}
\vspace{-0.5cm}
% \node[draw,fill=white,inner sep=0pt,above left=0.5em] at ($(group c2r1) + (7, 4)$) {\small
%     \begin{tabular}{cccl}
%               & FusionSeg & MATNet & RTNet \\
%     Dynamic & \ref{pgfplots:c1r1} & \ref{pgfplots:c1r2} & \ref{pgfplots:c1r3}\\
%     Static & \ref{pgfplots:c2r1} & \ref{pgfplots:c2r2} & \ref{pgfplots:c2r3}\\
%     \end{tabular}};
        
\end{tikzpicture}
}
\end{minipage}%
\begin{minipage}{0.45\textwidth}
%\vspace{3em}
\resizebox{1.0\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [
%     width=\axisdefaultwidth,
%     height=4cm,
%     xbar stacked,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     %ymin=0,
%     %title = \textbf{Individual Unit Analysis on Video Segmentation Architectures},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor F (\%),
%     ytick=data,
%     legend style={
%             draw = none,
% 			area legend,
% 			at={(0.5,1.3)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={FusionSeg, MATNet, MATNet NoBAR, RTNet},
%     enlarge x limits = {value = .1},
%     %enlarge y limits={abs=0.9}
% ]
% \addplot coordinates {(8.7890625,FusionSeg) (37.6953125,MATNet) (40.185546875,MATNet NoBAR) (0.0,RTNet)};
% \addplot coordinates {(17.08984375,FusionSeg) (47.8515625,MATNet) (45.3857421875,MATNet NoBAR) (1.171875,RTNet)};
% \addplot coordinates {(73.486328125,FusionSeg) (14.453125,MATNet) (14.4287109375,MATNet NoBAR) (98.828125,RTNet)};
% \addplot coordinates {(0.634765625,FusionSeg) (0.0,MATNet) (0.0,MATNet NoBAR) (0.0,RTNet)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.2cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 5},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.4)},anchor=north,row sep=0.01pt}, font =\large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]

\addplot coordinates {(8.7890625,FusionSeg) (37.6953125,MATNet) (37.5244140625,MATNet*) (40.185546875,MATNet NoBAR) (49.560546875,MATNet NoYTB) (0.0,RTNet)};
\addplot coordinates {(17.08984375,FusionSeg) (47.8515625,MATNet)  (44.62890625,MATNet*) (45.3857421875,MATNet NoBAR) (45.60546875,MATNet NoYTB) (1.171875,RTNet)};
\addplot coordinates {(73.486328125,FusionSeg) (14.453125,MATNet) (17.8466796875,MATNet*) (14.4287109375,MATNet NoBAR) (4.736328125,MATNet NoYTB) (98.828125,RTNet)};
\addplot coordinates {(0.634765625,FusionSeg) (0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.09,MATNet NoYTB) (0.0,RTNet)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture} 
\hfill
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.2cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 4},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    % xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,1.4)},anchor=north,row sep=0.01pt}, font =\large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]

\addplot coordinates {(28.6,MATNet) (33.7890625,MATNet*) (30.3,MATNet NoBAR) (46.044921875,MATNet NoYTB) (0.0,RTNet)};
\addplot coordinates {(40.3,MATNet) (37.40234375,MATNet*) (39.0,MATNet NoBAR) (32.080078125,MATNet NoYTB) (65.6,RTNet)};
\addplot coordinates {(31.1,MATNet) (28.80859375,MATNet*) (30.7,MATNet NoBAR) (9.716796875,MATNet NoYTB) (34.4,RTNet)};
\addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (12.158203125,MATNet NoYTB) (0.0,RTNet)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\vfill
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=\axisdefaultwidth,
    height=4.2cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 3},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    xlabel style = {font=\large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]
\addplot coordinates {(38.3,MATNet) (33.69140625,MATNet*) (33.3,MATNet NoBAR) (30.95703125,MATNet NoYTB) (3.9,RTNet)};
\addplot coordinates {(43.7,MATNet) (46.6796875,MATNet*) (44.9,MATNet NoBAR) (47.75390625,MATNet NoYTB) (64.1,RTNet)};
\addplot coordinates {(18.1,MATNet) (19.62890625,MATNet*) (21.8,MATNet NoBAR) (20.99609375,MATNet NoYTB) (26.6,RTNet)};
\addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.29296875,MATNet NoYTB) (5.5,RTNet)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis} [xbar stacked,
     width=\axisdefaultwidth,
    height=4.2cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Fusion Layer 2},
    title style={at={(axis description cs:0.5,1.15)},anchor=north,font=\large},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    xlabel style = {font=\large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={MATNet NoYTB, MATNet NoBAR, MATNet*, MATNet, RTNet, FusionSeg},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=10pt}
]
\addplot coordinates {(32.0,MATNet) (29.8828125,MATNet*) (31.1,MATNet NoBAR) (20.5078125,MATNet NoYTB) (6.3,RTNet) (32.421875,FusionSeg)};
\addplot coordinates {(45.9,MATNet) (46.2890625,MATNet*) (44.1,MATNet NoBAR) (52.5390625,MATNet NoYTB) (59.4,RTNet) (12.109375,FusionSeg)};
\addplot coordinates {(22.1,MATNet) (23.828125,MATNet*) (24.8,MATNet NoBAR) (26.7578125,MATNet NoYTB) (21.9,RTNet) (54.296875,FusionSeg)};
\addplot coordinates {(0.0,MATNet) (0.0,MATNet*) (0.0,MATNet NoBAR) (0.1953125,MATNet NoYTB) (12.5,RTNet) (1.171875,FusionSeg)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\end{minipage}
	\end{center}
	\vspace{-0.6cm}
	\caption{Layer and unit-wise analysis on off-the-shelf VOS networks. \textbf{Left}: Encoding of dynamic and static factors for motion, appearance streams and fusion layers in FusionSeg~\cite{jain2017fusionseg}, MATNet~\cite{zhou2020motion} and RTNet~\cite{ren2021reciprocal} using the layer-wise metric, (\ref{eq:biasscores}). Fusion layers are mostly biased toward the static factor. \textbf{Right}: Individual units analysis for the three models for fusion layer 5 using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}). MATNet has the largest number of dynamic units.}\label{fig:stagewise_vos}
	\vspace{-0.64cm}
\end{figure*}

\noindent\textbf{Implementation details.} For a fair comparison with MATNet and RTNet, that fuse motion and appearance features in the intermediate representations, we use a modified version of FusionSeg~\cite{jain2017fusionseg} trained on DAVIS16~\cite{Perazzi2016} in our analysis. Our modified model follows an encoder-decoder approach~\cite{chen2018encoder}, resulting in two fusion layers at stages two and five. Our FusionSeg model is trained with a batch size of eight, using SGD with learning rate 0.001, a momentum of 0.9, a ``poly'' learning rate policy using a power of 0.9 and weight decay $1\times10^{-4}$. 
As we want to isolate the effect of training datasets, we do not perform pretraining with the motion stream, as proposed in the original paper~\cite{jain2017fusionseg}. 
The MATNet variants are trained with two GPUs in parallel with batch size six (the original MATNet used a batch size of two and a single GPU), the rest of the hyperparameters follow the original work~\cite{zhou2020motion}. We denote the original model provided by the authors as ``MATNet'', while our reproduction of MATNet as ``MATNet*''. We analyze MATNet trained only on DAVIS16 (\ie without any Youtube-VOS data), which we call ``MATNet NoYTB'' and also MATNet trained without its boundary-aware refinement module and boundary loss, denoted as ``MATNet NoBAR''. 
% We train a MATNet variant that we call ``MATNet NoBAR'', where we remove all boundary aware refinement (BAR) modules and the boundary loss. We also experiment with another MATNet variant that, unlike the original model, does not train on additional YouTubeVOS data~\cite{xu2018youtube}. We call this version ``MATNet NoYTB''.

% \noindent\textbf{Architectures.} We study the dynamic and static biases of video object segmentation models with a focus on multi-modality two-stream fusion models: (i) FusionSeg~\cite{jain2017fusionseg} with no cross connections, (ii) MATNet~\cite{zhou2020motion} with motion-to-appearance (non-recirprocal) cross connections and (iii) RTNet~\cite{ren2021reciprocal} with bidirectional (reciprocal) cross connections. FusionSeg is the first two-stream video object segmentation model proposed. We use a modified version to ensure fusion occurs in the intermediate representation, by concatenating the features before the atrous spatial pyramid pooling module followed by a 1x1 convolutional layer. In order to make it comparable with the two other models that fuse motion and appearance in the intermediate representations. We further fuse early layer features and use a technique similar to~\cite{chen2018encoder} for the decoder but without allowing cross connections between both motion and appearance streams. Our modified FusionSeg model is able to perform similar to the original work~\cite{jain2017fusionseg} on DAVIS'16 benchmark with 70.8\% mean intersection over union. For both MATNet and RTNet we use the pre-trained models provided by the authors without any finetuning on our end. We use stylized DAVIS to evaluate the static and dynamic biases for the previous models. %, and report the 95\% confidence interval to show the statistical significance over 4 runs as DAVIS is a considerably smaller dataset 


\noindent \textbf{Layer-wise analysis.} Figure~\ref{fig:stagewise_vos} (left), shows the layer-wise analysis for the motion and appearance streams as well as the fusion layers according to our layer-wise metric, (\ref{eq:biasscores}).
%our layer-wise methodology,~\eqref{eq:biasscores}. 
Similar to our finding with the action recognition models in Sec.~\ref{sec:ar_models}, the majority of the video object segmentation models are biased toward the \textit{static} factor in the fusion layers (\ie fusion layers three, four and five). We observe an increase in the dynamic bias in the appearance stream as we go deeper in the network, especially for RTNet. In contrast, the static and dynamic biases in the motion streams of both FusionSeg and MATNet are somewhat consistent throughout layers. Interestingly, in RTNet, the \textit{static} bias increases as the representation goes deeper in the network. This result likely stems from the bidirectional cross-connections in RTNet.%, that strengthens the downstream task accuracy on DAVIS. 

\noindent \textbf{Unit-wise analysis.} 
% \blue{Kosta: These are not proper sentences - Although the static and dynamic biases in MATNet appear to be similar to FusionSeg, and RTNet appears to have more dynamic units in the final fusion layers. However, the individual unit analysis shows interesting patterns beyond that.}
The individual unit analysis for these models obtained using our unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}), with $\lambda=0.5$
%, obtained using the corresponding methodology,~\eqref{eq:ind_bias_scores_diff_b} ($\lambda=0.5$), 
is shown in Fig.~\ref{fig:stagewise_vos} (right). Looking at the final representation of the models (\ie fusion layer 5), we observe that MATNet has more dynamic and static units compared to RTNet and FusionSeg, which both show a greater number of jointly encoding units. This pattern indicates that cross connections, as present in MATNet, can lead to an increase in the specialized units that encode the static and dynamic factors in the late fusion layers. The ``MATNet NoBAR'' and ``MATNet NoYTB'' results are consistent, and confirm that the source behind such an increase is not the BAR module or YTB training. The earlier fusion layers in Fig.~\ref{fig:stagewise_vos} (right) also show that MATNet captures the most dynamic units. In fusion layer two, FusionSeg appears on par with MATNet in terms of dynamic units, but has fewer static units and more joint units. In comparison, RTNet tends to have the most unbalanced units of all three models, which become skewed toward joint encoding units in the late fusion layers. 
% This pattern confirms that models with less ability to capture dynamics in the late fusion layers (\ie FusionSeg and RTNet), generally tend to favour jointly encoding units over specialized units, and have less balance between static and dynamic units. 
These patterns show that over all fusion layers, MATNet generally has a more balanced ratio of dynamic and static units and more dynamic units than other models.
It also shows that MATNet trained on solely DAVIS'16 exhibits a similar pattern of capturing more dynamic units than other models, but has less dynamic units in the earlier layers, unlike the original MATNet. This result suggests models with cross connections that are not pretrained on saliency segmentation datasets are beneficial to the model's encoding capabilities when the goal is to capture dynamics, \eg camouflage object segmentation.
% As with action recognition, \textcolor{red}{experiments in the supplement demonstrates that our observations are robust with respect to variations of the threshold, $\lambda$.}





\begin{figure} [t]
	\begin{center}
     \centering 
     \begin{minipage}{0.185\textwidth}
		\resizebox{\textwidth}{!}{
     \begin{tikzpicture}  \ref{legend_color_instance_vos}
     \begin{axis} [
     line width=1.0,
                 title={\textbf{VIS - Layerwise}},
                 title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
                 xlabel={Network Layer},
                 ylabel={Number of Units (\%)},
                 xmin=0.5, xmax=12.5,
                 ymin=20, ymax=45,
                 xtick={2,4,6,8,10,12},
                 ytick={15,20,25,30,35,40,45},
                 x tick label style={font=\small},
                 y tick label style={font=\small},
                 x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\normalsize},
                 y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\normalsize},
                 xtick pos=left,
                 ytick pos=bottom,
                 width=6.5cm,
                 height=5cm,
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend style={
                     %draw=none,
                     nodes={scale=0.7, transform shape},
                     cells={anchor=west},
                     legend style={at={(3,1)},anchor=south}, font =\small},
                     legend columns=2,
                     legend entries={[black]R50-Dyn,[black]R50-Stat,[black]R101-Dyn,[black]R101-Stat},
                    legend to name=legend_color_instance_vos,
        ]

            %VisTR-R50
            \addplot[line width=1.2pt,mark options={line width=0.8pt,scale=1,solid}, color=blue, mark=square, style=dashdotted]
                     coordinates {(1,23.7)
                                  (2,24.2)
                                  (3,24.2)
                                  (4,25.0)
                                  (5,25.0)
                                  (6,24.7)
                                  (7,22.9)
                                  (8,23.4)
                                  (9,22.9)
                                  (10,23.2)
                                  (11,23.4)
                                  (12,22.9)};
                                  
            \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=dashdotted]
                     coordinates {(1,37.5)
                                  (2,36.5)
                                  (3,36.5)
                                  (4,35.9)
                                  (5,35.9)
                                  (6,36.5)
                                  (7,38.8)
                                  (8,38.3)
                                  (9,38.3)
                                  (10,38.3)
                                  (11,38.0)
                                  (12,38.5)};
                       
                                  
            %VisTR-R101
            \addplot[line width=1pt,mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=triangle, style=solid]
                     coordinates {(1,25.3)
                                  (2,23.4)
                                  (3,23.4)
                                  (4,23.2)
                                  (5,23.2)
                                  (6,24.0)
                                  (7,23.2)
                                  (8,22.4)
                                  (9,22.4)
                                  (10,22.4)
                                  (11,22.4)
                                  (12,22.7)};
                                  
            \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=+, style=solid]
                     coordinates {(1,36.2)
                                  (2,37.2)
                                  (3,37.0)
                                  (4,37.2)
                                  (5,36.7)
                                  (6,36.5)
                                  (7,38.0)
                                  (8,38.5)
                                  (9,38.5)
                                  (10,38.5)
                                  (11,38.8)
                                  (12,38.3)};
                                  
            % \legend {R50-Dyn,R50-Stat,R101-Dyn,R101-Stat};
        \end{axis}
\end{tikzpicture}
}
\end{minipage}%
\begin{minipage}{0.31\textwidth}
%\vspace{3em}
% \resizebox{\textwidth}{!}{
%      \begin{tikzpicture}  \ref{legend_color_instance_vos_indv}
%      \begin{axis} [
%      line width=1.0,
%                  title={\textbf{VIS - Unitwise}},
%                  title style={at={(axis description cs:0.5,0.97)},anchor=north,font=\normalsize},
%                  xlabel={Network Layer},
%                 %  ylabel={Number of Units (\%)},
%                  xmin=0.5, xmax=12.5,
%                  ymin=17, ymax=76,
%                  xtick={1,2,3,4,5,6,7,8,9,10,11,12},
%                  ytick={10,20,30,40,50,60,70},
%                  x tick label style={font=\footnotesize},
%                  y tick label style={font=\footnotesize},
%                  x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\small},
%                  y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\normalsize},
%                 xtick pos=left,
%                 ytick pos=bottom,
%                  width=6.5cm,
%                  height=5cm,
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                  legend style={
%                      %draw=none,
%                      nodes={scale=0.66, transform shape},
%                      cells={anchor=west},
%                      legend style={at={(3.27,0.15)},anchor=south}, font =\footnotesize},
%                      legend columns=2,
%                      legend entries={[black]R50-Stat,[black]R50-Joint,[black]R101-Stat,[black]R101-Joint},
%                     legend to name=legend_color_instance_vos_indv,
%         ]

%             %VisTR-R50               
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=square, style=dotted]
%                      coordinates {(1,63.3)
%                                   (2,59.1)
%                                   (3,64.1)
%                                   (4,49.2)
%                                   (5,46.4)
%                                   (6,49.2)
%                                   (7,46.4)
%                                   (8,47.4)
%                                   (9,53.4)
%                                   (10,51.3)
%                                   (11,51.6)
%                                   (12,50.5)};
%             % Joint          
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=orange, mark=oplus, style=dotted]
%                      coordinates {(1,36.7)
%                                   (2,40.9)
%                                   (3,35.9)
%                                   (4,50.8)
%                                   (5,53.6)
%                                   (6,50.8)
%                                   (7,53.6)
%                                   (8,52.6)
%                                   (9,46.6)
%                                   (10,48.7)
%                                   (11,48.4)
%                                   (12,49.5)};     
%VisTR-R101     
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=triangle, style=solid]
%                      coordinates {(1,53.9)
%                                   (2,62.0)
%                                   (3,62.8)
%                                   (4,71.1)
%                                   (5,68.0)
%                                   (6,63.0)
%                                   (7,57.0)
%                                   (8,59.1)
%                                   (9,64.3)
%                                   (10,61.7)
%                                   (11,58.3)
%                                   (12,62.0)};
%             % Joint          
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=orange, mark=+, style=solid]
%                      coordinates {(1,46.1)
%                                   (2,38.0)
%                                   (3,37.2)
%                                   (4,28.9)
%                                   (5,32.0)
%                                   (6,37.0)
%                                   (7,43.0)
%                                   (8,40.9)
%                                   (9,35.7)
%                                   (10,38.3)
%                                   (11,41.7)
%                                   (12,38.0)};
%         \end{axis}
% \end{tikzpicture}}

\resizebox{1.0\textwidth}{!}{

\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 3},
    title style={at={(axis description cs:0.5,1.5)},anchor=north,font=\LARGE},
    x tick label style={font=\large},
    y tick label style={font=\large},
    x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\large},
    y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\large},
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,2.3)},anchor=north,row sep=0.01pt}, font =\Large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={R101,R50},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]

\addplot coordinates {(0,R101) (0,R50)};
\addplot coordinates {(62.8,R101) (64.1,R50)};
\addplot coordinates {(37.2,R101) (35.9,R50)};
\addplot coordinates {(0.0,R101) (0.0,R50)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture} 
\hfill
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 6},
    title style={at={(axis description cs:0.5,1.5)},anchor=north,font=\LARGE},
    x tick label style={font=\large},
    y tick label style={font=\large},
    x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\large},
    y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\large},
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,2.3)},anchor=north,row sep=0.01pt}, font =\Large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={R101,R50},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]

\addplot coordinates {(0,R101) (0,R50)};
\addplot coordinates {(63.0,R101) (49.2,R50)};
\addplot coordinates {(37.0,R101) (50.8,R50)};
\addplot coordinates {(0.0,R101) (0.0,R50)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}
\vfill
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 9},
    title style={at={(axis description cs:0.5,1.5)},anchor=north,font=\LARGE},
    x tick label style={font=\large},
    y tick label style={font=\large},
    x label style={at={(axis description cs:0.5,0.0)},anchor=north,font=\Large},
    xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={R101,R50},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]
\addplot coordinates {(0,R101) (0,R50)};
\addplot coordinates {(64.3,R101) (53.4,R50)};
\addplot coordinates {(35.7,R101) (46.6,R50)};
\addplot coordinates {(0.0,R101) (0.0,R50)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 12},
    title style={at={(axis description cs:0.5,1.5)},anchor=north,font=\LARGE},
    xlabel = Units Encoding Factor $F$ (\%),
    x tick label style={font=\large},
    y tick label style={font=\large},
    xlabel style={at={(axis description cs:0.5,0.0)},anchor=north,font=\Large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={R101,R50},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]
\addplot coordinates {(0,R101) (0,R50)};
\addplot coordinates {(62.0,R101) (50.5,R50)};
\addplot coordinates {(38.0,R101) (49.5,R50)};
\addplot coordinates {(0.0,R101) (0.0,R50)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}

\end{minipage}
	\end{center}
	\vspace{-0.6cm}
	\caption{Layer and unit-wise analysis on off-the-shelf state-of-the-art VIS models. \textbf{Left}: Encoding of dynamic and static factors for motion, appearance streams and fusion layers in VisTR-R50 and VisTR-101~\cite{wang2021end} using the layer-wise metric, (\ref{eq:biasscores}). All layers are biased toward the static factor. \textbf{Right}: Individual units analysis for the two VisTR variants using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}).}\label{fig:inst_vos_arch}
	\vspace{-0.8cm}
\end{figure}


\vspace{-0.3cm}
\subsubsection{Video instance segmentation} 
\label{sec:vis_archs}




\noindent\textbf{Architectures.}For the VIS task, we conduct our analysis on two versions of the state-of-the-art VisTR~\cite{wang2021end} model. VisTR is an end-to-end trained encoder-decoder transformer based architecture with a 2D CNN backbone used for the initial feature extraction. Both the encoder and decoder have six layers for which we compute the static and dynamic biases.

\noindent\textbf{Implementation details.} All pre-trained models are retrieved from the original repository~\cite{wang2021end} with no training done on our end. All VIS models are trained on the YouTube-VIS~\cite{xu2018youtube} dataset. We use the same 2D CNN backbones as per the original paper~\cite{wang2021end}, either a ResNet50 or ResNet101. We perform the static and dynamic estimation using the stylized DAVIS16 dataset.

\noindent\textbf{Layer-wise analysis.} Figure~\ref{fig:inst_vos_arch} (left) shows the results of our layer-wise analysis on two variants of VisTR~\cite{wang2021end}. It is observed that both models are strongly biased toward the static factor. This bias toward static information increases later in the network, \eg at the first transformer layer the ResNet101 variant has static and dynamic biases of 36.2\% and 25.3\%, respectively, and at the last layer has biases of 38.3\% and 22.7\%, respectively. This result likely stems due to the nature of the VIS task that requires tracking and object-level matching across frames.

\noindent\textbf{Unit-wise analysis.}Figure~\ref{fig:inst_vos_arch} (right) shows the results of our layer-wise and per-unit analysis on two variants of VisTR~\cite{wang2021end}. Notably, VisTR with either backbone produces solely static and joint units, however, the ratio of these units differ at various layers of the models. The ResNet50 backbone contains about twice the number of static units compared with joint units for the first three layers, and then converges to an even ratio thereafter. Meanwhile, the ResNet101 backbone contains a larger number of static units throughout the entire architecture. This suggests that the 2D backbone plays a role in the type of information captured for spatiotemporal models and that deeper backbones may capture more static information.  


%In the supplement, we also demonstrate that motion-to-appearance cross connections relate to the performance for a task requiring dynamic information (\ie the segmentation of camouflaged moving objects (MoCA)~\cite{lamdouar2020betrayed}). 





















% \blue{Kosta: Is this paragraph suppose to refer to a figure?}
% Our layer-wise measure as previously shown in Fig.~\ref{fig:stagewise_vos} appears to have MATNet with less dynamic bias than RTNet unlike the individual unit analysis. This is explained by the Softmax normalization applied in (\ref{eq:biasscores}), which results in a relative measure between the dynamic and static bias. Analyzing individual units resolves this discrepancy as it does not use normalization, allowing us to inspect more the static/dynamic units and showing increased specialized static and dynamic units in MATNet than the other models.

% there are many more units in MATNet than in RTNet that have correlations for the dynamic factor > 0.5, but the dynamic corerlations in RTNet's joint units are very large and sum to a larger total amount of dynamic information contained in the model's last layer

%In Fig.~\ref{fig:vos_models_indiv} right, we show that motion-to-appearance cross connections in MATNet is a better approach on MoCA. This consequently correlates with the larger number of dynamic units found in MATNet. 

%In Figure~\ref{fig:vos_indiviual_units} it shows the histogram of the biases computed following equation~\ref{eq:ind_bias_scores_diff_a}, for the different models on the late sensor fusion layer. Interestingly, MATNet clearly follows a bi-modal distribution, unlike uni-modal distribution form both FusionSeg and RTNet. 

%\input{tex/graphs/vos_arch_indiv_2}

\vspace{-0.3cm}
\subsubsection{Summary and shared insights}
% We showed in both action recognition and video segmentation that most of the examined state-of-the-art models are biased toward encoding static information.
We showed that most of the examined state-of-the-art models for all tasks are biased toward encoding static information.
We also demonstrated the efficacy of two-stream models with motion-to-appearance~\cite{zhou2020motion} (fast-to-slow~\cite{feichtenhofer2019slowfast}) cross connections to enable greater encoding of dynamic information. For the VIS task, we observed that solely static and joint units are produced in the architectures analyzed, however the 2D backbone can influence the ratio between these units. Finally, we documented that the final layers of dynamic biased models are capable of producing more specialized dynamic units compared to the joint units produced by static biased models. 

%The main different insight between both is ...(not sure whats different).

%In Figure~\ref{fig:indiviual_units_all_models} we show the joint encoding analysis for all three models at threshold $\lambda=0.5$ for both early and late sensor fusion layers. It clearly shows that video object segmentation models consistently have units that jointly encode dynamic and static factors similar to action recognition. It also confirms that motion-to-appearance cross connections in MATNet causes the largest increase in the dynamic bias of certain units within the sensor fusion layers while maintaining jointly encoding units, with respect to FusionSeg and RTNet.  Surprisingly, we found that MATNet model does not have any units that neither correlate with static or dynamic factors unlike both FusionSeg and RTNet, even when trying higher $\lambda$ refer to Appendix. This indicates that the hard assumption on the residual factors to always exist might not be correct in certain models, and having a different analysis method as in equation~\ref{eq:ind_bias_scores_diff_b} enriches our understanding of what these models learn.

%MatNet~\cite{zhou2020motion} is a two-stream model that investigates the use of cross connections in a non-reciprocal fashion from the motion stream to the appearance stream. A motion attentive blocks are used for such task. This is followed by scale sensitive attention modules that learns to fuse the features from both motion and appearance followed by boundary aware refinement modules. Finally, RTNet~\cite{ren2021reciprocal} follows a reciprocal cross-connection two stream model, where motion-to-appearance and appearance-to-motion attention is performed. Along with the use of cross-frame attention on pairs of sampled frames. A spatiotemporal attention fusion is performed on the motion and appearance features before the segmentation decoder.

%Table~\ref{table:vos_motappbias} demonstrates the motion/appearance bias on the final layer of the motion and appearance streams just before the fusion, and after the cross-connection blocks in case of MATNet and RTNet. It also shows the sensor fusion layers bias in all models, corresponding to the features extracted after the fusion blocks. This is mapped to the simple 1x1 convolution fusion layer in FusionSeg, the SSA module in MATNet and the spatiotemporal fusion block in RTNet. It clearly demonstrates the success of our metric and proposed sampling scheme to capture that the features in the intermediate layers of motion/appearance streams are biased toward the corresponding factors. Figure~\ref{fig:stagewise_vos} shows the stage-wise analysis along both motion and appearance streams to confirm on it, where we plot the 95\% confidence interval to show the statistical significance of the bias change on different stages. Interestingly, it shows the increase of motion bias in the appearance stream as we go deeper similar to action reocgnition models, especially with cross-connections as in RTNet. That confirms on the exchange between both streams that leads to an improved segmentation. On the other hand, the motion stream for both FusionSeg and MATNet does not show significant change along the stages, but is rather noticeable in RTNet where the appearance bias increases as we go deeper. This stems from the reciprocal transformation proposed in their method, which strengthens the downstream task accuracy. It is further confirmed on RTNet with ResNet-34 backbone (refer to the appendix) that similar to ResNeXt-50 the reciprocal cross connections closes the gap between motion and appearance bias in both streams. 

%Nonetheless, we can clearly see in all models that the majority of sensor fusion layers are appearance biased, this has relation to both the fact that higher semantics are incorporated in the later layer features and would be biased more toward the appearance. Along with the bias existent in the training datasets specifically DAVIS'16 which will be discussed in the following section. Finally, we generally observe an increase in the appearance bias in MATNet more than the other models. This is mainly due to the use of the proposed boundary aware refinement modules and the boundary loss that focuses more on the appearance than motion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure} [t]
 \def\arraystretch{1.35}
 \setlength\tabcolsep{2.4pt}
\centering
\begin{minipage}{0.57\linewidth}
\resizebox{1.0\textwidth}{!}{
	\begin{tabu}{c cccc}
	\tabucline[1pt]{-}
	 \multirow{2}{*}{Dataset}&  \multicolumn{2}{c}{\textbf{SlowOnly}} & \multicolumn{2}{c}{\textbf{FastOnly}} \\
	 \cline{2-3} \cline{4-5}
	%\hline
	  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)\\
	   \tabucline[1pt]{-}
	   %Kinetics& 21.4 & 38.4 & 28.1 & 20.3 \\
	   Kinetics& 21.4 & 38.4 & 27.3 & 30.9 \\
	   Diving48& 23.1 & 34.0 & 23.8 & 27.3\\
	   SSv2& 23.6 & 32.6 & 28.5 & 23.0 \\
	  % \hline
	\tabucline[1pt]{-}
	\end{tabu}}
		\end{minipage} \hfill   
	\begin{minipage}{0.4\linewidth}
	\resizebox{1.0\textwidth}{!}{
	\begin{tikzpicture} \ref{target_legend}
    \begin{axis}[
       line width=1.0,
        title={Performance on Shuffled Frames},
        title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
        xlabel={Dataset},
        % x label style={font=\small},
        ylabel={Relative Performance Drop (\%)},
        % xmin=0, xmax=550,
        ymin=-65, ymax=12,
        % xtick={50,100,200,300,400,500},
        ytick={0,-10,-20,-30,-40,-50,-60},
        symbolic x coords={SSv2, Diving48, Kinetics},
        xtick=data,
        x tick label style={font=\footnotesize},
        % x tick label style={font=\footnotesize,rotate=20,anchor=east},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0.03)},anchor=north,font=\small},
        y label style={at={(axis description cs:0.12,.5)},anchor=south,font=\small},
        width=6.7cm,
        height=5.5cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
         %draw=none,
         nodes={scale=0.9, transform shape},
         cells={anchor=west},
         legend style={at={(3.8,0.25)},anchor=south}, font =\footnotesize},
         %legend columns=1,
         legend entries={[black]SlowOnly,[black]FastOnly,[black]Baseline},
        legend to name=target_legend,
    ]
    
    \addplot[only marks,mark size=3.3pt,color=orange,mark=*,]
    coordinates {(SSv2,-59.8) (Diving48,-2.0) (Kinetics,-0.5)};
    
    
    % SlowOnly
    % \addplot[line width=1.8pt,mark size=1.9pt,color=orange,mark=*,]
    %     coordinates {(50,72.8)(100,71.9)(200,70.2)(300,69.6)(400,67.9)(500,64.7)};
        
    % FastOnly
    \addplot[only marks,mark size=3.3pt,color=blue,mark=triangle*,]
        coordinates {(SSv2,-33.6) (Diving48,-18.0) (Kinetics,-1.2)};
        
        
    \addplot[line width=1.3pt,black,dotted,sharp plot,update limits=false] 
	    coordinates {([normalized]-10,0)([normalized]10,0)};
    \end{axis}
\end{tikzpicture}}
\end{minipage} 
\vspace{-0.3cm}
\caption{Analyses of biases of action recognition datasets. \textbf{Left:} \textit{Dynamic} and \textit{static} biases using the layer-wise metric, (\ref{eq:biasscores}), for models trained on Kinetics-400~\cite{carreira2017quo}, Diving48~\cite{li2018resound} and SSv2~\cite{goyal2017something}. \textbf{Right:} Relative drop in Top 1 Acc (\%) for the SlowOnly and FastOnly models trained with shuffled frames with respect to standard training (\ie baseline).}\label{fig:dataset_compare}
\vspace{-0.7cm}
\end{figure}

\vspace{-0.5cm}
\subsection{Training datasets}\label{sec:dataset_effect}
\vspace{-0.1cm}

\subsubsection{Action recognition}\label{sec:ar_dataset}
\noindent \textbf{Datasets.} With the knowledge that action recognition models often use static context biases in the data to make predictions~\cite{derpanis2012action,choi2019can,ilic2022appearance}, we 
consider datasets in the following evaluations which were designed with the goal of benchmarking a model's ability to capture dynamic information. Two popular datasets of this type are Something-Something-v2~\cite{goyal2017something} (SSv2) and Diving48~\cite{li2018resound}. SSv2 is a fine-grained ego-centric dataset with 174 classes and over 30,000 unique objects. Notably, different actions in SSv2 include similar appearance but different motions, \eg the classes `moving something from right-to-left' and `moving something from left-to-right'. Diving48~\cite{li2018resound} was created to be ``a dataset with no significant biases toward static or short-term motion representations, so that the capability of models to capture long-term dynamics information could be evaluated''~\cite{d48_web}. All actions are a particular type of dive and differ by only a single rotation or flip. We compare Kinetics-400, Diving48 and SSv2 to determine the extent that each dataset requires dynamics for action recognition. 

% "The purpose was to create an action recognition dataset with no significant biases toward static or short-term motion representations, so that the capability of models to capture long-term dynamics information could be evaluated."
% \input{tex/graphs/ar_datasets}

% \begin{table} [t]
% \def\arraystretch{1.35}
% \setlength\tabcolsep{2.4pt}
% \centering
% \resizebox{0.49\textwidth}{!}{
% 	\begin{tabular}{c |cc|cc|cc}
% 	\specialrule{1.2pt}{1pt}{1pt}
	
% 	 \multirow{2}{*}{Method}&  \multicolumn{2}{c}{\textbf{SSv2}} & \multicolumn{2}{c}{\textbf{Diving48}} &  \multicolumn{2}{c}{\textbf{Kinetics}}   \\
% 	%\hline
% 	  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%) \\
% 	    \specialrule{1.2pt}{1pt}{1pt}
% 	   % STYLIZED ACTIVITYNET RESULTS
% 	   %SlowOnly-8x8 & 22.6 & 36.8 & 23.6 & 32.6 & TBD  & TBD \\
% 	   %\hline
% 	   %SlowFast (cat)  & 26.3 & 31.4 & 27.2  & 24.8 & 24.0 & 24.2 \\
% 	   %SlowFast (slow) & 24.7 & 33.3 & 26.0 & 26.0 & 21.5  & 27.9 \\
% 	   %SlowFast (fast) & 33.6 & 23.0 & 31.2 & 21.5 & 24.2 & 20.7 \\
	   
%         % RANDOM SUBSET KINETICS RESULTS
% 	   %SlowOnly-8x8 & 21.4 & 38.4 & 23.6 & 32.6 & 16.7  & 38.0 \\
% 	   %\hline
% 	   %SlowFast (cat) & 27.2  & 24.8 & 24.0 & 24.2 \\
% 	   %SlowFast (slow) & 23.4 & 33.2 & 26.0 & 26.0 & 21.5  & 27.9 \\
% 	   %SlowFast (fast) & 28.5 & 22.7 & 31.2 & 21.5 & 24.2 & 20.7 \\
	   
% 	   SlowOnly  & 23.6 & 32.6 & 16.7  & 38.0 & 21.4 & 38.4 \\
% 	  % \hline
% 	   %SlowFast (cat) & 27.2  & 24.8 & 24.0 & 24.2   & 24.7& 31.1\\
% 	   %SlowFast (slow) & 26.0 & 26.0 & 21.5  & 27.9 & 23.4 & 33.2 \\
% 	   %SlowFast (fast) & 31.2 & 21.5 & 24.2 & 20.7 & 28.5 & 22.7  \\
% 	  % \hline
% 	   FastOnly & 28.5 & 23.0 & 24.6 & 25.4 & 28.1 & 20.3 \\
% 	  % \hline
% 	   %MViT & - & - & 25.3 & 29.9 & 27.0 & 30.6 \\
% 	\specialrule{1.2pt}{1pt}{1pt}
% 	\end{tabular}
% 	}
% \caption{\textit{Dynamic} and \textit{static} dimensions for networks trained on Kinetics-400, Something-Something-v2, and Diving-48 datasets. All networks use a sampling of 8x8. All measurements are taken using the global pooled representation of the last layer of the network before the fully connected layer. Slow and fast, refer to the slow branch, fast branch, and concatenation (along the channel dimension) of the SlowFast model.}\label{tab:dataset_compare}
% \end{table}



\noindent \textbf{Dataset bias.} We use the layer-wise metric,  (\ref{eq:biasscores}), to estimate the static and dynamic units captured in the last layer of two models trained on the three datasets, as shown in the table of Fig.~\ref{fig:dataset_compare} (left). We generate Stylized SSv2 and Stylized Diving48 to produce the static and dynamic estimates (and continue using Stylized ActivityNet for Kinetics-400 trained models). We measure the last layer, as the final prediction is made directly from it and thus is most representative of what information the model uses for the final prediction. The SlowOnly and FastOnly architectures follow a similar pattern to that found in Sec.~\ref{sec:architectures}, with the FastOnly consistently capturing more dynamic information. Surprisingly, models trained on Diving48 capture a similar amount of dynamics compared to Kinetics. These results may seem curious at first, as it seems unlikely that models could perform well on Diving48 without dynamic information.% a significant amount of dynamic information. 

To further understand this result, we conduct a simple experiment, where the model only has static information to learn from. As discussed in Sec.~\ref{sec:sampling}, frame-shuffled videos will have the same static information as a non-shuffled input, but the temporal correlations, and hence dynamic information, will be corrupted. This forces the model to focus on static information for classification. We compare the Top-1 validation accuracy of models trained and validated on shuffled frames to that of models with standard training. Figure~\ref{fig:dataset_compare} (right) shows the results of the SlowOnly and FastOnly networks on Diving48, SSv2 and Kinetics-400, in terms of the relative performance on shuffled frames compared to unshuffled. For a fair comparison, we initialize all models from Kinetics-400. Both models show strong relative performance when trained on shuffled videos for Diving48 and Kinetics-400; however, for SSv2 the classification performance is decreased to a greater extent when trained on shuffled frames. These results show that SSv2 is a better alternative for temporally benchmarking networks.

% \input{tex/graphs/ar_dataset_indiv}
\begin{figure}[t]
    \centering
    \resizebox{0.49\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [
    width=\axisdefaultwidth,
    height=3.2cm,
    xbar stacked,
    bar width = 10pt,
    xmin = 0,
    xmax = 100,
    %ymin=0,
    %title = \textbf{Individual Unit Analysis on Video Segmentation Architectures},
    % ylabel = Model,
    xlabel = Units Encoding Factor F (\%),
    ytick=data,
    legend style={
            draw = none,
			area legend,
			at={(0.5,1.4)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={Diving48, Kinetics, SSv2},
    enlarge x limits = {value = 0.1},
    %enlarge y limits={value = 18pt}
]


% \addplot coordinates { (0,Diving48) (2,Kinetics)  (173,SSv2)};
% \addplot coordinates { (1839,Diving48) (1668,Kinetics)  (313,SSv2)};
% \addplot coordinates { (0,Diving48) (378,Kinetics) (1553,SSv2)};
% \addplot coordinates {(209,Diving48) (0,Kinetics) (9,SSv2)};

\addplot coordinates { (0,Diving48) (0.09765625,Kinetics) (8.447265625,SSv2)};
\addplot coordinates { (89.79492188,Diving48) (81.4453125,Kinetics) (15.28320313,SSv2)};
\addplot coordinates { (0,Diving48) (18.45703125,Kinetics) (75.83007813,SSv2)};
\addplot coordinates { (10.20507813,Diving48) (0,Kinetics) (0.439453125,SSv2)};


\legend {Dynamic, Static, Joint, Residual};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis} [
    width=\axisdefaultwidth,
    height=3.2cm,
    xbar stacked,
    bar width = 10pt,
    xmin = 0,
    xmax = 100,
    %ymin=0,
    %title = \textbf{Individual Unit Analysis on Video Segmentation Architectures},
    % ylabel = Model,
    xlabel = Units Encoding Factor F (\%),
    ytick=data,
    legend style={
            draw = none,
			area legend,
			at={(0.5,1.4)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={Diving48, Kinetics, SSv2},
    enlarge x limits = {value = .1},
    %enlarge y limits={abs=0.9}
]

% \addplot  coordinates {(27,Diving48) (23,Kinetics)  (200,SSv2)};
% \addplot  coordinates {(36,Diving48)  (82,Kinetics) (4,SSv2)};
% \addplot  coordinates { (0,Diving48) (149,Kinetics) (43,SSv2)};
% \addplot  coordinates {(193,Diving48) (2,Kinetics) (9,SSv2)};

\addplot  coordinates {(10.5,Diving48) (8.9,Kinetics)  (78.1,SSv2)};
\addplot  coordinates {(14.1,Diving48)  (32.0,Kinetics) (1.5,SSv2)};
\addplot  coordinates {(0,Diving48) (58.2,Kinetics) (16.8,SSv2)};
\addplot  coordinates {(75.4,Diving48) (0.8,Kinetics) (3.5,SSv2)};
\legend {Dynamic, Static, Joint, Residual};
\end{axis}
\end{tikzpicture}
}
\vspace{-0.7cm}
\caption{Estimating the dynamic, static, joint and residual units using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}), for the SlowOnly (\textbf{left}) and FastOnly (\textbf{right}) models on Kinetics-400~\cite{carreira2017quo}, Diving48~\cite{li2018resound} and SSv2~\cite{goyal2017something}. Dynamic units arise from dynamic-biased models (\eg FastOnly) and residual units from training on Diving48.}
\label{fig:ar_dataset_indiv}
\vspace{-0.6cm}
\end{figure}
 
%\input{tex/graphs/vos_dataset_astable}
Figure~\ref{fig:ar_dataset_indiv} shows the individual units (from the last layer) for two models (one static biased, SlowOnly, and one dynamic biased, FastOnly) on Kinetics-400, Diving48 and SSv2. The SlowOnly model trained on Kinetics-400 contains only static and joint units; however, when trained on Diving48 or SSv2, both residual and dynamic units emerge, demonstrating the impact of the training dataset on producing specialized units. Unlike the SlowOnly model, the FastOnly model contains many dynamic units trained on any dataset, showing the efficacy of the architecture for producing specialized dynamic units. Interestingly, each dataset is unique in the type of units that emerge. Diving48 produces residual units, suggesting there are other factors at play beyond dynamic and static information. On the other hand, SSv2 produces the most dynamic units for both models. 
% \textcolor{red}{The supplement shows this observation is consistent with other models. }



% \begin{figure*}[t]
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 5},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1.)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(0.09765625,SlowOnly) (0.29296875,SF-Slow) (37.890625,SF-Fast) (20.3125,FastOnly) (0.0,MViT)};
% \addplot coordinates {(78.41796875,SlowOnly) (64.94140625,SF-Slow) (30.078125,SF-Fast) (23.046875,FastOnly) (76.5625,MViT)};
% \addplot coordinates {(21.484375,SlowOnly) (34.619140625,SF-Slow) (29.296875,SF-Fast) (46.09375,FastOnly) (23.4375,MViT)};
% \addplot coordinates {(0.0,SlowOnly) (0.146484375,SF-Slow) (2.734375,SF-Fast) (10.546875,FastOnly) (0.0,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \hfill
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 4},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(0.48828125,SlowOnly) (14.53125,SF-Slow) (41.40625,SF-Fast) (39.0625,FastOnly) (0.13020833333333334,MViT)};
% \addplot coordinates {(41.015625,SlowOnly) (36.71875,SF-Slow)  (3.125,SF-Fast) (6.25,FastOnly) (43.619791666666664,MViT)};
% \addplot coordinates {(58.49609375,SlowOnly) (48.671875,SF-Slow) (55.46875,SF-Fast) (49.21875,FastOnly) (56.25,MViT)};
% \addplot coordinates {(0.0,SlowOnly) (0.078125,SF-Slow) (0.0,SF-Fast) (5.46875,FastOnly) (0.0,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{0.8\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 3},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(0.0,SlowOnly) (8.59375,SF-Slow) (20.3125,SF-Fast) (26.5625,FastOnly) (0.78125,MViT)};
% \addplot coordinates {(61.71875,SlowOnly) (50.15625,SF-Slow) (9.375,SF-Fast) (17.1875,FastOnly) (29.166666666666668,MViT)};
% \addplot coordinates {(38.28125,SlowOnly) (40.78125,SF-Slow) (68.75,SF-Fast) (48.4375,FastOnly) (69.53125,MViT)};
% \addplot coordinates {(0.0,SlowOnly) (0.46875,SF-Slow) (1.5625,SF-Fast) (7.8125,FastOnly) (0.5208333333333334,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 2},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(0.0,SlowOnly) (6.5625,SF-Slow) (18.75,SF-Fast) (15.625,FastOnly) (1.8229166666666667,MViT)};
% \addplot coordinates {(78.90625,SlowOnly) (66.875,SF-Slow) (6.25,SF-Fast) (31.25,FastOnly) (38.541666666666664,MViT)};
% \addplot coordinates {(21.09375,SlowOnly) (25.9375,SF-Slow) (75.0,SF-Fast) (43.75,FastOnly) (58.333333333333336,MViT)};
% \addplot coordinates {(0.0,SlowOnly) (0.625,SF-Slow) (0.0,SF-Fast) (9.375,FastOnly) (1.3020833333333333,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (\ref{eq:ind_bias_scores_diff_b}), $\lambda=0.5$ for models trained on Kinetics-400~\cite{goyal2017something}. We compare SlowOnly, SlowFast, FastOnly, and MViT at different layers. Since MViT has 16 layers, we estimate the dimensionality at layers 6, 9, 13, 16.}
% \label{fig:ar_alllayers}
% \end{figure*}





% \begin{figure*}[t]
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 5},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1.)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(0.634765625,SlowOnly) (5.224,SF-Slow) (40.234375,SF-Fast) (18.75,FastOnly) (0.0,MViT)};
% \addplot coordinates {(68.45703125,SlowOnly) (40.91796875,SF-Slow) (10.9375,SF-Fast) (24.21875,FastOnly) (83.59375,MViT)};
% \addplot coordinates {(9.716796875,SlowOnly) (20.556640625,SF-Slow) (30.078125,SF-Fast) (48.4375,FastOnly) (9.895,MViT)};
% \addplot coordinates {(21.19140625,SlowOnly) (33.30078125,SF-Slow) (18.75,SF-Fast) (8.59375,FastOnly) (6.510,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture} 
% \hfill
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 4},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(1.85546875,SlowOnly) (15.15625,SF-Slow) (46.875,SF-Fast) (39.0625,FastOnly) (3.90625,MViT)};
% \addplot coordinates {(34.47265625,SlowOnly) (30.46875,SF-Slow)  (3.125,SF-Fast) (7.03125,FastOnly) (42.317708333333336,MViT)};
% \addplot coordinates {(53.80859375,SlowOnly) (45.0,SF-Slow) (48.4375,SF-Fast) (49.21875,FastOnly) (48.697916666666664,MViT)};
% \addplot coordinates {(9.86328125,SlowOnly) (9.375,SF-Slow) (1.5625,SF-Fast) (4.6875,FastOnly) (5.078125,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \vfill
% \resizebox{0.8\textwidth}{!}{
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%     width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 3},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(1.3671875,SlowOnly) (10.46875,SF-Slow) (20.3125,SF-Fast) (26.5625,FastOnly) (9.375,MViT)};
% \addplot coordinates {(54.296875,SlowOnly) (40.15625,SF-Slow) (7.8125,SF-Fast) (15.625,FastOnly) (22.917,MViT)};
% \addplot coordinates {(36.5234375,SlowOnly) (36.5625,SF-Slow) (70.3125,SF-Fast) (50.0,FastOnly) (63.0208,MViT)};
% \addplot coordinates {(7.8125,SlowOnly) (12.8125,SF-Slow) (1.5625,SF-Fast) (7.8125,FastOnly) (4.6875,MViT)};

% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis} [xbar stacked,
%      width=\axisdefaultwidth,
%     height=5cm,
%     bar width = 10pt,
%     xmin = 0,
%     xmax = 100,
%     title = \textbf{Stage 2},
%     % ylabel = Model,
%     xlabel = Units Encoding Factor $F$ (\%),
%     ytick=data,
%     legend style={
% 			area legend,
% 			at={(0.5,1)},
% 			anchor=north,
% 			legend columns=-1},
%     % nodes near coords, # uncomment these three lines for numbers to appear by the bars
%     % point meta=explicit symbolic,
%     % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
%     symbolic y coords={SlowOnly,SF-Slow,SF-Fast,FastOnly,MViT},
%     enlarge x limits = {value = .1},
%     enlarge y limits={abs=24pt}
% ]

% \addplot coordinates {(2.734375,SlowOnly) (10.0,SF-Slow) (25.0,SF-Fast) (21.875,FastOnly) (12.239,MViT)};
% \addplot coordinates {(72.65625,SlowOnly) (60.3125,SF-Slow) (9.375,SF-Fast) (34.375,FastOnly) (28.125,MViT)};
% \addplot coordinates {(16.40625,SlowOnly) (20.9375,SF-Slow) (65.625,SF-Fast) (37.5,FastOnly) (52.34375,MViT)};
% \addplot coordinates {(8.203125,SlowOnly) (8.75,SF-Slow) (0,SF-Fast) (6.25,FastOnly) (7.2916,MViT)};
% \legend {Dynamic,Static,Joint,Residual};

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Estimates of the dynamic, static, joint and residual units using our metric for unit-wise analysis, (\ref{eq:ind_bias_scores_diff_b}), $\lambda=0.5$ for models trained on Kinetics-400~\cite{goyal2017something}. We compare SlowOnly, SlowFast, FastOnly, and MViT at different layers. Since MViT has 16 layers, we estimate the dimensionality at layers 6, 9, 13, 16.}
% \label{fig:ar_alllayers}
% \end{figure*}




% \begin{table}[t]
% \setlength\tabcolsep{4.1pt}
% 		\def\arraystretch{1.25}
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c c|cccc}
% \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{\multirow{1}{*}{Shuffle}} & \multirow{2}{*}{SlowOnly 8x8}& \multirow{2}{*}{SlowFast 8x8}  & \multirow{2}{*}{FastOnly 32x2} & \multirow{2}{*}{MViT 16x4}  \\ 
% %\multicolumn{2}{c|}{} &&&& \\
% \cline{1-2}
% Train & Inference &&&& \\ \specialrule{1.2pt}{1pt}{1pt}
% \xmark &  \xmark & 61.7 & 69.8 & 60.7 & 66.9\\ %\cline{1-6}
% \xmark & \cmark & 34.5 & 13.0 & 8.8 & 36.8 \\ %\cline{1-6}
% \cmark & \cmark & 63.7 & 65.4 & 49.8 & 66.3\\ \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{Relative Performance} & 103.2\% & 93.7\% & 82.0\% & 99.1\% \\ \specialrule{1.2pt}{1pt}{1pt}
% \end{tabular}}
% \caption{Top 1 Accuracy (\%) on Diving48 under various input shuffling settings}\label{table:d48_shuffle}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%Final Table %%%%%%%%%%%%%%%%%% (Separate D48)
% \begin{table}[t]
% \setlength\tabcolsep{4.1pt}
% 		\def\arraystretch{1.25}
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c c|cccc}
% \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{\multirow{1}{*}{Shuffle}} & \multirow{2}{*}{SlowOnly 8x8}& \multirow{2}{*}{SlowFast 8x8}  & \multirow{2}{*}{FastOnly 32x2} & \multirow{2}{*}{MViT 16x4}  \\ 
% %\multicolumn{2}{c|}{} &&&& \\
% \cline{1-2}
% Train & Inference &&&& \\ \specialrule{1.2pt}{1pt}{1pt}
% \xmark &  \xmark & 61.7 & 69.8 & 60.7 & 66.9\\ %\cline{1-6}
% \xmark & \cmark & 34.5 & 13.0 & 8.8 & 36.8 \\ %\cline{1-6}
% \cmark & \cmark & 63.7 & 65.4 & 49.8 & 66.3\\ \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{Relative Performance} & 103.2\% & 93.7\% & 82.0\% & 99.1\% \\ \specialrule{1.2pt}{1pt}{1pt}
% \end{tabular}}
% \caption{Top 1 Accuracy (\%) on Diving48 under various input shuffling settings}\label{table:d48_shuffle}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%Final Table %%%%%%%%%%%%%%%%%% (Separate SSv2)
% \begin{table}[t]
% \setlength\tabcolsep{4.1pt}
% 		\def\arraystretch{1.25}
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c c|cccc}
% \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{\multirow{1}{*}{Shuffle}} & \multirow{2}{*}{SlowOnly 8x8}& \multirow{2}{*}{SlowFast 8x8}  & \multirow{2}{*}{FastOnly 32x2} & \multirow{2}{*}{MViT 16x4}  \\ 
% %\multicolumn{2}{c|}{} &&&& \\
% \cline{1-2}
% Train & Inference &&&& \\ \specialrule{1.2pt}{1pt}{1pt}
% \xmark &  \xmark & 52.0 &  &  & 33.8\\ %\cline{1-6}
% \xmark & \cmark & 20.2 &  & & \\ %\cline{1-6}
% \cmark & \cmark & 20.2 &  & & 26.4 \\ \specialrule{1.2pt}{1pt}{1pt}
% \multicolumn{2}{c|}{Relative Performance} & 103.2\% & 93.7\% & 82.0\% & 99.1\% \\ \specialrule{1.2pt}{1pt}{1pt}
% \end{tabular}}
% \caption{Top 1 Accuracy (\%) on SSv2 under various input shuffling settings}\label{table:ssv2_shuffle}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{tex/graphs/test_groupplots}


\noindent\textbf{Datasets.} We study the impact of the following four video segmentation datasets on a model's static and dynamic biases:
DAVIS16~\cite{Perazzi2016}, Weakly Labelled ImageNet VID~\cite{jain2017fusionseg}, YouTube-VOS~\cite{xu2018youtube} and TAO-VOS~\cite{Voigtlaender21WACV}.
%: (i) DAVIS'16~\cite{Perazzi2016}, (ii) Weakly Labelled ImageNet VID~\cite{jain2017fusionseg} and (iii) TAO-VOS~\cite{Voigtlaender21WACV}.
DAVIS16~\cite{Perazzi2016} is the most widely used benchmark for automatic VOS, with 50 short-temporal extent sequences of two to four seconds and 3455 manually annotated frames. ImageNet VID~\cite{jain2017fusionseg} contains 3251 weakly labelled videos and was used in previous work to pretrain a model's motion stream~\cite{jain2017fusionseg}; in contrast, we use it as a general training dataset (\ie beyond just for motion streams). YouTube-VOS~\cite{xu2018youtube} is another widely used AVOS dataset with 3471 videos in the training set, which is usually combined with DAVIS dataset following~\cite{zhou2020motion} to end up with 14K training images. We assess the two training datasets separately and evaluate how they affect the static and dynamic biases. Finally, TAO-VOS~\cite{Voigtlaender21WACV} contains 626 relatively long videos (36 seconds on average) that are annotated in a hybrid fashion between manually and weakly labelled frames, resulting in 74,187 frames.
%It is built on the original TAO dataset that was annotating all moving objects in sequences acquired from different domains (\ie, action recognition~\cite{sigurdsson2016hollywood}\cite{gu2018ava}\cite{zhao2019hacs} and autonomous driving~\cite{yu2020bdd100k}\cite{chang2019argoverse}). 
We convert the annotations to exclude instances and instead consider foreground/background annotations only.

\noindent\textbf{Dataset bias.} We train our modified FusionSeg with two fusion layers (layers two and five) on the four datasets. We compute the static and dynamic biases for the training datasets using the layer-wise metric,
(\ref{eq:biasscores}), and report the results in Table~\ref{fig:vos_dataset}. The model trained on TAO-VOS has the least amount of static bias out of all four datasets. However, the datasets do not differ much in their dynamic bias.


\vspace{-0.2cm}
\subsubsection{Automatic video object segmentation} 
\label{sec:vos_datasets}
\begin{table}
\resizebox{0.45\textwidth}{!}{
\begin{tabu}{c cccc}
\tabucline[1pt]{-}
 \multirow{2}{*}{Dataset}&  \multicolumn{2}{c}{\textbf{Fusion Layer 5}} & \multicolumn{2}{c}{\textbf{Fusion Layer 2}}    \\
\cline{2-5}
  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)\\
\tabucline[1pt]{-}
DAVIS & 27.8 & 30.1 & 34.0 & 25.9 \\
YouTube-VOS & 25.2 & 34.2 & 33.5 & 24.9\\
ImageNetVID & 26.4 & 33.1 & 33.0 & 24.6\\
TAO-VOS & 26.4 & 25.8  & 33.7 & 23.2 \\
\tabucline[1pt]{-}
\end{tabu}}
\caption{Biases of video object segmentation datasets using the layer-wise metric, (\ref{eq:biasscores}), for FusionSeg's fusion layers five and two, trained on DAVIS16~\cite{Perazzi2016}, YouTube-VOS~\cite{xu2018youtube}, ImageNetVID~\cite{jain2017fusionseg} and TAO-VOS~\cite{Voigtlaender21WACV}.}
\label{fig:vos_dataset}
\vspace{-0.5cm}
\end{table}

%\input{tex/graphs/vos_dataset_indiv}
\begin{figure}
    \centering
\begin{minipage}{0.35\textwidth}
\resizebox{\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [
    width=\axisdefaultwidth,
    height=3.2cm,
    xbar stacked,
    bar width = 10pt,
    xmin = 0,
    xmax = 100,
    %ymin=0,
    title = \textbf{Fusion Layer 5},
    % ylabel = Model,
    %xlabel = Units Encoding Factor F (\%),
    ytick=data,
    legend style={
            draw = none,
			area legend,
			at={(0.5,1.4)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={TAO-VOS, ImageNetVID, YouTube-VOS, DAVIS},
    enlarge x limits = {value = .1},
    %enlarge y limits={abs=0.9}
] 
\addplot coordinates { (8.7890625,DAVIS) (0.9765625,ImageNetVID) (0.0,YouTube-VOS) (49.70703125,TAO-VOS)};
\addplot coordinates { ( 17.08984375,DAVIS) ( 20.654296875,ImageNetVID) (41.6,YouTube-VOS) (18.5546875,TAO-VOS)};
\addplot coordinates { ( 73.486328125,DAVIS) (78.173828125,ImageNetVID) (58.4,YouTube-VOS) (22.021484375,TAO-VOS)};
\addplot coordinates { (0.6,DAVIS) (0.1953125,ImageNetVID) (0.0,YouTube-VOS) (9.716796875,TAO-VOS)};
%\legend {Dynamic,Static,Joint, Residual};
\end{axis}
\end{tikzpicture}}

\resizebox{\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [
    width=\axisdefaultwidth,
    height=3.2cm,
    xbar stacked,
    bar width = 10pt,
    xmin = 0,
    xmax = 100,
    %ymin=0,
    title = \textbf{Fusion Layer 2},
    % ylabel = Model,
    xlabel = Units Encoding Factor $F$ (\%),
    ytick=data,
    legend style={
            draw = none,
			area legend,
			at={(0.5,-0.7)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={TAO-VOS, ImageNetVID, YouTube-VOS, DAVIS},
    enlarge x limits = {value = .1},
    %enlarge y limits={abs=0.9}
] 
 % [0.70703125, 0.03515625, 0.23828125, 0.01953125]
\addplot coordinates { (32.421875,DAVIS) (60.15625,ImageNetVID) (48.4,YouTube-VOS) (70.703125,TAO-VOS)};
\addplot coordinates { (12.109375,DAVIS) (8.203125,ImageNetVID) (7.0,YouTube-VOS) (3.515625,TAO-VOS)};
\addplot coordinates { (54.296875,DAVIS) (30.46875,ImageNetVID) (42.6,YouTube-VOS) (23.828125,TAO-VOS)};
\addplot coordinates { (1.171875,DAVIS) (1.171875,ImageNetVID) (2.0,YouTube-VOS) (1.953125,TAO-VOS)};
 
\legend {Dynamic, Static, Joint, Residual};
\end{axis}
\end{tikzpicture}}
\end{minipage}%
\begin{minipage}{0.13\textwidth}
\resizebox{\textwidth}{!}{
\includegraphics[width=\textwidth]{images/SaliencyPriors.pdf}}
\end{minipage}
\vspace{-0.2cm}
\caption{Analyses of biases of AVOS datasets. \textbf{Left}: Estimating the dynamic, static, joint and residual units using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}), for FusionSeg's fusion layers five and two trained on DAVIS16~\cite{Perazzi2016}, YouTube-VOS~\cite{xu2018youtube}, ImageNetVID~\cite{jain2017fusionseg} and TAO-VOS~\cite{Voigtlaender21WACV}. \textbf{Right}: Center bias plots for the four datasets. The results show the emergence of more dynamic units for both fusion layers when trained on the least center biased dataset (\ie TAO-VOS).}
\label{fig:vos_dataset_indiv}
\vspace{-0.6cm}
\end{figure}

% \noindent\textbf{Individual units analysis.} 
We analyse the datasets in terms of the individual unit analysis using the unit-wise metric, (\ref{eq:ind_bias_scores_diff_b}), with $\lambda=0.5$. It is seen in Fig.~\ref{fig:vos_dataset_indiv} (left) that models trained on TAO-VOS produce the highest number of specialized dynamic biased units compared to the other datasets. To explore this matter further, we evaluate the center bias for the four datasets by calculating the average number of groundtruth segmentation masks for each pixel over the entire dataset (normalized to 0-1), with results shown in Fig.~\ref{fig:vos_dataset_indiv} (right). It is seen that for both layers, the percentage of specialized dynamic units is greatest for the dataset that has least center bias, \ie TAO-VOS, as its center bias map is far more diffuse than the others. These results have implications for how the datasets can be used best for different tasks. For example, more general motion segmentation without concern for centering might be better served by training with a dynamic biased dataset (\eg TAO-VOS).





\begin{figure} [t]
	\begin{center}
     \centering 
    %  \begin{minipage}{0.25\textwidth}
% 		\resizebox{\textwidth}{!}{
%      \begin{tikzpicture}  \ref{legend_vis_dataset_layer}
%      \begin{axis} [
%      line width=1.0,
%                  title={\textbf{VIS - Layerwise}},
%                  title style={at={(axis description cs:0.5,0.95)},anchor=north,font=\normalsize},
%                  xlabel={Network Layer},
%                  ylabel={Number of Units (\%)},
%                  xmin=0.5, xmax=12.5,
%                  ymin=20, ymax=45,
%                  xtick={2,4,6,8,10,12},
%                  ytick={15,20,25,30,35,40,45},
%                  x tick label style={font=\small},
%                  y tick label style={font=\small},
%                  x label style={at={(axis description cs:0.5,0.085)},anchor=north,font=\normalsize},
%                  y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\normalsize},
%                  xtick pos=left,
%                  ytick pos=bottom,
%                  width=6.5cm,
%                  height=5cm,
%                  ymajorgrids=false,
%                  xmajorgrids=false,
%                  major grid style={dotted,green!20!black},
%                  legend style={
%                      %draw=none,
%                      nodes={scale=0.7, transform shape},
%                      cells={anchor=west},
%                      legend style={at={(2.9,1)},anchor=south}, font =\small},
%                      legend columns=2,
%                      legend entries={[black]OVIS-Dyn,[black]OVIS-Stat,[black]YTVIS-Dyn,[black]YTVIS-Stat},
%                     legend to name=legend_vis_dataset_layer,
%         ]

%             %OVIS-Dyn
%             \addplot[line width=1.2pt,mark options={line width=0.8pt,scale=1,solid}, color=blue, mark=square, style=dashdotted]
%                      coordinates {(1,24.2)
%                                   (2,24.2)
%                                   (3,23.7)
%                                   (4,24.2)
%                                   (5,24.7)
%                                   (6,26.3)
%                                   (7,21.4)
%                                   (8,21.1)
%                                   (9,21.4)
%                                   (10,21.4)
%                                   (11,21.4)
%                                   (12,21.4)};
%             %OVIS-Stat            
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=oplus, style=dashdotted]
%                      coordinates {(1,37.2)
%                                   (2,36.7)
%                                   (3,37)
%                                   (4,36.5)
%                                   (5,35.4)
%                                   (6,34.6)
%                                   (7,38.5)
%                                   (8,38.5)
%                                   (9,38.3)
%                                   (10,38.3)
%                                   (11,38.3)
%                                   (12,38.3)};
                       
                                  
%             %YTVIS-Dyn
%             \addplot[line width=1pt,mark options={line width=0.8pt,scale=1.1,solid}, color=blue, mark=triangle, style=solid]
%                      coordinates {(1,22.4)
%                                   (2,22.1)
%                                   (3,21.9)
%                                   (4,21.6)
%                                   (5,21.9)
%                                   (6,21.9)
%                                   (7,22.9)
%                                   (8,22.7)
%                                   (9,22.7)
%                                   (10,22.7)
%                                   (11,22.7)
%                                   (12,22.1)};
%              %YTVIS-Stat                     
%             \addplot[line width=1pt, mark options={line width=0.5pt,scale=1.2,solid}, color=red, mark=+, style=solid]
%                      coordinates {(1,38.5)
%                                   (2,38.5)
%                                   (3,38.8)
%                                   (4,39.3)
%                                   (5,39.3)
%                                   (6,39.6)
%                                   (7,38)
%                                   (8,38)
%                                   (9,38)
%                                   (10,38)
%                                   (11,38)
%                                   (12,38.5)};
                                  
%         \end{axis}
% \end{tikzpicture}
\begin{minipage}{0.28\textwidth}
\resizebox{1.0\textwidth}{!}{
	\begin{tabu}{c cccc}
	\tabucline[1pt]{-}
	 \multirow{2}{*}{Dataset}&  \multicolumn{2}{c}{\textbf{Layer 6}} & \multicolumn{2}{c}{\textbf{Layer 12}} \\
	 \cline{2-3} \cline{4-5}
	%\hline
	  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)\\
	   \tabucline[1pt]{-}
	   YTVIS~\cite{yang2019video} & 21.9 & 39.6 & 22.1 & 38.5   \\
	   OVIS~\cite{qi2022occluded} & 26.3 & 34.6 & 21.4 & 38.3 \\
	  % \hline
	\tabucline[1pt]{-}
	\end{tabu}}
\end{minipage} \hfill   
\begin{minipage}{0.2\textwidth}
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 6},
    title style={at={(axis description cs:0.5,1.4)},anchor=north,font=\Large},
    x tick label style={font=\large},
    y tick label style={font=\large},
    x label style={at={(axis description cs:0.5,0.07)},anchor=north,font=\large},
    y label style={at={(axis description cs:0.17,.5)},anchor=south,font=\large},
    ytick=data,
    legend style={
         draw=none,
         legend style={row sep=0.1pt},
        nodes={scale=0.87, transform shape},
        legend columns=-1,
        cells={anchor=west},
        legend style={at={(0.5,2.2)},anchor=north,row sep=0.01pt}, font =\Large},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={OVIS,YTVIS},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]

% AVERAGE
% \addplot coordinates {(0,OVIS) (0,YTVIS)};
% \addplot coordinates {(59.2,OVIS) (72.8,YTVIS)};
% \addplot coordinates {(40.8,OVIS) (27.2,YTVIS)};
% \addplot coordinates {(0.0,OVIS) (0.0,YTVIS)};

% LAST LAYER
\addplot coordinates {(0,OVIS) (0,YTVIS)};
\addplot coordinates {(50.8,OVIS) (68.2,YTVIS)};
\addplot coordinates {(49.2,OVIS) (31.8,YTVIS)};
\addplot coordinates {(0.0,OVIS) (0.0,YTVIS)};

\legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture} 
}
\vfill
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}
\begin{axis} [xbar stacked,
    width=8cm,
    height=2.6cm,
    bar width = 8pt,
    xmin = 0,
    xmax = 100,
    title = \textbf{Layer 12},
    title style={at={(axis description cs:0.5,1.4)},anchor=north,font=\Large},
    xlabel = Units Encoding Factor $F$ (\%),
    x tick label style={font=\large},
    y tick label style={font=\large},
    xlabel style={at={(axis description cs:0.5,0.0)},anchor=north,font=\Large},
    ytick=data,
    legend style={
			area legend,
			at={(0.5,1)},
			anchor=north,
			legend columns=-1},
    % nodes near coords, # uncomment these three lines for numbers to appear by the bars
    % point meta=explicit symbolic,
    % nodes near coords align={west}, % need to get these aligned correctly, should be different for each factor i.e., (right, left, left, right)
    symbolic y coords={OVIS,YTVIS},
    enlarge x limits = {value = .1},
    enlarge y limits={abs=8pt}
]
% AVERAGE
% \addplot coordinates {(0,OVIS) (0,YTVIS)};
% \addplot coordinates {(77.4,OVIS) (57.2,YTVIS)};
% \addplot coordinates {(22.6,OVIS) (42.8,YTVIS)};
% \addplot coordinates {(0.0,OVIS) (0.0,YTVIS)};

% LAST LAYER
\addplot coordinates {(0,OVIS) (0,YTVIS)};
\addplot coordinates {(76.3,OVIS) (59.9,YTVIS)};
\addplot coordinates {(23.7,OVIS) (40.1,YTVIS)};
\addplot coordinates {(0.0,OVIS) (0.0,YTVIS)};

% \legend {Dynamic,Static,Joint,Residual};

\end{axis}
\end{tikzpicture}
}

\end{minipage}
	\end{center}
	\vspace{-0.3cm}
	\caption{Analyses of biases of VIS datasets. \textbf{Left:} Results for the static and dynamic biases using the layer-wise metric, (\ref{eq:biasscores}), for layers 6 and 12 of VisTR-R50 trained on OVIS~\cite{qi2022occluded} and YTVIS~\cite{yang2019video}. \textbf{Right:} Unit-wise analysis, (\ref{eq:bias_scores_indv}), of a VisTR-R50 model trained on both datasets for layers 6 and 12.}\label{fig:inst_vos_dataset}
	\vspace{-0.4cm}
\end{figure}


% For both datasets, all training settings are the same as in the original paper~\cite{wang2021end} except for we train for four epochs and use 24 input frames.
 

\vspace{-0.2cm}
\subsubsection{Video instance segmentation}\label{sec:vis_dataset}

\noindent \textbf{Datasets.} We study the impact of the following two datasets on a VIS model's static and dynamic biases:  YouTube-VIS 2019 (YTVIS)~\cite{yang2019video} and Occluded Video Instance Segmentation (OVIS)~\cite{qi2022occluded}. YTVIS is a popular VIS benchmark and contains 2,883 videos, 40 categories, 131k total masks, an average of 1.7 instances per video and an average video length of 4.6 seconds. OVIS contains 901 videos and corresponding annotations of \textit{occluded objects} (\ie masks of occluded objects are also labelled). OVIS contains 901 videos, 25 categories, 296k masks, an average of 5.8 instances per video and an average video length of 10.1 seconds. Both datasets are manually labelled every 5 frames.


\noindent \textbf{Dataset bias.} Figure~\ref{fig:inst_vos_dataset} (left) shows the static and dynamic biases of a VisTR-R50 model trained on both datasets using the layer-wise metric, (\ref{eq:biasscores}). The model trained on OVIS contains notably more dynamic bias than the YTVIS trained model in the last layer of the encoder (\ie layer six) while the biases are similar in the final decoder layer (\ie layer 12). This result is further demonstrated when observing the unit-wise results, (\ref{eq:bias_scores_indv}), shown in Fig.~\ref{fig:inst_vos_dataset} (right). While both datasets produce solely static and joint units, the model trained on OVIS produces more jointly encoding units in the encoder than the model trained on YTVIS and the opposite is true in the decoder. 
These results suggest that while dynamics are learned in the encoding layers, the model may lack the ability to decode the dynamics. 
We observe a similar pattern when comparing to the biases of action recognition transformers (Sec.~\ref{sec:ar_models}) where solely static and joint units also are produced. This pattern might be due to the mixing of information that is present in self-attention layers, which could inhibit specialized dynamic units from emerging. An interesting future direction suggested by these results is the design of self-attention layers which can admit specialized dynamic units throughout the model (\eg by introducing two streams, as in the SlowFast model). The unit-wise results show that OVIS has a similar pattern to TAO-VOS: When moving deeper through the model, less dynamic and joint units are produced while more static units emerge. Contrastingly, all other AVOS datasets and YTVIS produce notably more joint units in the final layer. This pattern suggests that OVIS may be a better dataset for pre-training if the goal is for the model to encode maximal dynamics.





% The first takeaway from these results is that segmenting occluded objects requires a different distribution of static and dynamic information throughout the architecture.

% More specifically, it seems that dynamics and jointly encoding units are learned in the first few layers of the model, while static information becomes more important near the final segmentation layer. 

% This could have implications for architectural design such as implementing occlusion-specific architecture modifications in the encoder to better track occluded objects.


\subsubsection{Summary and shared insights}
For action recognition, our results raise questions about some of the widely adopted datasets. In particular, Diving48 is claimed to be a good benchmark for learning dynamics~\cite{li2018resound}, while our results suggest that SSv2 is better suited for evaluating a model's ability to capture dynamics. In AVOS, we found training on TAO-VOS yields the largest number of specialized dynamic units. Thus, it may be a better training dataset for tasks that rely on capturing dynamics (\eg motion segmentation). Similarly, for VIS, we demonstrated that OVIS may provide a better signal for learning dynamic information, particularly in the earlier layers of a network.

% In video object segmentation, we found the training on TAO-VOS yields the \textcolor{blue}{largest number of specialized dynamic units in comparison to DAVIS and ImageNet VID.}

%In action recognition, we measured the static and dynamic information contained in three popular action recognition datasets. While models trained on SSv2 consistently contain more dynamic units, Diving48 and Kinetics-400 were both more biased toward static information.

%\begin{table*}[]
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
%\hline
%\multicolumn{4}{|l|}{} & \multicolumn{6}{l|}{Success Rate} \\ \hline
%Model & RGB & Flow & $\mathcal{J}$ & $\tau = 0.5$  & $\tau = 0.6$  & $\tau = 0.7$  & $\tau = 0.8$  & $\tau = 0.9$  & $SR_{\text{mean}}$  \\ \hline
%COD & \xmark   & \cmark &  44.9  &  41.4 & 33.0  & 23.5 & 14.0   & 5.9  &  23.6 \\ \hline
%COD (Two-stream) & \cmark  & \cmark & 55.3    & 60.2  & 52.3  & 41.3  & 26.7  & 8.8  &  37.9 \\ \hline
%COSNet & \cmark  & \xmark    &  50.7   &  58.8 &  53.4 &  45.7 & 33.7  & 16.7  & 41.7  \\ \hline
%RTNet (ResNet34) & \cmark & \cmark    &  55.0   & 62.2  &  57.4  &  48.0 & 38.4  & 21.0  &  47.0 \\ \hline
%RTNet (ResNext50) & \cmark & \cmark    & 60.7 &  68.0 & 62.4  & 53.6  & 43.4  & 23.9  &  52.0 \\ \hline
%Our Reproduced & \cmark & \cmark    & 66.4  & 77.6 &  71.3 &  59.6 &  43.3 &  19.3  &  \\ \hline
%3D MATNet (SingleGPU, T=10) & \cmark & \cmark   & 61.1  & 70.8 & 63.5  & 52.5  & 36.4 & 14.1  &  \\ \hline
%MATNet & \cmark & \cmark    & \textbf{64.2}  &  \textbf{71.2} & \textbf{67.0}  & \textbf{59.9}  & \textbf{49.2}  & \textbf{24.6}  & \textbf{54.4}  \\ \hline
%Our Reproduced (MultiGPU) & \cmark & \cmark   & 67.8  & 78.0 & 72.3  & 61.3  & 45.2 &  21.5 &  \\ \hline
%3D MATNet (MultiGPU, T=5) & \cmark & \cmark    &  64.8 & 74.0 & 67.4 & 56.5 & 40.8 & 16.8  &  \\ \hline
%3-Stream (MultiGPU, T=5) & \cmark & \cmark    &  58.4 & 66.7 & 58.4 & 45.5 & 29.4 & 10.3  &  \\ \hline \hline
%
%\multicolumn{10}{c}{Temporal Ablation} \\ \hline
%
%3D MATNet (MultiGPU, T=5,S=1) & \cmark & \cmark    &  63.7 & 75.0 & 65.9 & 65.6 & 53.5 & 14.2  &  \\ \hline
%3D MATNet (MultiGPU, T=5,S=2) & \cmark & \cmark    &  60.8 & 70.2 & 63.4 & 51.9 & 35.6 & 16.0  &  \\ \hline
%3D MATNet (MultiGPU, T=5,S=3) & \cmark & \cmark    &  62.4 & 73.1 & 66.0 & 53.7 & 37.1 &  16.6 &  \\ \hline
%3D MATNet (MultiGPU, T=10,S=1) & \cmark & \cmark    &  61.3 & 70.7 & 62.4 & 50.9 & 36.7 & 13.8  &  \\ \hline
%3D MATNet (MultiGPU, T=10,S=2) & \cmark & \cmark    &  62.4 & 72.2 & 62.0 & 48.0 & 30.5 & 9.4  &  \\ \hline
%3D MATNet (MultiGPU, T=10,S=3) & \cmark & \cmark    &  61.4 & 69.9 & 62.6 & 52.0 & 37.3 & 14.3  &  \\ \hline
%TAttention MATNet (MultiGPU, T=5, S=1) & \cmark & \cmark & 61.4  & 72.9 & 66.2 & 54.7 & 35.6 & 12.7 &  \\ \hline
%TAttention + WarpingMATNet (MultiGPU, T=5, S=1) & \cmark & \cmark & 61.4 & 71.0 & 62.7 & 50.7 & 33.8 & 11.5 &  \\ \hline
%TAttention + WarpingMATNet (MultiGPU, T=5, S=2) & \cmark & \cmark &  &  &  &  &  &  &  \\ \hline
%%MATNet (10\% Removed Residual) & \cmark & \cmark    & 63.9  & 71.5 & 66.6 & 58.1 & 44.7 & 21.5 & \\ \hline
%%MATNet (20\% Removed Residual) & \cmark & \cmark    & 63.6  &   70.9 & 65.9 & 57.5 & 44.5 & 21.4  &  \\ \hline
%%MATNet (30\% Removed Residual) & \cmark & \cmark    & 63.0  & 70.3 & 65.2 & 56.7 & 44.3 & 21.4  &  \\ \hline
%%MATNet (40\% Removed Residual) & \cmark & \cmark    & 63.0  & 70.2 & 65.0 & 56.7 & 44.2 & 21.8 &  \\ \hline
%%MATNet (50\% Removed Residual) & \cmark & \cmark    & 62.3  & 69.2 & 64.2 & 56.3 & 43.6 & 21.6 &  \\ \hline
%%Ours & \cmark  & \cmark &     &   &   &   &   &   &   \\ \hline
%\end{tabular}
%\end{table*}

% baseline at thresh=0.4: Js: (0.614). SR at 0.5: (0.690), 0.6: (0.631), 0.7: (0.536), 0.8: (0.415), 0.9: (0.211)
% baseline at thresh=0.1: Js: (0.678). SR at 0.5: (0.780), 0.6: (0.723), 0.7: (0.613), 0.8: (0.452), 0.9: (0.215),
% Two Str Att only, thresh = 0.4, (0.593). SR at 0.5: (0.690), 0.6: (0.627), 0.7: (0.526), 0.8: (0.396), 0.9: (0.181)
% Two Str Att only, thresh = 0.1, Js: (0.614). SR at 0.5: (0.729), 0.6: (0.662), 0.7: (0.547), 0.8: (0.356), 0.9: (0.127),
% Att + Warping, thresh = 0.3, Js: (0.633). SR at 0.5: (0.732), 0.6: (0.674), 0.7: (0.569), 0.8: (0.396), 0.9: (0.180),
% Baseline at thresh = 0.3,   Js: (0.650). SR at 0.5: (0.738), 0.6: (0.683), 0.7: (0.590), 0.8: (0.458), 0.9: (0.233),
% Att only thresh = 0.3, Js: (0.615). SR at 0.5: (0.717), 0.6: (0.656), 0.7: (0.561), 0.8: (0.421), 0.9: (0.185),

% After the fix: 
% Att + Warping, thresh=0.3, Js: (0.636). SR at 0.5: (0.736), 0.6: (0.677), 0.7: (0.571), 0.8: (0.397), 0.9: (0.180),
% Att only, thresh=0.3, Js: (0.616). SR at 0.5: (0.717), 0.6: (0.656), 0.7: (0.561), 0.8: (0.421), 0.9: (0.186),
% Baseline, thresh=0.3, Js: (0.651). SR at 0.5: (0.739), 0.6: (0.683), 0.7: (0.590), 0.8: (0.459), 0.9: (0.234),


%\input{tex/graphs/vos_layer-wise_4factors}
%\input{tex/graphs/vos_moca}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Jointly Encoding and Dynamic Units Analysis} % Use this broader term to indicate both joint and residuals as correlated to Neither
% \label{sec:per-unit}

%\input{tex/graphs/ar_datasets}

%\input{tex/graphs/vos_moca}

\begin{figure} [t]
\begin{center}
     \centering 
		\resizebox{0.47\textwidth}{!}{
		\begin{tikzpicture}[trim axis left,trim axis right]\ref{legend_i3d}
    \begin{axis}[
      line width=1.0,
        title={\textbf{I3D}},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
        xlabel={\% of Training Epochs},
        x label style={font=\small},
        ylabel={Dimensions (\%)},
        xmin=0, xmax=102,
        ymin=9, ymax=44,
        xtick={0,10,20,30,40,50,60,70,80,90},
        ytick={15, 20, 25, 30, 35, 40},
        x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        y label style={at={(axis description cs:.14,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend style={
         legend columns=3,
         nodes={scale=0.75, transform shape},
         cells={anchor=west},
         legend style={at={(3.05,0.13)},anchor=south,row sep=0.01pt}, font =\small},
         legend entries={[black]K400-Dyn,[black]K400-Stat,[black]D48-Dyn,[black]D48-Stat,[black]SSv2-Dyn,[black]SSv2-Stat},
        legend to name=legend_i3d,
    ]
    % I3D-K400 MOTION
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=blue, style=solid]
        coordinates {(0,20.9)(2.5,22.5)(5,24.0)(7.5,23.9)(10,24.0)(12.5,24.0)(15,24.8)(17.5,23.6)(20,24.5)(22.5,24.3)(25,24.2)(27.5,22.9)(30,25.0)(35,24.3)(37.5,24.3)(40,23.2)(42.5,24.1)(45,24.2)(47.5,25.4)(52.5,23.1)(55,24.3)(57.5,23.8)(60,23.9)(67.5,24.9)(70,24.6)(72.5,24.7)(75,23.6)(77.5,24.6)(80,23.9)(82.5,23.3)(85,23.9)(90,23.7)(92.5,23.6)(95,23.6)(100,23.3)};
    % I3D-K400 APPEARANCE
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=solid]
        coordinates {(0,38.5)(2.5,37.9)(5,36.4)(7.5,36.3)(10,35.8)(12.5,35.6)(15,34.7)(17.5,35.6)(20,35.0)(22.5,34.6)(25,34.9)(27.5,36.2)(30,34.4)(35,35.1)(37.5,35.0)(40,35.3)(42.5,34.9)(45,34.6)(47.5,33.3)(52.5,35.4)(55,34.8)(57.5,35.3)(60,35.0)(67.5,34.2)(70,34.2)(72.5,34.0)(75,35.1)(77.5,34.2)(80,35.1)(82.5,35.5)(85,34.9)(90,35.0)(92.5,35.0)(95,35.1)(100,35.3)};
        
    % I3D-D48 MOTION
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=blue, style=dashed]
        coordinates {(0,14.8)(5,17.5)(10,17.4)(15,16.4)(20,17.6)(25,17.0)(30,17.4)(35,17.0)(40,17.3)(45,18.0)(50,17.6)(55,17.2)(60,17.5)(65,17.3)(70,17.6)(75,17.4)(80,17.6)(85,17.7)(90,17.9)(95,17.5)(100,17.5)};
    % I3D-D48 APPEARANCE
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=dashed]
        coordinates {(0,41.7)(5,38.9)(10,37.8)(15,39.6)(20,37.6)(25,38.7)(30,38.8)(35,38.8)(40,38.3)(45,37.6)(50,38.2)(55,38.6)(60,38.4)(65,38.2)(70,38.2)(75,38.2)(80,38.1)(85,38.0)(90,37.7)(95,38.2)(100,38.4)}; 
        
        
    % I3D ssv2 MOTION
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=blue, style=densely dotted]
        coordinates {(0,15.6)(3.33,25.6)(6.66,29.5)(10,28.7)(13.33,30.7)(16.66,30.4)(20,28.6)(23.33,33.5)(26.66,32.2)(30,33.3)(33.33,30.0)(36.66,28.6)(40,31.1)(43.33,30.1)(46.66,29.1)(50,34.1)(53.33,29.9)(56.66,30.2)(60,32.9)(63.33,29.5)(66.66,30.5)(70,29.7)(73.33,29.1)(76.66,29.4)(80,32.8)(83.33,30.7)(86.66,32.8)(90,30.0)(93.33,29.9)(96.66,30.5)(100,29.7)};
    %  I3D ssv2 APPEARANCE
    \addplot[line width=1.2pt,  mark options={line width=0.5pt,scale=1.2,solid}, color=red, style=densely dotted]
        coordinates {(0,42.6)(3.33,35.0)(6.66,31.2)(10,30.7)(13.33,28.2)(16.66,28.0)(20,30.2)(23.33,25.3)(26.66,27.3)(30,26.3)(33.33,29.1)(36.66,30.0)(40,27.3)(43.33,28.6)(46.66,29.8)(50,24.7)(53.33,28.8)(56.66,28.6)(60,26.3)(63.33,29.7)(66.66,28.5)(70,29.4)(73.33,30.3)(76.66,29.6)(80,26.2)(83.33,28.4)(86.66,26.5)(90,28.9)(93.33,28.9)(96.66,28.4)(100,29.0)};
    
\end{axis}


\end{tikzpicture}
\hspace{0.3cm}
\begin{tikzpicture}[trim axis left,trim axis right]\ref{two_stream_leg}
    \begin{axis}[
      line width=1.0,
        title={\textbf{SlowFast - K400}},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
        xlabel={Epoch},
        x label style={font=\small},
        % ylabel={Dimensions (\%)},
        xmin=0, xmax=200,
        ymin=10, ymax=42,
        xtick={0,20,40,60,80,100,120,140,160,180},
        ytick={15, 20, 25, 30, 35, 40},
        x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        % major grid style={dotted,green!20!black},
        % legend style={
        %  nodes={scale=0.5, transform shape},
        %  cells={anchor=west},
        %  legend style={at={(1.6,3.4)},anchor=south,row sep=0.01pt}, font =\small},
        %  legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
        % legend to name=target_legend7,
    ]

        % SLOW
        % MOTION
    \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,20.0)(5,22.5)(10,23.3)(15,25.0)(25,24.5)(45,26.5)(50,25.4)(60,28.5)(75,23.8)(80,24.4)(85,24.7)(90,24.7)(95,26.0)(105,24.7)(110,24.3)(115,23.7)(120,24.3)(125,23.7)(130,25.5)(140,24.1)(145,23.0)(150,23.5)(155,24.6)(160,24.1)(165,23.9)(170,24.3)(175,24.2)(180,23.4)(185,24.1)(190,24.0)};
    % APPEARANCE
    \addplot[line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,39.6)(5,35.9)(10,23.3)(15,25.0)(25,34.0)(45,29.1)(50,30.7)(60,28.3)(75,34.0)(80,33.4)(85,32.5)(90,32.5)(95,31.4)(105,31.7)(110,31.1)(115,33.9)(120,33.7)(125,34.5)(130,31.1)(140,33.9)(145,33.3)(150,33.9)(155,32.7)(160,32.9)(165,33.4)(170,33.0)(175,32.8)(180,33.5)(185,32.9)(190,32.9)};
        
        % FAST
        % MOTION
    \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,22.3)(5,25.8)(10,27.3)(15,28.5)(25,27.7)(45,32.0)(50,31.2)(60,29.7)(75,28.5)(80,30.9)(85,31.6)(90,31.6)(95,32.8)(105,29.3)(110,31.6)(115,31.2)(120,33.6)(125,33.6)(130,31.2)(140,30.5)(145,30.9)(150,32.0)(155,32.4)(160,30.5)(165,31.2)(170,30.9)(175,30.1)(180,30.1)(185,30.9)(190,29.7)};
    % APPEARANCE
     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,38.3)(5,32.4)(10,27.0)(15,25.0)(25,27.0)(45,23.0)(50,23.4)(60,22.7)(75,21.9)(80,21.9)(85,22.7)(90,20.7)(95,20.7)(105,21.9)(110,23.0)(115,23.4)(120,21.9)(125,22.3)(130,20.7)(140,22.7)(145,22.7)(150,21.9)(155,22.7)(160,22.7)(165,22.7)(170,21.1)(175,21.9)(180,23.4)(185,22.3)(190,22.7)};
\end{axis}


\end{tikzpicture}
}
\resizebox{0.47\textwidth}{!}{
\begin{tikzpicture}[trim axis left,trim axis right]\ref{two_stream_leg}
    \begin{axis}[
      line width=1.0,
        title={\textbf{SlowFast - Diving48}},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
        % xlabel={Epoch},
        x label style={font=\small},
        xmin=0, xmax=101,
        ymin=8, ymax=44,
        xtick={0,10,20,30,40,50,60,70,80,90,100},
        ytick={15,20,25,30,35,40},
        ylabel={Dimensions (\%)},
        x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        y label style={at={(axis description cs:.15,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        % major grid style={dotted,green!20!black},
        % legend style={
        %  nodes={scale=0.7, transform shape},
        %  cells={anchor=west},
        %  legend style={at={(1.9,3.4)},anchor=south,row sep=0.01pt}, font =\normalsize},
        %  legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
        % legend to name=target_legend7,
    ]

        % SLOW
        % MOTION
    \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,14.8)(5,22.1)(10,22.9)(15,22.9)(20,24.2)(25,24.9)(30,24.3)(35,25.1)(40,24.5)(45,24.8)(50,24.9)(55,24.6)(60,24.1)(65,24.2)(70,24.1)(75,24.7)(80,24.5)(85,24.3)(90,24.4)(95,24.1)(100,24.1)};
    % APPEARANCE
    \addplot[line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,42.8)(5,31.2)(10,29.9)(15,31.0)(20,28.9)(25,27.7)(30,28.2)(35,27.2)(40,27.6)(45,27.9)(50,28.2)(55,27.9)(60,28.9)(65,28.8)(70,28.7)(75,27.9)(80,28.0)(85,28.4)(90,28.2)(95,28.4)(100,28.7)};
        
        
        
        % FAST
        % MOTION
    \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,15.2)(5,27.3)(10,28.9)(15,28.5)(20,32.4)(25,27.0)(30,31.2)(35,29.3)(40,28.5)(45,24.7)(50,29.7)(55,28.9)(60,28.9)(65,29.3)(70,30.1)(75,28.9)(80,28.5)(85,29.7)(90,28.9)(95,28.5)(100,29.3)};
    % APPEARANCE
     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,41.0)(5,21.5)(10,19.1)(15,21.1)(20,17.2)(25,21.1)(30,19.5)(35,20.3)(40,21.5)(45,27.7)(50,19.5)(55,20.3)(60,19.9)(65,20.3)(70,19.5)(75,19.9)(80,19.5)(85,19.9)(90,20.3)(95,19.9)(100,19.9)};
\end{axis}
\end{tikzpicture}
\hspace{0.3cm}
\begin{tikzpicture}[trim axis left,trim axis right]\ref{two_stream_leg}
    \begin{axis}[
      line width=1.0,
        title={\textbf{SlowFast - SSv2}},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
        % xlabel={Epoch},
        x label style={font=\small},
        % ylabel={Dimensions (\%)},
        xmin=0, xmax=23,
        ymin=13, ymax=45,
        xtick={1,3,5,7,9,11,13,15,17,19,21},
        ytick={20, 25, 30, 35, 40},
        x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        % major grid style={dotted,green!20!black},
        legend style={
		 legend columns=2,
         nodes={scale=0.85, transform shape},
         cells={anchor=west},
         legend style={at={(3,0.13)},anchor=south,row sep=0.01pt}, font =\normalsize},
         legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
        legend to name=two_stream_leg,
    ]

        % SLOW
        % MOTION
    \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,15.0)(2,31.2)(4,30.1)(6,29.2)(8,29.2)(10,29.1)(12,29.0)(14,28.7)(16,28.7)(18,28.6)(20,28.5)(22,28.5)};
    % APPEARANCE
    \addplot[line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,42.1)(2,25.8)(4,24.0)(6,22.7)(8,24.4)(10,24.5)(12,24.3)(14,23.4)(16,23.8)(18,23.5)(20,24.0)(22,23.8)};
        
        % FAST
        % MOTION
    \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
        coordinates {(0,14.1)(2,30.1)(4,31.2)(6,29.3)(8,30.5)(10,32.0)(12,30.9)(14,31.6)(16,32.8)(18,32.8)(20,32.0)(22,33.2)};
    % APPEARANCE
     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
        coordinates {(0,43.0)(2,26.6)(4,22.3)(6,21.9)(8,23.0)(10,23.8)(12,24.6)(14,24.6)(16,24.2)(18,23.4)(20,23.8)(22,23.0)};
\end{axis}

\end{tikzpicture}
}
\resizebox{0.45\textwidth}{!}{
\begin{tikzpicture}[trim axis left,trim axis right] \ref{vos_dataset_per_epoch_legend}
\begin{axis}[
      line width=1.0,
        title={\textbf{MATNet Fusion 2}},
        title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\large},
        xlabel={Epoch},
        x label style={font=\small},
        ylabel={Dimensions (\%)},
        xmin=0, xmax=21,
        ymin=8, ymax=55,
        xtick={1,3,5,7,9,11,13,15,17,19,21},
        ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
         x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        y label style={at={(axis description cs:.14,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        legend style={
		 legend columns=2,
         nodes={scale=0.85, transform shape},
         cells={anchor=west},
         legend style={at={(3.21,0.13)},anchor=south,row sep=0.01pt}, font =\normalsize},
         legend entries={[black]Stat-DAVIS+YTB,[black]Dyn-DAVIS+YTB,[black]Stat-DAVIS,[black]Dyn-DAVIS},
        legend to name=vos_dataset_per_epoch_legend,
    ]
    % DAVIS + YTB
  % Appearance
    \addplot[line width=1.2pt,mark size=1.1pt,color=red]
        coordinates{(1,28.8)(2,27.7)(3,27.0)(4,26.4)(5,26.2)(6,26.6)(7,26.2)(8,26.9)(9,25.5)(10,27.4)(11,27.2)(12,26.6)(13,27.0)(14,26.5)(15,26.8)(16,26.4)(17,27.7)(18,25.5)(19,26.6)(20,27.8)};
   % MOTION
   \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
            coordinates{(1,28.6)(2,30.2)(3,31.2)(4,32.5)(5,32.4)(6,31.4)(7,32.3)(8,31.3)(9,33.6)(10,30.7)(11,31.0)(12,31.6)(13,31.3)(14,32.4)(15,31.6)(16,31.6)(17,30.5)(18,33.8)(19,31.1)(20,30.6)};
    
    % DAVIS
    %APP
    \addplot[line width=1.2pt,mark size=1.1pt,color=red,style=dotted]
    coordinates{(1,35.4)(2,35.2)(3,34.4)(4,36.9)(5,31.4)(6,31.0)(7,39.0)(8,32.8)(9,37.6)(10,38.5)(11,29.4)(12,37.0)(13,35.5)(14,33.4)(15,34.0)(16,28.8)(17,31.2)(18,28.3)(19,34.5)(20,31.6)};
    % MOT
   \addplot[line width=1.2pt,mark size=1.1pt,color=blue,style=dotted]
    coordinates {(1,21.9)(2,21.4)(3,22.8)(4,20.3)(5,24.5)(6,23.1)(7,18.1)(8,22.0)(9,19.2)(10,19.6)(11,27.6)(12,19.8)(13,18.9)(14,22.5)(15,23.0)(16,23.9)(17,24.1)(18,26.0)(19,21.0)(20,24.3)};
     
\end{axis}
\end{tikzpicture}%
\hspace{0.5cm}
\begin{tikzpicture}[trim axis left,trim axis right]%\ref{vos_dataset_per_epoch_legend}
  \begin{axis}[
      line width=1.0,
        title={\textbf{MATNet - Fusion 5}},
        title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\large},
        xlabel={Epoch},
        x label style={font=\small},
        % ylabel={Dimensions (\%)},
        xmin=0, xmax=21,
        ymin=8, ymax=55,
        xtick={1,3,5,7,9,11,13,15,17,19,21},
        ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
         x tick label style={font=\small, rotate=60},
        y tick label style={font=\footnotesize},
        x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
        % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
        width=8cm,
        height=6cm,        
        ymajorgrids=false,
        xmajorgrids=false,
        % major grid style={dotted,green!20!black},
%         legend style={
% 		 legend columns=2,
%          nodes={scale=0.85, transform shape},
%          cells={anchor=west},
%          legend style={at={(3.1,0.13)},anchor=south,row sep=0.01pt}, font =\normalsize},
%          legend entries={[black]Stat-DAVIS+YTB,[black]Dyn-DAVIS+YTB,[black]Stat-DAVIS,[black]Dyn-DAVIS},
%         legend to name=vos_dataset_per_epoch_legend,
    ]
    % DAVIS + YTB
    % APP
     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
            coordinates{(1,29.5)(2,24.4)(3,31.9)(4,34.4)(5,31.6)(6,21.3)(7,33.8)(8,31.9)(9,34.7)(10,35.3)(11,16.3)(12,30.8)(13,34.7)(14,15.0)(15,14.4)(16,34.1)(17,34.3)(18,31.1)(19,32.2)(20,31.0)};
            
    % MOTION
    \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
            coordinates{(1,24.1)(2,37.0)(3,23.0)(4,24.3)(5,23.2)(6,21.2)(7,24.5)(8,23.0)(9,24.1)(10,23.5)(11,48.3)(12,23.7)(13,23.9)(14,45.0)(15,47.1)(16,24.5)(17,24.1)(18,23.6)(19,23.4)(20,24.0)};
            
    % DAVIS
    % App
    \addplot[line width=1.2pt,mark size=1.1pt,color=red,style=dotted]
        coordinates {(1,18.4)(2,16.3)(3,22.6)(4,35.8)(5,32.2)(6,33.3)(7,27.6)(8,35.2)(9,36.6)(10,34.8)(11,33.2)(12,27.3)(13,33.2)(14,33.8)(15,35.2)(16,33.3)(17,33.7)(18,33.3)(19,34.4)(20,33.5)};
    % MOTION
    \addplot[line width=1.2pt,mark size=1.1pt,color=blue,style=dotted]
        coordinates {(1,35.3)(2,41.0)(3,30.8)(4,22.1)(5,22.1)(6,20.4)(7,21.9)(8,23.1)(9,20.4)(10,23.2)(11,25.4)(12,23.1)(13,18.9)(14,24.4)(15,22.7)(16,25.0)(17,24.3)(18,24.7)(19,23.9)(20,24.8)};
    
\end{axis}
\end{tikzpicture}}
\end{center}
\vspace{-0.55cm}
	\caption{\textbf{Top and middle:} The encoding of static and dynamic bias for I3D~\cite{carreira2017quo} (8x8 R18) and SlowFast~\cite{feichtenhofer2019slowfast} (4x16 R18) over the course of training on Kinetics-400. \textbf{Bottom:} The encoding of static and dynamic bias over the course of training for MATNet trained on DAVIS and DAVIS + YouTube-VOS.}\label{fig:per_epoch}
 \vspace{-0.6cm}
\end{figure}

\vspace{-0.3cm}
\subsection{When are statics and dynamics learned in training?}
\vspace{-0.08cm}
\label{sec:epoch_effect}
Based on our previous analysis of models post-training, we now ask: ``What are characteristics of learning static and dynamic information over the course of training?''. Understanding how the models learn static and dynamic information can potentially inform researchers to build better training protocols for learning specific types of information.
% To this end, we perform an analysis using our layer-wise metric, (\ref{eq:biasscores}), on models throughout training.

\vspace{-0.3cm}
\subsubsection{Action Recognition}
We examine both a single and multi-stream architecture and choose the I3D~\cite{carreira2017quo} and SlowFast~\cite{feichtenhofer2019slowfast} models. We evaluate these models on Kinetics~\cite{carreira2017quo}, Diving48~\cite{li2018resound} and SSv2~\cite{goyal2017something} as each dataset differs in the static and dynamic information learned during training (see Sec.~\ref{sec:ar_dataset}). Figure~\ref{fig:per_epoch} (top) shows the layer-wise results for action recognition. Both the static and dynamic information are largely learned during the first half of training in all cases. Comparing both models for Kinetics-400 and Diving48 further confirms our previous finding (see Sec.~\ref{sec:ar_dataset}) that both datasets result in similar amounts of static and dynamic information. Conversely, models trained on SSv2 encode more dynamic information for both the single stream and two-stream models. The I3D model has a balance of static and dynamic information throughout training, while both branches in the SlowFast model quickly converge to be biased toward encoding dynamic information. The latter indicates that, given a model which has the ability to encode either type of information (\eg within the two branches in the SlowFast model), SSv2 will yield a greater amount of dynamics.

% \begin{figure} [t]
% \begin{center}
%      \centering 
% 		\resizebox{0.47\textwidth}{!}{
% 		\begin{tikzpicture}[trim axis left,trim axis right]%\ref{target_legend6}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{I3D - K400}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
%         % xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=200,
%         ymin=13, ymax=45,
%         xtick={0,10,20,30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180,190},
%         ytick={20, 25, 30, 35, 40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.85, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.4,0)},anchor=south,row sep=0.01pt}, font =\small},
%         %  legend entries={[black]Dynamic,[black]Static},
%         % legend to name=target_legend6,
%     ]
%     % MOTION
%     \addplot[line width=1.6pt,mark size=1.1pt,color=blue]
%         coordinates {(0,20.9)(5,22.5)(10,24.0)(15,23.9)(20,24.0)(25,24.0)(30,24.8)(35,23.6)(40,24.5)(45,24.3)(50,24.2)(55,22.9)(60,25.0)(70,24.3)(75,24.3)(80,23.2)(85,24.1)(90,24.2)(95,25.4)(105,23.1)(110,24.3)(115,23.8)(120,23.9)(135,24.9)(140,24.6)(145,24.7)(150,23.6)(155,24.6)(160,23.9)(165,23.3)(170,23.9)(180,23.7)(185,23.6)(190,23.6)(195,23.3)};
%     % APPEARANCE
%     \addplot[line width=1.6pt,mark size=1.1pt,color=red]
%         coordinates {(0,38.5)(5,37.9)(10,36.4)(15,36.3)(20,35.8)(25,35.6)(30,34.7)(35,35.6)(40,35.0)(45,34.6)(50,34.9)(55,36.2)(60,34.4)(70,35.1)(75,35.0)(80,35.3)(85,34.9)(90,34.6)(95,33.3)(105,35.4)(110,34.8)(115,35.3)(120,35.0)(135,34.2)(140,34.2)(145,34.0)(150, 35.1)(155,34.2)(160,35.1)(165,35.5)(170,34.9)(180,35.0)(185,35.0)(190,35.1)(195,35.3)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% \hspace{0.3cm}
% \begin{tikzpicture}[trim axis left,trim axis right]%\ref{target_legend7}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{SlowFast - K400}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
%         % xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=200,
%         ymin=13, ymax=45,
%         xtick={0,10,20,30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180,190},
%         ytick={20, 25, 30, 35, 40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.5, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.6,3.4)},anchor=south,row sep=0.01pt}, font =\small},
%         %  legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
%         % legend to name=target_legend7,
%     ]
%     % CAT
%     % MOTION
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=orange,mark=*,]
%     %     coordinates {(0,20.4)(5,23.1)(10,23.4)(15,25.7)(25,24.3)(45,27.2)(50,25.7)(60,28.7)(75,24.4)(80,25.7)(85,24.9)(90,25.3)(95,26.6)(105,25.3)(110,25.2)(115,24.4)(120,25.4)(125,24.8)(130,26.5)(140,25.0)(145,24.3)(150,24.6)(155,25.4)(160,25.0)(165,24.5)(170,25.0)(175,25.0)(180,24.2)(185,24.7)(190,24.5)};
%     % % APPEARANCE
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=cyan,mark=*,]
%     %     coordinates {(0,39.5)(5,35.4)(10,34.8)(15,33.4)(25,34.2)(45,28.3)(50,30.3)(60,27.6)(75,32.4)(80,31.4)(85,32.1)(90,32.2)(95,30.3)(105,30.1)(110,29.8)(115,32.7)(120,32.4)(125,32.9)(130,30.0)(140,32.2)(145,31.9)(150,32.5)(155,31.5)(160,31.5)(165,32.2)(170,31.7)(175,31.1)(180,32.3)(185,31.8)(190,31.9)};
        
%         % SLOW
%         % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,20.0)(5,22.5)(10,23.3)(15,25.0)(25,24.5)(45,26.5)(50,25.4)(60,28.5)(75,23.8)(80,24.4)(85,24.7)(90,24.7)(95,26.0)(105,24.7)(110,24.3)(115,23.7)(120,24.3)(125,23.7)(130,25.5)(140,24.1)(145,23.0)(150,23.5)(155,24.6)(160,24.1)(165,23.9)(170,24.3)(175,24.2)(180,23.4)(185,24.1)(190,24.0)};
%     % APPEARANCE
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,39.6)(5,35.9)(10,23.3)(15,25.0)(25,34.0)(45,29.1)(50,30.7)(60,28.3)(75,34.0)(80,33.4)(85,32.5)(90,32.5)(95,31.4)(105,31.7)(110,31.1)(115,33.9)(120,33.7)(125,34.5)(130,31.1)(140,33.9)(145,33.3)(150,33.9)(155,32.7)(160,32.9)(165,33.4)(170,33.0)(175,32.8)(180,33.5)(185,32.9)(190,32.9)};
        
%         % FAST
%         % MOTION
%     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,22.3)(5,25.8)(10,27.3)(15,28.5)(25,27.7)(45,32.0)(50,31.2)(60,29.7)(75,28.5)(80,30.9)(85,31.6)(90,31.6)(95,32.8)(105,29.3)(110,31.6)(115,31.2)(120,33.6)(125,33.6)(130,31.2)(140,30.5)(145,30.9)(150,32.0)(155,32.4)(160,30.5)(165,31.2)(170,30.9)(175,30.1)(180,30.1)(185,30.9)(190,29.7)};
%     % APPEARANCE
%      \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,38.3)(5,32.4)(10,27.0)(15,25.0)(25,27.0)(45,23.0)(50,23.4)(60,22.7)(75,21.9)(80,21.9)(85,22.7)(90,20.7)(95,20.7)(105,21.9)(110,23.0)(115,23.4)(120,21.9)(125,22.3)(130,20.7)(140,22.7)(145,22.7)(150,21.9)(155,22.7)(160,22.7)(165,22.7)(170,21.1)(175,21.9)(180,23.4)(185,22.3)(190,22.7)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% }
% 		\resizebox{0.47\textwidth}{!}{
% 		\begin{tikzpicture}[trim axis left,trim axis right]%\ref{target_legend6}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{I3D - Diving48}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
%         % xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=101,
%         ymin=13, ymax=45,
%         xtick={0,10,20,30,40,50,60,70,80,90,100},
%         ytick={20, 25, 30, 35, 40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.85, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.4,0)},anchor=south,row sep=0.01pt}, font =\small},
%         %  legend entries={[black]Dynamic,[black]Static},
%         % legend to name=target_legend6,
%     ]
%     % MOTION
%     \addplot[line width=1.6pt,mark size=1.1pt,color=blue]
%         coordinates {(0,14.8)(5,17.5)(10,17.4)(15,16.4)(20,17.6)(25,17.0)(30,17.4)(35,17.0)(40,17.3)(45,18.0)(50,17.6)(55,17.2)(60,17.5)(65,17.3)(70,17.6)(75,17.4)(80,17.6)(85,17.7)(90,17.9)(95,17.5)(100,17.5)};
%     % APPEARANCE
%     \addplot[line width=1.6pt,mark size=1.1pt,color=red]
%         coordinates {(0,41.7)(5,38.9)(10,37.8)(15,39.6)(20,37.6)(25,38.7)(30,38.8)(35,38.8)(40,38.3)(45,37.6)(50,38.2)(55,38.6)(60,38.4)(65,38.2)(70,38.2)(75,38.2)(80,38.1)(85,38.0)(90,37.7)(95,38.2)(100,38.4)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% \hspace{0.3cm}
% \begin{tikzpicture}[trim axis left,trim axis right]%\ref{target_legend7}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{SlowFast - Diving48}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
%         % xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=101,
%         ymin=13, ymax=45,
%         xtick={0,10,20,30,40,50,60,70,80,90,100},
%         ytick={20,25,30,35,40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.7, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.9,3.4)},anchor=south,row sep=0.01pt}, font =\normalsize},
%         %  legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
%         % legend to name=target_legend7,
%     ]
%     % CAT
%     % MOTION
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=orange,mark=*,]
%     %     coordinates {(0,20.4)(5,23.1)(10,23.4)(15,25.7)(25,24.3)(45,27.2)(50,25.7)(60,28.7)(75,24.4)(80,25.7)(85,24.9)(90,25.3)(95,26.6)(105,25.3)(110,25.2)(115,24.4)(120,25.4)(125,24.8)(130,26.5)(140,25.0)(145,24.3)(150,24.6)(155,25.4)(160,25.0)(165,24.5)(170,25.0)(175,25.0)(180,24.2)(185,24.7)(190,24.5)};
%     % % APPEARANCE
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=cyan,mark=*,]
%     %     coordinates {(0,39.5)(5,35.4)(10,34.8)(15,33.4)(25,34.2)(45,28.3)(50,30.3)(60,27.6)(75,32.4)(80,31.4)(85,32.1)(90,32.2)(95,30.3)(105,30.1)(110,29.8)(115,32.7)(120,32.4)(125,32.9)(130,30.0)(140,32.2)(145,31.9)(150,32.5)(155,31.5)(160,31.5)(165,32.2)(170,31.7)(175,31.1)(180,32.3)(185,31.8)(190,31.9)};
        
%         % SLOW
%         % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,14.8)(5,22.1)(10,22.9)(15,22.9)(20,24.2)(25,24.9)(30,24.3)(35,25.1)(40,24.5)(45,24.8)(50,24.9)(55,24.6)(60,24.1)(65,24.2)(70,24.1)(75,24.7)(80,24.5)(85,24.3)(90,24.4)(95,24.1)(100,24.1)};
%     % APPEARANCE
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,42.8)(5,31.2)(10,29.9)(15,31.0)(20,28.9)(25,27.7)(30,28.2)(35,27.2)(40,27.6)(45,27.9)(50,28.2)(55,27.9)(60,28.9)(65,28.8)(70,28.7)(75,27.9)(80,28.0)(85,28.4)(90,28.2)(95,28.4)(100,28.7)};
        
        
        
%         % FAST
%         % MOTION
%     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,15.2)(5,27.3)(10,28.9)(15,28.5)(20,32.4)(25,27.0)(30,31.2)(35,29.3)(40,28.5)(45,24.7)(50,29.7)(55,28.9)(60,28.9)(65,29.3)(70,30.1)(75,28.9)(80,28.5)(85,29.7)(90,28.9)(95,28.5)(100,29.3)};
%     % APPEARANCE
%      \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,41.0)(5,21.5)(10,19.1)(15,21.1)(20,17.2)(25,21.1)(30,19.5)(35,20.3)(40,21.5)(45,27.7)(50,19.5)(55,20.3)(60,19.9)(65,20.3)(70,19.5)(75,19.9)(80,19.5)(85,19.9)(90,20.3)(95,19.9)(100,19.9)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% }
% 		\resizebox{0.47\textwidth}{!}{
% 		\begin{tikzpicture}[trim axis left,trim axis right]\ref{single_stream_leg}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{I3D - SSv2}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},        xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=31,
%         ymin=13, ymax=45,
%         xtick={0,5,10,15,20,25,30},
%         ytick={20, 25, 30, 35, 40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         legend style={
% 			legend columns=2,
%          nodes={scale=1, transform shape},
%          cells={anchor=west},
%          legend style={at={(3,0.15)},anchor=south,row sep=0.01pt}, font =\normalsize},
%          legend entries={[black]Dynamic,[black]Static},
%         legend to name=single_stream_leg,
%     ]
%     % MOTION
%     \addplot[line width=1.6pt,mark size=1.1pt,color=blue]
%         coordinates {(0,15.6)(1,25.6)(2,29.5)(3,28.7)(4,30.7)(5,30.4)(6,28.6)(7,33.5)(8,32.2)(9,33.3)(10,30.0)(11,28.6)(12,31.1)(13,30.1)(14,29.1)(15,34.1)(16,29.9)(17,30.2)(18,32.9)(19,29.5)(20,30.5)(21,29.7)(22,29.1)(23,29.4)(24,32.8)(25,30.7)(26,32.8)(27,30.0)(28,29.9)(29,30.5)(30,29.7)};
%     % APPEARANCE
%     \addplot[line width=1.6pt,mark size=1.1pt,color=red]
%         coordinates {(0,42.6)(1,35.0)(2,31.2)(3,30.7)(4,28.2)(5,28.0)(6,30.2)(7,25.3)(8,27.3)(9,26.3)(10,29.1)(11,30.0)(12,27.3)(13,28.6)(14,29.8)(15,24.7)(16,28.8)(17,28.6)(18,26.3)(19,29.7)(20,28.5)(21,29.4)(22,30.3)(23,29.6)(24,26.2)(25,28.4)(26,26.5)(27,28.9)(28,28.9)(29,28.4)(30,29.0)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% \hspace{0.3cm}
% \begin{tikzpicture}[trim axis left,trim axis right]\ref{two_stream_leg}
%     \begin{axis}[
%       line width=1.0,
%         title={\textbf{SlowFast - SSv2}},
%         title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\large},
%         xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=23,
%         ymin=13, ymax=45,
%         xtick={0,5,10,15,20},
%         ytick={20, 25, 30, 35, 40},
%         x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         legend style={
% 		 legend columns=2,
%          nodes={scale=1, transform shape},
%          cells={anchor=west},
%          legend style={at={(3,0.15)},anchor=south,row sep=0.01pt}, font =\normalsize},
%          legend entries={[black]DynSlow,[black]StatSlow,[black]DynFast,[black]StatFast},
%         legend to name=two_stream_leg,
%     ]
%     % CAT
%     % MOTION
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=orange,mark=*,]
%     %     coordinates {(0,20.4)(5,23.1)(10,23.4)(15,25.7)(25,24.3)(45,27.2)(50,25.7)(60,28.7)(75,24.4)(80,25.7)(85,24.9)(90,25.3)(95,26.6)(105,25.3)(110,25.2)(115,24.4)(120,25.4)(125,24.8)(130,26.5)(140,25.0)(145,24.3)(150,24.6)(155,25.4)(160,25.0)(165,24.5)(170,25.0)(175,25.0)(180,24.2)(185,24.7)(190,24.5)};
%     % % APPEARANCE
%     % \addplot[line width=1.6pt,mark size=1.1pt,color=cyan,mark=*,]
%     %     coordinates {(0,39.5)(5,35.4)(10,34.8)(15,33.4)(25,34.2)(45,28.3)(50,30.3)(60,27.6)(75,32.4)(80,31.4)(85,32.1)(90,32.2)(95,30.3)(105,30.1)(110,29.8)(115,32.7)(120,32.4)(125,32.9)(130,30.0)(140,32.2)(145,31.9)(150,32.5)(155,31.5)(160,31.5)(165,32.2)(170,31.7)(175,31.1)(180,32.3)(185,31.8)(190,31.9)};
        
%         % SLOW
%         % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,15.0)(2,31.2)(4,30.1)(6,29.2)(8,29.2)(10,29.1)(12,29.0)(14,28.7)(16,28.7)(18,28.6)(20,28.5)(22,28.5)};
%     % APPEARANCE
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,42.1)(2,25.8)(4,24.0)(6,22.7)(8,24.4)(10,24.5)(12,24.3)(14,23.4)(16,23.8)(18,23.5)(20,24.0)(22,23.8)};
        
%         % FAST
%         % MOTION
%     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(0,14.1)(2,30.1)(4,31.2)(6,29.3)(8,30.5)(10,32.0)(12,30.9)(14,31.6)(16,32.8)(18,32.8)(20,32.0)(22,33.2)};
%     % APPEARANCE
%      \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(0,43.0)(2,26.6)(4,22.3)(6,21.9)(8,23.0)(10,23.8)(12,24.6)(14,24.6)(16,24.2)(18,23.4)(20,23.8)(22,23.0)};
% \end{axis}

% % \begin{axis}[
% %   width=8cm,
% %   height=6cm,  
% %   axis y line*=right,
% %   axis x line=none,
% %   ymin=0, ymax=0.175,
% %   ylabel={Learning Rate (\%)},
% %   y tick label style={font=\footnotesize},
% % %   y label style={at={(axis description cs:-0.08,.5)},anchor=south,font=\normalsize},
% % ]
% %     \addplot[dotted,line width=0.8pt,mark size=0.5pt,color=gray]
% %         coordinates {(0,0.01)(5,0.02217016738)(10,0.03434033475)(15,0.04651050213)(20,0.0586806695)(25,0.07085083688)(30,0.08302100425)(35,0.09233620996)(40,0.09007068109)(45,0.08754792207)(50,0.08478412753)(55,0.08179703939)(60,0.07860583301)(70,0.07169418696)(75,0.06801811599)(80,0.06422637933)(85,0.06034331771)(90,0.05639385808)(95,0.05240335366)(105,0.04440177619)(110,0.04044206856)(115,0.03654371722)(120,0.03273174728)(135,0.02205512133)(140,0.01882550991)(145,0.01579602033)(150,0.01298610015)(155,0.01041378738)(160,0.008095594755)(165,0.006046403714)(170,0.004279368849)(180,0.001635256848)(185,0.0007751533516)(190,0.0002310443525)(195,0.00000642271000343974)};
        
% % \end{axis}

% \end{tikzpicture}
% }
% \end{center}
% 	\caption{The encoding of static and dynamic factors in an I3D~\cite{carreira2017quo} (8x8 R18) and SlowFast~\cite{feichtenhofer2019slowfast} (4x16 R18) over the course of training on Kinetics-400.}\label{fig:ar_per_epoch}
% \end{figure}





% \begin{figure}
% \resizebox{0.45\textwidth}{!}{
% \begin{tikzpicture}[trim axis left,trim axis right] \ref{vos_dataset_per_epoch_legend}
% \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet Fusion 2}},
%         title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
%         %xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=8, ymax=55,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\large},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         legend style={
% 		 legend columns=2,
%          nodes={scale=0.85, transform shape},
%          cells={anchor=west},
%          legend style={at={(3.21,0.13)},anchor=south,row sep=0.01pt}, font =\normalsize},
%          legend entries={[black]Stat-DAVIS+YTB,[black]Dyn-DAVIS+YTB,[black]Stat-DAVIS,[black]Dyn-DAVIS},
%         legend to name=vos_dataset_per_epoch_legend,
%     ]
%     % DAVIS + YTB
%   % Appearance
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates{(1,28.8)(2,27.7)(3,27.0)(4,26.4)(5,26.2)(6,26.6)(7,26.2)(8,26.9)(9,25.5)(10,27.4)(11,27.2)(12,26.6)(13,27.0)(14,26.5)(15,26.8)(16,26.4)(17,27.7)(18,25.5)(19,26.6)(20,27.8)};
%   % MOTION
%   \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%             coordinates{(1,28.6)(2,30.2)(3,31.2)(4,32.5)(5,32.4)(6,31.4)(7,32.3)(8,31.3)(9,33.6)(10,30.7)(11,31.0)(12,31.6)(13,31.3)(14,32.4)(15,31.6)(16,31.6)(17,30.5)(18,33.8)(19,31.1)(20,30.6)};
    
%     % DAVIS
%     %APP
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red,style=dotted]
%     coordinates{(1,35.4)(2,35.2)(3,34.4)(4,36.9)(5,31.4)(6,31.0)(7,39.0)(8,32.8)(9,37.6)(10,38.5)(11,29.4)(12,37.0)(13,35.5)(14,33.4)(15,34.0)(16,28.8)(17,31.2)(18,28.3)(19,34.5)(20,31.6)};
%     % MOT
%   \addplot[line width=1.2pt,mark size=1.1pt,color=blue,style=dotted]
%     coordinates {(1,21.9)(2,21.4)(3,22.8)(4,20.3)(5,24.5)(6,23.1)(7,18.1)(8,22.0)(9,19.2)(10,19.6)(11,27.6)(12,19.8)(13,18.9)(14,22.5)(15,23.0)(16,23.9)(17,24.1)(18,26.0)(19,21.0)(20,24.3)};
     
% \end{axis}
% \end{tikzpicture}%
% \hspace{0.5cm}
% \begin{tikzpicture}[trim axis left,trim axis right]%\ref{vos_dataset_per_epoch_legend}
%   \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet - Fusion 5}},
%         title style={at={(axis description cs:0.5,0.94)},anchor=north,font=\normalsize},
%         %xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=8, ymax=55,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
% %         legend style={
% % 		 legend columns=2,
% %          nodes={scale=0.85, transform shape},
% %          cells={anchor=west},
% %          legend style={at={(3.1,0.13)},anchor=south,row sep=0.01pt}, font =\normalsize},
% %          legend entries={[black]Stat-DAVIS+YTB,[black]Dyn-DAVIS+YTB,[black]Stat-DAVIS,[black]Dyn-DAVIS},
% %         legend to name=vos_dataset_per_epoch_legend,
%     ]
%     % DAVIS + YTB
%     % APP
%      \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%             coordinates{(1,29.5)(2,24.4)(3,31.9)(4,34.4)(5,31.6)(6,21.3)(7,33.8)(8,31.9)(9,34.7)(10,35.3)(11,16.3)(12,30.8)(13,34.7)(14,15.0)(15,14.4)(16,34.1)(17,34.3)(18,31.1)(19,32.2)(20,31.0)};
            
%     % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%             coordinates{(1,24.1)(2,37.0)(3,23.0)(4,24.3)(5,23.2)(6,21.2)(7,24.5)(8,23.0)(9,24.1)(10,23.5)(11,48.3)(12,23.7)(13,23.9)(14,45.0)(15,47.1)(16,24.5)(17,24.1)(18,23.6)(19,23.4)(20,24.0)};
            
%     % DAVIS
%     % App
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red,style=dotted]
%         coordinates {(1,18.4)(2,16.3)(3,22.6)(4,35.8)(5,32.2)(6,33.3)(7,27.6)(8,35.2)(9,36.6)(10,34.8)(11,33.2)(12,27.3)(13,33.2)(14,33.8)(15,35.2)(16,33.3)(17,33.7)(18,33.3)(19,34.4)(20,33.5)};
%     % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue,style=dotted]
%         coordinates {(1,35.3)(2,41.0)(3,30.8)(4,22.1)(5,22.1)(6,20.4)(7,21.9)(8,23.1)(9,20.4)(10,23.2)(11,25.4)(12,23.1)(13,18.9)(14,24.4)(15,22.7)(16,25.0)(17,24.3)(18,24.7)(19,23.9)(20,24.8)};
    
% \end{axis}
% \end{tikzpicture}}
% \caption{The encoding of static and dynamic factors over the course of training for our best performing model MATNet that balances static and dynamic factors, when trained with DAVIS only and DAVIS + YouTube-VOS.}\label{fig:vos_iterwise}
% \end{figure}

% \begin{figure}
% \resizebox{0.47\textwidth}{!}{
% \begin{tikzpicture}[trim axis left,trim axis right] %\ref{target_legend_iterwise_vos}
% \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet - DAVIS+YTB - Fusion 2}},
%         title style={at={(axis description cs:0.5,1.1)},anchor=north,font=\normalsize},
%         %xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=10, ymax=50,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\large},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         legend style={
% 		 legend columns=2,
%          nodes={scale=1, transform shape},
%          cells={anchor=west},
%          legend style={at={(3,0.15)},anchor=south,row sep=0.01pt}, font =\normalsize},
%          legend entries={[black]Static,[black]Dynamic},
%         legend to name=target_legend_iterwise_vos,
%     ]
%   % Appearance
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates{(1,28.8)(2,27.7)(3,27.0)(4,26.4)(5,26.2)(6,26.6)(7,26.2)(8,26.9)(9,25.5)(10,27.4)(11,27.2)(12,26.6)(13,27.0)(14,26.5)(15,26.8)(16,26.4)(17,27.7)(18,25.5)(19,26.6)(20,27.8)};
%   % MOTION
%   \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%             coordinates{(1,28.6)(2,30.2)(3,31.2)(4,32.5)(5,32.4)(6,31.4)(7,32.3)(8,31.3)(9,33.6)(10,30.7)(11,31.0)(12,31.6)(13,31.3)(14,32.4)(15,31.6)(16,31.6)(17,30.5)(18,33.8)(19,31.1)(20,30.6)};
     
% \end{axis}
% \end{tikzpicture}%
% \hspace{0.5cm}
% \begin{tikzpicture}[trim axis left,trim axis right]%\ref{target_legend_iterwise_vos_1}
%   \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet - DAVIS+YTB - Fusion 5}},
%         title style={at={(axis description cs:0.5,1.1)},anchor=north,font=\normalsize},
%         %xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=10, ymax=50,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.5, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.6,3.4)},anchor=south,row sep=0.01pt}, font =\small},
%     ]
%      \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%             coordinates{(1,29.5)(2,24.4)(3,31.9)(4,34.4)(5,31.6)(6,21.3)(7,33.8)(8,31.9)(9,34.7)(10,35.3)(11,16.3)(12,30.8)(13,34.7)(14,15.0)(15,14.4)(16,34.1)(17,34.3)(18,31.1)(19,32.2)(20,31.0)};
            
%     % MOTION
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%             coordinates{(1,24.1)(2,37.0)(3,23.0)(4,24.3)(5,23.2)(6,21.2)(7,24.5)(8,23.0)(9,24.1)(10,23.5)(11,48.3)(12,23.7)(13,23.9)(14,45.0)(15,47.1)(16,24.5)(17,24.1)(18,23.6)(19,23.4)(20,24.0)};
    
% \end{axis}
% \end{tikzpicture}}
% \resizebox{0.47\textwidth}{!}{
% \begin{tikzpicture}[trim axis left,trim axis right] \ref{target_legend_iterwise_vos}
% \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet - DAVIS - Fusion 2}},
%         title style={at={(axis description cs:0.5,1.1)},anchor=north,font=\normalsize},
%         xlabel={Epoch},
%         x label style={font=\small},
%         ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=10, ymax=50,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         y label style={at={(axis description cs:.14,.5)},anchor=south,font=\large},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.5, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.6,3.4)},anchor=south,row sep=0.01pt}, font =\small},
%     ]
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%     coordinates{(1,35.4)(2,35.2)(3,34.4)(4,36.9)(5,31.4)(6,31.0)(7,39.0)(8,32.8)(9,37.6)(10,38.5)(11,29.4)(12,37.0)(13,35.5)(14,33.4)(15,34.0)(16,28.8)(17,31.2)(18,28.3)(19,34.5)(20,31.6)};
    
%   \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%     coordinates {(1,21.9)(2,21.4)(3,22.8)(4,20.3)(5,24.5)(6,23.1)(7,18.1)(8,22.0)(9,19.2)(10,19.6)(11,27.6)(12,19.8)(13,18.9)(14,22.5)(15,23.0)(16,23.9)(17,24.1)(18,26.0)(19,21.0)(20,24.3)};
     
% \end{axis}
% \end{tikzpicture}%
% \hspace{0.5cm}
% \begin{tikzpicture}[trim axis left,trim axis right]\ref{target_legend_iterwise_vos}
%   \begin{axis}[
%       line width=1.0,
%         title={\textbf{MATNet - DAVIS - Fusion 5}},
%         title style={at={(axis description cs:0.5,1.1)},anchor=north,font=\normalsize},
%         xlabel={Epoch},
%         x label style={font=\small},
%         % ylabel={Dimensions (\%)},
%         xmin=0, xmax=21,
%         ymin=10, ymax=50,
%         xtick={1,3,5,7,9,11,13,15,17,19,21},
%         ytick={10, 15, 20, 25, 30, 35, 40, 45, 50},
%          x tick label style={font=\small, rotate=60},
%         y tick label style={font=\footnotesize},
%         x label style={at={(axis description cs:0.5,0)},anchor=north,font=\normalsize},
%         % y label style={at={(axis description cs:0.1,.5)},anchor=south,font=\normalsize},
%         width=8cm,
%         height=6cm,        
%         ymajorgrids=false,
%         xmajorgrids=false,
%         % major grid style={dotted,green!20!black},
%         % legend style={
%         %  nodes={scale=0.5, transform shape},
%         %  cells={anchor=west},
%         %  legend style={at={(1.6,3.4)},anchor=south,row sep=0.01pt}, font =\small},
%     ]
%     \addplot[line width=1.2pt,mark size=1.1pt,color=red]
%         coordinates {(1,18.4)(2,16.3)(3,22.6)(4,35.8)(5,32.2)(6,33.3)(7,27.6)(8,35.2)(9,36.6)(10,34.8)(11,33.2)(12,27.3)(13,33.2)(14,33.8)(15,35.2)(16,33.3)(17,33.7)(18,33.3)(19,34.4)(20,33.5)};
    
%     \addplot[line width=1.2pt,mark size=1.1pt,color=blue]
%         coordinates {(1,35.3)(2,41.0)(3,30.8)(4,22.1)(5,22.1)(6,20.4)(7,21.9)(8,23.1)(9,20.4)(10,23.2)(11,25.4)(12,23.1)(13,18.9)(14,24.4)(15,22.7)(16,25.0)(17,24.3)(18,24.7)(19,23.9)(20,24.8)};
    
% \end{axis}
% \end{tikzpicture}}
% \caption{The encoding of static and dynamic factors over the course of training for our best performing model MATNet that balances static and dynamic factors, when trained with DAVIS only and DAVIS + YouTube-VOS.}\label{fig:vos_iterwise}
% \end{figure}

\vspace{-0.2cm}
\subsubsection{Video Segmentation}
\label{sec:epochwise_vos}
We train MATNet two datasets: (i) DAVIS16 only (DAVIS) and (ii) DAVIS16 combined with YouTube-VOS (DAVIS+YTB) as originally proposed~\cite{zhou2020motion}. Figure~\ref{fig:per_epoch} (bottom) shows the epoch-wise biases learned by MATNet on both settings. When trained on DAVIS+YTB, fusion layer 2 learns more dynamics compared to DAVIS alone, which confirms our previous findings (see Fig.~\ref{fig:vos_dataset_indiv} fusion layer 2). Additionally, when trained on DAVIS+YTB, the model quickly converges toward being dynamics biased. On the other hand, fusion layer 5 shows an interesting pattern of alternation between the static and dynamic factors throughout training and culminates to being static biased. These results align with our previous findings that MATNet's early fusion layers converge to being dynamics biased, unlike late fusion layers (see Fig.~\ref{fig:stagewise_vos}c). This result may stem from the fact that deeper layers tend to capture more abstract information compared to earlier layers. When trained on DAVIS, the final fusion layer becomes static biased in the early epochs, which aligns with the findings from action recognition.

\vspace{-0.2cm}
\subsubsection{Summary and shared insights}
All models in both tasks converge to their culminating biases within the first half of training epochs, except for MATNet trained on DAVIS+YTB. We also observed an interaction between models and datasets in which certain combinations of the two produce significantly more stability in their learned biases than others over the course of training.


